Trustworthy Machine Learning under Social and Adversarial Data Sources

Machine learning has witnessed remarkable breakthroughs in recent years. As machine learning permeates various aspects of daily life, individuals and organizations increasingly interact with these systems, exhibiting a wide range of social and adversarial behaviors. These behaviors may have a notable impact on the behavior and performance of machine learning systems. Specifically, during these interactions, data may be generated by strategic individuals, collected by self-interested data collectors, possibly poisoned by adversarial attackers, and used to create predictors, models, and policies satisfying multiple objectives. As a result, the machine learning systems' outputs might degrade, such as the susceptibility of deep neural networks to adversarial examples (Shafahi et al., 2018; Szegedy et al., 2013) and the diminished performance of classic algorithms in the presence of strategic individuals (Ahmadi et al., 2021). Addressing these challenges is imperative for the success of machine learning in societal settings.

==> calibrated/ec-src/camara.tex <==
\section{Comparison to \cite{camara2020mechanisms}\hsedit{tbd}}
\subsection{A set of alternative assumptions}
In this section, we propose a set of alternative assumptions, which are weaker than assumptions in \cite{camara2020mechanisms}.
The main difference of assumptions in this subsection from those in Section~\ref{sec:general} is that under the constant mechanism $\sigma^{p_0}$, the signal $I_t$ in round $t$ is $(p_t,r_t,p^0,r^{p_0}_t, a^{p_0}_t)$ instead of $(p^0,r^{p_0}_t, a^{p_0}_t)$.

\begin{definition}[finer multi-calibration error of the forecast]
We consider the calibration error on finer partition of the sequence.
For the proposed mechanism $\sigma^\dagger$, similar to Definition~\ref{def:principal-cal}, we consider the calibration error on the subsequences defined by the policy and the recommendation.
For the fixed constant mechanisms $\{\sigma^{p_0}\}_{p_0\in \cP}$, we consider the calibration error on the subsequences defined by the policy, the recommendation and the policy-recommmendation under the proposed mechanism.
forand the calibration error on the subsequences defined by the policy, the recommendation for
Specifically, let $E' = \{S_{p,r}|(p,r)\in \cP\times \cA\} \cup \{S''_{p_0,r,p',r'}|(p_0,r,p',r')\in \cP\times \cA\times \cP\times \cA\}$ where
\begin{equation*}
    S_{p,r} = \{\pi| \brp(\pi) = p , \brr(p,\pi) =r\}\,,
\end{equation*}
and 
\begin{equation*}
    S''_{p_0,r,p',r'} : = \{\pi|\brr(p_0,\pi) =r, \brp(\pi) = p' , \brr(p',\pi) =r'\}\,.
\end{equation*}
We say the multi-calibration error is upper bounded by $\alpha'$ if $\calerr(S)\leq \alpha'$ for all $S\in E'$.
\end{definition}

\begin{definition}[signal]
    Under the proposed mechanism $\sigma^\dagger$, the signal $I^\dagger_t = (p_t,r_t,a_t)$ is the triple of the policy, the recommendation and the action.
    Under the constant mechanism $p_0\in \cP$, the signal $I^{p_0}_t = (p_t,r_t,p^0,r^{p_0}_t, a^{p_0}_t)$ is a tuple of the policy and the recommendation under $\sigma^\dagger$, and the policy, the recommendation and the action under $\sigma^{p_0}$. 
\end{definition}

\begin{assumptionp}{\ref*{asp:alignment}$'$}[alignment]\label{asp-alt:alignment}
   We assume that there exists a constant $M>0$ such that for any prior distribution $\pi$ and signal structure $\gamma$, for any $\epsilon$-approximately optimal response $\mu^\epsilon(\gamma, p^*(\pi),\pi)$ to $(\gamma, p^*(\pi),\pi)$, we have
    \begin{align}
        &V(a^*(p^*(\pi), \pi), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(\mu_I^\epsilon(\gamma, p^*(\pi),\pi), p^*(\pi),y)}}\nonumber\\
        \leq& M (\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(a^*_I(\gamma, p^*(\pi),\pi), p^*(\pi),y)}} - U(a^*(p^*(\pi), p^*(\pi), \pi) ) + \epsilon\,;\label{eq:alignment-alt}
    \end{align}
   and for any fixed policy $p_0\in \cP$, for any $\epsilon$-approximately optimal response $\mu^\epsilon(\gamma, p_0,\pi)$ to $(\gamma, p_0,\pi)$, we have
    \begin{align}
        &\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(\mu_I^\epsilon(\gamma, p_0,\pi), p_0,y)}}-\max_{p'\in \cP}V(a^*(p',\pi),p', \pi)\nonumber\\
        \leq& M (\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(a_I^*(\gamma, p_0,\pi), p_0,y)}} -  U(a^*(p_0), p_0, \pi) ) +  \epsilon\,.\label{eq:alignment-alt-2}
    \end{align}
\end{assumptionp}

\begin{assumptionp}{\ref*{asp:no-internal-reg}$'$}[no finer counterfactual internal regret for Agent]\label{asp-alt:no-finer-internal-reg}
Let $\ecf$ be an upper bound on the counterfactual internal regret with the context being the signal for the realized sequence of states $y_{1:T}$ and realized sequence of policies and recommendations generated by either the proposed mechanism or the constant mechanisms.
That is,
    \begin{equation*}        \cir(y_{1:T},p_{1:T},r_{1:T}):=\max_{h:\cP \times \cA\times \cA\mapsto \cA}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,r_t,a_t),p_t, y_t) - U(a_t,p_t,y_t)) \leq \ecf\,,
    \end{equation*}
    and for all $p_0\in \cP$,
    \begin{equation*}        
    \cir(y_{1:T},(p_0,\ldots,p_0),r^{p_0}_{1:T}):=\max_{h:\cP^2\times \cA^3\mapsto \cA}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,r_t, p_0, r^{p_0}_t,a^{p_0}_t),p_0, y_t) - U(a^{p_0}_t,p_0,y_t)) \leq \ecf\,.
    \end{equation*}
    We assume that there exists a small $\ecf$.
% Let $\eint$ be an upper bound on the internal regret with context of $(p_t,\rho_t, p^*_t, \rho^*_t, r_t)$ for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanisms.
\end{assumptionp}

% \begin{assumption}[Agent has no secret information.]\label{asp:no-sec-info}
% Let $\eneg$ be an upper bound on the negative cross-swap regret for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by the proposed mechanism and constant mechanisms.
% That is,
%     \begin{equation*}
%         \nr(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^*_t,p^*_t,y_t)- \max_{h:\cP\times \cA\mapsto \cA} \frac{1}{T}\sum_{t=1}^T U(h(p^*_t, \rho^{*}_t),p^*_t,y_t) \leq\eneg\,,
%     \end{equation*}
%     and for all $p\in \cP$,
%     \begin{equation*}
%         \nr(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^p_t,p,y_t)- \max_{h:\cP\times \cA\mapsto \cA} \frac{1}{T}\sum_{t=1}^T U(h(p, \rho^{p}_t),p,y_t) \leq\eneg\,.
%     \end{equation*}
%     We assume that there exists a small $\eneg$.
% \end{assumption}


\begin{theorem}
    Under Assumptions~\ref{asp-alt:alignment}, \ref{asp-alt:no-finer-internal-reg},\ref{asp:no-sec-info}, the Principal's regret satisfies that 
    \begin{equation*}
        \textrm{PR}(L, y_{1:T}) \leq \cO(\abs{\cP}\abs{\cA}\alpha + \eint + \eneg).
    \end{equation*}
\end{theorem}
\begin{proof}
    To prove the theorem, we will prove that
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^*,p_t,y_t)\geq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t,y_t)-(M+1)T\eint-MT\eneg -(4M+2)\calerr(\pip)\,,
\end{equation*}
and for all $p\in \cP$
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^p,p,y_t)\leq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t,y_t) +  (M+1)T\eint + MT \eneg\,.
\end{equation*}
The first part has been proved in Lemma~\ref{lmm:utility-difference}. We only need to prove the second part.
For any constant mechanism $\sigma^p$, now we consider the subsequence in which $\brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$. 
Let $t\in (p,\rho,p',\rho')$ to present $t: \brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$.
In this subsequence, we let the signal structure be $\hat\gamma_{p,\rho,p',\rho'}((p,\rho,r), y) := \frac{\sum_{t\in (p,\rho,p',\rho')} \ind{r^p_t = r, y_t = y}}{\sum_{t\in (p,\rho,p',\rho')} \ind{y_t = y}}$.
Then we have
\begin{align*}
        &\EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}} \\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} -2\norm{\pip_{p,\rho,p',\rho'}  - \hat y_{p,\rho,p',\rho'}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,\rho,p',\rho'}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,\rho,p',\rho'}}\nr^p_{p,\rho,p',\rho'}+\frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} +4\norm{\pip_{p,\rho,p',\rho'}  -\hat y_{p,\rho,p',\rho'}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt-ver2:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat y_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat y_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat y_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M\nr^p_{p,r}+\frac{1}{n_{p,r}}(M+1)\ir^p_{p,r} +(4M+2)\norm{\pip_{p,r}  -\hat y_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M\nr^p_{p,r}+\frac{1}{n_{p,r}}(M+1)\ir^p_{p,r} +(4M+2)\norm{\pip_{p,r}  -\hat y_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat y_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M+1)T\eint + MT \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\end{proof}

\subsection{Comparison to Theorem~5 of \cite{camara2020mechanisms}}
\cite{camara2020mechanisms} adopt $\epsilon$-robust policy.
The $\epsilon$-robust policy is worst-case optimal over all $\epsilon$-approximately optimal response distributions.
Formally, for any $p,\pi,\epsilon$, let $\cB(\pi,p,\epsilon)$ denote the set of all $\epsilon$-approximately optimal response distributions, i.e., 
\begin{equation*}
        \cB(\pi,p,\epsilon)=\{\mu\in \Delta(\cR)|\max_{\tilde r}\EEs{y\sim \pi}{U(\tilde r,p,y)} - \EEs{y\sim \pi}{\EEs{r\sim \mu}{U(r,p,y)}}\leq \epsilon\}\,.
\end{equation*}
The $\epsilon$-robust policy is $\argmax_{p\in \cP} \min_{r\in \cB(\pi,p,\epsilon)}$. Similarly, when there is a signal structure $\gamma$, let $\cB(\pi,p,\gamma,\epsilon)$ denote denotes the set of all $\epsilon$-approximately optimal responses given the signal $I$, i.e.,
    \begin{equation*}
        \cB(\pi,p,\gamma,\epsilon)=\left\{\mu_I\in\Delta(\mathcal{R})\mid\max_{\tilde{r}_I\in\mathcal{R}}\EEs{y\sim\pi}{\EEs{J
        \sim\gamma(\cdot,y)}{U(\tilde{r}_J,p,y)-\EEs{r\sim\mu_I}{U(r,p,y)}}}\leq \epsilon\right\}\,.
    \end{equation*}
    
\begin{assumption}[bounded cost of $\epsilon$-robustness]\label{camara-asp:eps-robust}
    For any distribution $\pi$, 
    \begin{equation*}
        \max_{p\in \cP} \max_{r\in \cB(\pi,p,\epsilon)}U(r,p,\pi) - \max_{p\in \cP} \min_{r\in \cB(\pi,p,\epsilon)}U(r,p,\pi) = \cO(\epsilon)\,.
    \end{equation*}
\end{assumption}
\begin{assumption}[$\epsilon$-bounded FCIR]\label{camara-asp:fcir}
\begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(\pip_t,r_t^*,(r_t^p)_{p\in\cP}),p_t, y_t) - U(r_t,p_t,y_t)) \leq \epsilon\,.
\end{equation*}    
\end{assumption}
\begin{assumption}[$\tilde \epsilon$-lower bounded FER]\label{camara-asp:fer}
    \begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(\pip_t),p_t, y_t) - U(r_t,p_t,y_t)) \geq -\tilde \epsilon\,.
\end{equation*} 
\end{assumption}
\begin{assumption}[Alignment. Assumption 9 of \cite{camara2020mechanisms}]\label{camara-asp:alignment}
For any prior distribution $\pi$, let $p^*(\pi)$ denote the policy deployed by the Principal when the forecast is $\pi$.
There exists a constant $M_1>0$ and a small $\epsilon>0$ s.t. for any prior distribution $\pi$ and signal structure $\gamma$,
    \begin{align*}
        &\min_{r\in \cB(\pi,p^*(\pi),\bar \epsilon)} V(r,p^*(\pi),\pi) - \min_{r_I\in \cB(\pi,p^*(\pi),\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right) +\epsilon\,,
    \end{align*}
    and 
    \begin{align*}
        &\max_{r_I\in \cB(\pi,p,\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p,y)}-\max_{\tilde p\in \cP}\max_{r\in \cB(\pi,\tilde p,\bar \epsilon)} V(r,p,\pi) \\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right) +\epsilon\,.
    \end{align*}

\end{assumption}
\begin{remark}
    Note that the deployed policy in \cite{camara2020mechanisms} is the $\epsilon$-robust policy $p^*(\pi) = \argmax_{p\in \cP} \min_{r\in \cB(\pi,p,\epsilon)}$ instead of $\brp(\pi)$ as we did in this work. Besides, the signal in our work is the action $I_t = r_t$ taken by the Agent while in \cite{camara2020mechanisms}, the signal is $I'_t = (\pip_t, r_t^*, (r^p_t)_{p\in \cP})$.
    Since no matter what mechanism is implemented, $I_t$ is always contained in $I'_t$, hence, for any structure $\gamma$ in our setting, we could define a corresponding structure $\gamma'$ with invariant $\pip_t$ and $r_t = r^*_t = r^p_t$ for all $p\in \cP$.
\end{remark}
\begin{theorem}[Theorem 5 of \cite{camara2020mechanisms}]
    Under Assumptions~\ref{camara-asp:eps-robust}, \ref{camara-asp:fcir}, \ref{camara-asp:fer} and \ref{camara-asp:alignment}, given that the forecast is fully calibrated, the Principal's regret is bounded.
\end{theorem}
We compare the assumptions in Table~\ref{tab:asp-compare}. 
\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
    ours & \citep{camara2020mechanisms}  \\\hline
     Principal forecast calibration (Assumption~\ref{asp:principal-cal}) & full calibration \\\hline
     Agent's forecast calibration (Assumption~\ref{asp:agent-cal})& \multirow{2}{*}{bounded FCIR (Assumption~\ref{camara-asp:fcir})} \\
     bounded internal regret (Assumption~\ref{asp-alt:no-internal-reg})&\\\hline
     lower bounded cross-swap regret (Assumption~\ref{asp:no-sec-info})& lower bounded FER (Assumption~\ref{camara-asp:fer})\\\hline
     Agent's utility margin (Assumption \ref{asp:utility-margin})& \multirow{2}{*}{alignment (Assumption~\ref{camara-asp:alignment})}\\
     alignment (Assumption~\ref{asp-alt:alignment})&\\\hline
     & bounded cost of $\epsilon$-robustness (Assumption~\ref{camara-asp:eps-robust})\\\hline
    \end{tabular}
    \caption{Comparison of assumptions}
    \label{tab:asp-compare}
\end{table}

\begin{lemma}
For any prior distribution $\pi$, let $p^*(\pi)$ denote the deployed policy. Under Assumption~\ref{camara-asp:eps-robust}, if Assumption~\ref{camara-asp:alignment} $\Rightarrow$ holds for $p^*(\cdot)$ and signal structure $\gamma$, then  Assumption~\ref{asp-alt:alignment} holds.\todohs{not right and not finished} 
\end{lemma}
\begin{proof}
By Assumption~\ref{camara-asp:alignment}, we have
    \begin{align*}
        &\min_{r\in \cB(\pi,p^*(\pi),\bar \epsilon)} V(r,p^*(\pi),\pi) - \min_{r_I\in \cB(\pi,p^*(\pi),\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right)+\epsilon\,.
    \end{align*}
    Since
    \begin{align*}
        \min_{r\in \cB(\pi,p^*(\pi),\bar \epsilon)} V(r,p^*(\pi),\pi) \geq& V(\tilde r(p^*(\pi)),p^*(\pi),\pi) - \bar \epsilon\tag{Assumption~\ref{camara-asp:eps-robust}}
    \end{align*}
    and for any $\bar \epsilon$-approximately optimal respond $(r_I^{\bar \epsilon})_{I\in \cI}$,
    \begin{align*}
        \min_{r_I\in \cB(\pi,p^*(\pi),\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p^*(\pi),y)} \leq \EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p^*(\pi),y)}\,,
    \end{align*}
    we have that 
    \begin{align*}
        &V(\tilde r(p^*(\pi)),p^*(\pi),\pi) - \bar \epsilon-\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right)+\epsilon\,.
    \end{align*}
    By rearranging terms, we have
\begin{align*}
    &V(\tilde r(p^*(\pi)),p^*(\pi),\pi) - \EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right)+\epsilon+\bar \epsilon\,.
\end{align*}
Thus, we have proved the first part of Assumption~\ref{asp-alt:alignment}.
    The proof of the second part is similar.
    By Assumption~\ref{camara-asp:alignment}, we have 
    \begin{align*}
        &\max_{r_I\in \cB(\pi,p,\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p,y)}-\max_{\tilde p\in \cP}\max_{r\in \cB(\pi,\tilde p,\bar \epsilon)} V(r,p,\pi) \\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)+\epsilon\,.
    \end{align*}
    For any $\bar \epsilon$-approximately optimal respond $(r_I^{\bar \epsilon})_{I\in \cI}$, we have
    \begin{align*}
        \max_{r_I\in \cB(\pi,p,\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p,y)}\geq \EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p,y)}\,.
    \end{align*}
    We also have
    \begin{align*}
        \max_{\tilde p\in \cP}\max_{r\in \cB(\pi,\tilde p,\bar \epsilon)} V(r,p,\pi)\leq \max_{\tilde p\in \cP} V(\brr(\tilde p,\pi),\tilde p,\pi) + \bar \epsilon\tag{Assumption~\ref{camara-asp:eps-robust}}\,.
    \end{align*}
    By combining these equations together, we have
    \begin{align*}
        &\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p,y)} - \max_{\tilde p\in \cP} V(\brr(\tilde p,\pi),\tilde p,\pi) - \bar \epsilon \\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)+\epsilon\,.
    \end{align*}
    Consider a distribution $\cD$ over $\pi$. In \cite{camara2020mechanisms}, the signal $I$ contains the forecast $\pi$, then we have
    \begin{align*}
         &\EEs{\pi\sim \cD}{\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p,y)} - \max_{\tilde p\in \cP} V(\brr(\tilde p,\pi),\tilde p,\pi)} - \bar \epsilon \\
        \leq& M_1\EEs{\pi\sim \cD}{\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)}+\epsilon\\
        =& M_1\max_{(r_I)_{I\in \cI}}\EEs{\pi\sim \cD}{\left( \EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)}+\epsilon
        \,.
    \end{align*}
\end{proof}

\begin{itemize}
    \item Assumption~\ref{asp:principal-cal} is weaker than full calibration.
    \item For both the proposed mechanism and the constant mechanism, when $\pip_t = \pip_\tau$, we have $(p_t,\rho_t)=(p_\tau,\rho_\tau)$.
    Assumption~\ref{asp-alt:no-internal-reg} assumes that
    \begin{equation*}
         \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,\rho_t,r_t),p_t, y_t) - U(r_t,p_t,y_t)) \leq \epsilon\,,
    \end{equation*}
    which is weaker than Assumption~\ref{camara-asp:fcir} as that $\pip_t = \pip_\tau$ implies that $(p_t,\rho_t) = (p_\tau,\rho_\tau)$.
    \item  Agent's utility margin (Assumption \ref{asp:utility-margin}) and alignment (Assumption~\ref{camara-asp:alignment}) are alternative assumptions to connect Principal's utility and Agent's utility.
    \item Assumption~\ref{asp:no-sec-info} looks to be stronger than Assumption~\ref{camara-asp:fer}. However, under full calibration,Assumption~\ref{asp:no-sec-info} is approximately equal to Assumption~\ref{camara-asp:fer}. Again, $\pip_t = \pip_\tau$ implies that $(p_t,\rho_t)=(p_\tau,\rho_\tau)$
    \begin{align*}
        &\max_{h}\frac{1}{T}\sum_{t=1}^T U(h(\pip_t),p_t, y_t)=\frac{1}{T}\sum_{\pi} \max_{r_\pi}\sum_{t:\pip_t = \pi} U(r_\pi,p_\pi, y_t)\\
        &=\frac{1}{T}\sum_{\pi} \max_{r_\pi}n_\pi U(r_\pi,p_\pi, \hat \pi_{\pi})\\
        &\approx_{(\text{full calibration})}\frac{1}{T}\sum_{\pi} \max_{r_\pi}\sum_{t:\pip_t = \pi} U(r_\pi,p_\pi, \pi)
        \\&= \frac{1}{T}\sum_{(p,r)\in \cP\times\cR}\sum_{\pi:p_\pi = p, \brr(p,\pi) =r}\max_{r_\pi}\sum_{t:\pip_t = \pi} U(r_\pi,p, \pi)\\
        &= \frac{1}{T}\sum_{(p,r)\in \cP\times\cR}n_{p,r} U(r,p, \pi_{p,r})\\
        &= \frac{1}{T}\sum_{(p,r)\in \cP\times\cR}\max_{\tilde r}n_{p,r} U(\tilde r,p, \pi_{p,r})\\
        &\approx_{(\text{full calibration})}\max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p_t, \rho_t),p_t,y_t)\,.
    \end{align*}   
    % \begin{align*}
    %     &\max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p_t, \rho_t),p_t,y_t) = \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}n_{p,r} \max_{\tilde r_{p,r}}U(\tilde r_{p,r},p,\hat \pi_{p,r})\\
    %     \geq & \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}n_{p,r} \max_{\tilde r_{p,r}}U(\tilde r_{p,r},p,\pi_{p,r}) - \abs{\cP}\abs{\cR}\alpha \tag{calibration error (Assumption~\ref{asp:principal-cal})}\\
    %     =& \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}\sum_{\pi: \brp(\pi) = p, \brr(p,\pi) =r}\sum_{t:\pip_t = \pi} U(r,p,\pip_t) - \abs{\cP}\abs{\cR}\alpha\tag{linearity}\\
    %     =& \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}\sum_{\pi: \brp(\pi) = p, \brr(p,\pi) =r}\max_{\tilde r}\sum_{t:\pip_t = \pi} U(\tilde r,p,\pip_t) - \abs{\cP}\abs{\cR}\alpha\tag{BR}\\
    %     =&\max_{h}\frac{1}{T}\sum_{t=1}^T U(h(\pip_t),p_t, y_t)
    % \end{align*}
\end{itemize}
\subsection{Unreasonableness of Assumptions in Theorem 2 of \cite{camara2020mechanisms}}
In Theorem~2 of \cite{camara2020mechanisms}, the $\pi_t$ is replaced with $p_t$ in the context. Again, they assumed bounded CIR, lower bounded ER and alignment.
\begin{assumption}[bounded CIR]
\begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,r_t^*,(r_t^p)_{p\in\cP}),p_t, y_t) - U(r_t,p_t,y_t)) \leq \epsilon\,.
\end{equation*}    
\end{assumption}
\begin{assumption}[lower-bounded ER]
    \begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t),p_t, y_t) - U(r_t,p_t,y_t)) \geq -\tilde \epsilon\,.
\end{equation*} 
\end{assumption}
\paragraph{Lower-bounded ER can be too stringent.}
Consider an example of contract design, where the contract space $\cP =\{1.5,1.6\}$, the action space of the Agent is $\{\text{work}, \text{shirk}\}$, and the nature state space is $\{\text{medium}, \text{hard}\}$. When the job is medium, working leads to success while shirking leads to failure; when the job is hard, both working and shirking lead to failure. The value of a job is $2$ and the cost of working is $1$.

Suppose that $y_t = \text{medium}$ for $t=1,\ldots,\frac{T}{2}$, and $y_t = \text{hard}$ for $t=\frac{T}{2}+1,\ldots,T$.
The Principal's forecast is $\abs{\sum_{t=1}^{\frac{T}{2}}\pi_t - y_t}$ is small, i.e., $\pi_t\approx y_t$ for most $t\leq \frac{T}{2}$. This should be true for any ``good'' forecaster (which has to maintain small calibration error for $y_t =\text{medium}$ for all $t=1\ldots,T$). 
Thus, the Principal's forecast is $\abs{\sum_{t=\frac{T}{2}+1}^{T}\pi_t - y_t}$ is small, i.e., $\pi_t\approx y_t$ for most $t> \frac{T}{2}$.
Consider the extreme case where $\pi_t = y_t$ for all $t\in [T]$.
The best in hindsight action is shirking and the utility of Agent is $0$.
Lower bounded ER requires the Agent to gain close to $0$ utility only, which not only assumes that the Agent has no extra information but also further restricts the Agent's behavior.

%\section{Auxiliary Lemmas}
%\begin{lemma}
%An Agent is best-responding to some predictor $\epsilon$-calibrated on the feature set $F$ iff they have $\epsilon$ regret, where the context is the Agent's own actions and $F$. 
%\end{lemma}
%\begin{proof}
%We will first show that calibration implies no internal regret.
%The Agent's payoff under the state sequence $y$ and the policy sequence $p$ can be written as



%$$\sum_{i=1}^{T}U(r_{t},p_{t},y_{t}) = \sum_{t =1}^{T}\sum_{f \in \mathcal{F}}U(r_{t},p_{t},y_{t})\ind{}$$

%Where $n_{f}$ is the number of rounds from $t=1$ to $T$ in which the context is $f$. 

%If $r_{t}$ is determined by the Agent best-responding to some predictor which is $\epsilon$-calibrated on $f \in F$, then 
%$$\sum_{f \in \mathcal{F}}U(r_{t},p_{t},y_{t})n_{f} - \sum_{f \in \mathcal{F}}U(r^{*},p_{t},\pi_{f})n_{f}$$

  %  \begin{equation*}
  %  \frac{1}{T} \norm{\sum_{t=1}^T \ind{(p_t ,\rho_t, \brr(p,\pir_t)) = (p,r,\bar r)} (\pir_t -y_t)}_1 \leq \alpha.
%\end{equation*}

%\end{proof}


==> calibrated/ec-src/general-bkup.tex <==
\section{Best response to forecasts}
We consider the case where both the Principal and the agent have (possibly different) forecasts and they always treat their forecasts as the true underlying prior and best respond to them.
More specifically, the interaction protocol is described as follows.
\begin{protocol}[H]
    \caption{Principal-Agent Interaction at round $t$}
    \label{prot:interaction}
        \begin{algorithmic}[1]
            \State{The Principal has a forecast $\pip_t$ and best responds to $\pip_t$ by choosing policy $p_t = \brp(\pip_t)$.}
            \State{The Principal has a recommendation of action to the agent based on her forecast $\pip_t$, i.e., $\rho_t = \brr(p_t,\pip_t)$.} 
            \State{The Principal reveals $(p_t, \rho_t)$ to the agent.}
            \State{The agent takes action $r_t$.}
            \State{The nature state $y_t$ is revealed.}
        \end{algorithmic}
    \end{protocol}

\subsection{Agent follows Principal's recommendation -- best responds to Principal's forecast}
We start with the simplest case where the agent follows the Principal's recommendation.
\begin{assumption}[calibration of Principal's forecast.]\label{asp:principal-cal}
For any sequence of nature states $y_{1:T}$, assume that for both the proposed mechanism $\sigma^*$ and the fixed constant mechanisms $\{\sigma^p\}_{p\in \cP}$, the principle's forecast $\pip_{1:T}$ is calibrated on the selected policy $p_t^*$ and the action taken by the agent $r_t^*$. More specifically, let $E = \{S_{p,r}|(p,r)\in \cP\times \cR\} \cup \{S'_{p,r}|(p,r)\in \cP\times \cR\}$ where
\begin{equation*}
    S_{p,r} : = \{\pi| \brp(\pi) = p , \brr(p,\pi) =r\}\,,
\end{equation*}
and 
\begin{equation*}
    S'_{p,r} : = \{\pi|\brr(p,\pi) =r\}\,.
\end{equation*}
More specifically, there exists a small $\alpha>0$ such that for any $S\in E$,
\begin{equation*}
    \frac{1}{T} \norm{\sum_{t=1}^T \ind{\pip_t \in S} (\pip_t -y_t)}_1 \leq \alpha.
\end{equation*}
\end{assumption}

\begin{lemma}\label{lmm:regret-follow-recommendation}
Under Assumption~\ref{asp:principal-cal}, the Principal's regret is bounded when the agent follows the Principal's recommendation. More specifically, we have
    \begin{align*}
        \max_{p\in \cP} \frac{1}{T}\sum_{t=1}^T \left(V(\rho_t^p, p, y_t)-V(\rho_t^*, p^*_t, y_t)\right) \leq  2\abs{\cP}\abs{\cR}\alpha\,,
    \end{align*}
    where $\rho_t^p = \brr(p,\pip_t)$ and $\rho_t^* = \brr(p^*_t,\pip_t)$ are recommendations under constant mechanism $\sigma^p$ and the proposed mechanism $\sigma^*$ respectively.
\end{lemma}
\begin{proof}
For any $S\in E$, let $\calerr(\pip,S) = \frac{1}{T} \norm{\sum_{t:\pip_t\in S} (\pip_t-y_t)}_1$ denote the calibration error on $S$.
Let $\calerr(\pip) = \max\left(\sum_{p,r} \calerr(\pip,S_{p,r}), \max_{p}\sum_{r}\calerr(\pip,S'_{p,r})\right)$, which is upper bounded by $\abs{\cP}\abs{\cR}\alpha$ under Assumption~\ref{asp:principal-cal}.
For proposed mechanism $\sigma^*$, let $t\in (p,r)$ denote $t:(p_t^*,\rho_t^*) = (p,r)$. Let $n_{p,r} = \sum_{t=1}^T\ind{t\in (p,r)}$ denote the number of rounds in which $(p_t^*,\rho_t^*) = (p,r)$. 
Let $\hat \pi_{p,r} = \frac{1}{n_{p,r}}\sum_{t\in (p,r)} y_t$ denote the empirical distribution of states in these rounds and $\pip_{p,r} = \frac{1}{n_{p,r}}\sum_{t\in (p,r)} \pip_t$ denote the empirical distribution of the forecasts.
For constant mechanism $\sigma^p$, let $t\in (r)$ denote $t: \rho_t^p = r$. 
Then we have
    \begin{align*}
        &\sum_{t=1}^T V(\rho_t^*,p_t^*,y_t) \\
        =& \sum_{(p,r)\in \cP\times \cR} \sum_{t\in (p,r)} V(r,p,y_t)\\
        =& \sum_{(p,r)\in \cP\times \cR} n_{p,r} \inner{V(r,p,\cdot)}{\hat \pi_{p,r}} \\
        \geq & \sum_{(p,r)\in \cP\times \cR} \left(n_{p,r} \inner{V(r,p,\cdot)}{\pip_{p,r}} -T\cdot\calerr(\pip,S_{p,r})\right)\tag{{calibration on }$S_{p,r}$}\\
        = & \sum_{(p,r)\in \cP\times \cR} \sum_{t\in(p,r)} \inner{V(\brr(p,\pip_t),p,\cdot)}{\pip_t} -T\cdot\calerr(\pip)\\
        \geq& \sum_{(p,r)\in \cP\times \cR} \sum_{t\in(p,r)} \max_{p'\in\cP}\inner{V(\brr(p',\pip_t),p',\cdot)}{\pip_t} -T\cdot\calerr(\pip) \tag{{best response}}\\
        \geq& \max_{p'\in\cP} \sum_{t=1}^T \inner{V(\brr(p',\pip_t),p',\cdot)}{\pip_t} -T\cdot\calerr(\pip)\\
        =& \max_{p'\in\cP} \sum_{r}\sum_{t:\brr(p',\pip_t) =r} \inner{V(r,p',\cdot)}{\pip_t} -T\cdot\calerr(\pip)\\
        \geq & \max_{p'\in\cP} \sum_{r}\left(\sum_{t:\brr(p',\pip_t) =r} V(r,p',y_t) - T
        \cdot\calerr(\pip, S'_{p',r})\right) -T\cdot\calerr(\pip)\tag{calibration on $S'_{p',r}$}\\
        =& \max_{p'\in \cP}\sum_{t=1}^T V(\rho_t^{p'}, p',y_t)-2T\cdot\calerr(\pip)\,.
    \end{align*}
    Under Assumption~\ref{asp:principal-cal}, we have $2T\cdot\calerr(\pip) \leq 2\alpha T$. We are done with the proof.
\end{proof}

\subsection{Agent best respond to her own forecast}
The agent does not necessarily follow the Principal's recommendation.
Instead, the agent could have her own forecast of nature states and best responds to it.

\begin{assumption}[calibration of agent's forecast.]\label{asp:agent-cal}
Suppose that the agent has a forecast $\pir_{1:T}$. At round $t$, the agent best responds to $(p_t,\pir_t)$ by taking $r_t = \brr(p_t,\pir_t)$. For any sequence of nature states $y_{1:T}$ and any realized sequence of policies $p_{1:T}$,  
    the agent's forecast is calibrated on time steps $t$ where $p_t = p, \rho_t=\brr(p_t,\pip_t) = \rho$ and $\brr(p_t, \pir_t) =  r$ for all $(p,\rho, r) \in \cP\times \cR\times \cR$. More specifically, there exists a small $\alpha>0$ such that for all $(p,\rho, r)\in \cP\times \cR\times \cR$, 
    \begin{equation*}
    \frac{1}{T} \norm{\sum_{t=1}^T \ind{(p_t ,\rho_t, \brr(p,\pir_t)) = (p,\rho, r)} (\pir_t -y_t)}_1 \leq \alpha\,,
\end{equation*}
\end{assumption}

\begin{assumptionp}{\ref*{asp:agent-cal}$'$}[no internal regret for agent]\label{asp-alt:no-internal-reg}
Let $\eint$ be an upper bound on the internal regret with context of $(p_t,\rho_t, r_t)$ for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanisms.
That is,
    \begin{equation*}        \ir(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\max_{h:\cP\times \cR\times \cR\mapsto \cR}\frac{1}{T}\sum_{t=1}^T (U(h(p^*_t,\rho^{*}_t,r^*_t),p^*_t, y_t) - U(r^*_t,p^*_t,y_t)) \leq \eint\,,
    \end{equation*}
    and for all $p\in \cP$,
    \begin{equation*}        \ir(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\max_{h:\cP\times \cR\times \cR\mapsto \cR}\frac{1}{T}\sum_{t=1}^T (U(h(p,\rho^{p}_t,r^p_t),p, y_t) - U(r^p_t,p,y_t)) \leq \eint\,.
    \end{equation*}
    We assume that there exists a small $\eint$.
    % There exists a small $>0$ such that for any sequence of nature states $y_{1:T}$ and any realized sequence of policies $p_{1:T}$,  the agent's achieves no-internal regret, i.e.,
\end{assumptionp}
For the proposed mechanism $\sigma^*$, let 
    $$\ir^*_{p,\rho} = \max_{h:\cR\mapsto \cR}\sum_{t\in (p,\rho)} \left(U(h(r^*_t),p^*_t, y_t) - U(r^*_t,p^*_t,y_t)\right)$$
    denote the internal regret for the agent in the rounds where  $(p^*_t,\rho^{*}_t) = (p,\rho)$.
    For the fixed mechanism $\sigma^p$, let 
    $$\ir^p_{\rho} = \max_{h:\cR\mapsto \cR}\sum_{t\in (\rho)} \left(U(h(r^p_t),p, y_t) - U(r^p_t,p,y_t)\right)$$
    denote the internal regret for the agent in the rounds where $\rho^{p}_t =  \rho$.
% Let $\ir^*_{p,r} = \max_{h:\cR\mapsto \cR}\sum_{t\in (p,r)} U(h(r_t),p_t, y_t) - U(r_t,p_t,y_t)$ denote the internal regret for the agent for the time steps $(p_t,\rho_t) = (p,r)$.
% By Assumption~\ref{asp-alt:no-internal-reg}, we have $\sum_{p,r}\ir_{p,r} \leq \epsilon T$.
\begin{remark}
    Note that Assumption~\ref{asp-alt:no-internal-reg} is weaker than Assumption~\ref{asp:agent-cal}.
    When Assumption~\ref{asp:agent-cal} holds, we have the internal regret satisfying that
    \begin{align*}
        \ir(y_{1:T},p_{1:T},\rho_{1:T})=&\max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,\rho_t,r_t),p_t, y_t) - U(r_t,p_t,y_t)) \\
        =& \frac{1}{T}\sum_{(p,\rho, r)\in \cP\times \cR\times \cR}n_{p,\rho, r}\max_{\tilde r_{p,\rho, r}}(U(\tilde r_{p,\rho, r},p, \hat \pi_{p,\rho, r}) - U(r,p,\hat \pi_{p,\rho, r}))\\
        \leq &\frac{1}{T}\sum_{(p,\rho, r)\in \cP\times \cR\times \cR}\sum_{t\in (p,\rho, r)}\max_{\tilde r_{p,\rho, r}}(U(\tilde r_{p,\rho, r},p, \pir_t) - U( r,p,\pir_t))+ 2\abs{\cP}\abs{\cR}^2\alpha\\
        =& 2\abs{\cP}\abs{\cR}^2\alpha\,.
    \end{align*}
    where $n_{p,\rho, r}=\abs{\{t|p_t = p, \rho_t = \rho, r_t = r\}} $ and $\hat \pi_{p,\rho, r} = \frac{1}{n_{p,\rho, r}}\sum_{t=1}^T y_t\ind{p_t = p, \rho_t = \rho, r_t = r}$.
\end{remark}
% the principal has a forecast $\pip_{1:T}$. At each round $t$, the principal best responds to $\pip_t$ by choosing policy 
% \begin{equation*}
%     p_t = \brp(\pip_t):= \argmax_{p\in\cP} V(\brr(p,\pip_t),p,\pip_t)\,.
% \end{equation*}
% The principal also has a guess on action taken by the agent, $\rho_t = \brr(p_t,\pip_t)$, which does not necessarily to be the true action taken by the agent.
% Suppose that $\pip_{1:T}$ is calibrated on 



% The agent does not necessarily follow $\rho_t$.
% Instead, the agent has her own forecast $\pir_{1:T}$ and she will best respond to $(p_t, \pir_t)$ by taking action $r_t = \brr(p_t, \pir_t)$. 


\begin{assumption}[agent has no secret information.]\label{asp:no-sec-info}
Let $\eneg$ be an upper bound on the negative cross-swap regret for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by the proposed mechanism and constant mechanisms.
That is,
    \begin{equation*}
        \nr(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^*_t,p^*_t,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p^*_t, \rho^{*}_t),p^*_t,y_t) \leq\eneg\,,
    \end{equation*}
    and for all $p\in \cP$,
    \begin{equation*}
        \nr(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^p_t,p,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p, \rho^{p}_t),p,y_t) \leq\eneg\,.
    \end{equation*}
    We assume that there exists a small $\eneg$.
\end{assumption}
For the proposed mechanism $\sigma^*$, let 
    $$\nr^*_{p,\rho} = \sum_{t\in (p,\rho) }U(r^*_t,p^*_t,y_t)-\max_{\tilde r}\sum_{t\in (p,\rho)}U(\tilde r,p_t,y_t)$$
    denote the negative regret for the agent for the time steps $(p^*_t,\rho^{*}_t) = (p,\rho)$.
For the constant mechanism $\sigma^p$, let
    $$\nr^{p}_{\rho} = \sum_{t\in (\rho) }U(r^p_t,p,y_t)-\max_{\tilde r}\sum_{t\in (\rho)}U(\tilde r,p,y_t)$$
    denote the negative regret for the agent for the time steps $\rho^{p}_t =  \rho$.
% Let the negative regret in $\{t|p_t = p, \rho_t =r\}$ be
% \begin{equation}
%     \nr_{p,r} := \sum_{t:p_t = p, \rho_t =r }U(r_t,p_t,y_t)-\max_{\tilde r}\sum_{t:p_t = p, \rho_t =r}U(\tilde r,p_t,y_t)\,.\label{eq:x-swap}
% \end{equation}
% Then we have $\sum_{p,r}\nr_{p,r} \leq \eneg T$ according to Assumption~\ref{asp:no-sec-info}.

A more intuitive and direct way to model ``no secret information'' is assuming that the agent cannot consistently outperforms the Principal's recommendation, i.e., 
    \begin{equation}
        \frac{1}{T}\sum_{t=1}^T U(r_t,p_t,y_t) - \frac{1}{T}\sum_{t=1}^T U(\rho_t,p_t,y_t) \leq\eneg\,.\label{eq:no-better-than-guess}
    \end{equation}
\begin{lemma}
    If the agent can't consistently outperforms the Principal's  recommendation (Eq~\eqref{eq:no-better-than-guess}), then Assumption~\ref{asp:no-sec-info} holds.
\end{lemma}

\begin{assumption}[agent's utility margin.]\label{asp:utility-margin}\todohs{relax the assumption to get rid the polynomial dependence on $\abs{\cP}\abs{\cR}$}
There exists a $\pmargin>0$ such that
for policy sequence $p_{1:T}$ and recommendation sequence $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanism , for all $(p,\rho, r)\in \cP\times \cR\times \cR$, 
either
\begin{equation*}
    n_{p,\rho, r}:=\abs{\{t|p_t = p, \rho_t = \rho, r_t = r\}} \leq \frac{1}{\pmargin^2}\,,
\end{equation*}
or
\begin{equation*}
    \abs{U(p,\bar r, \hat \pi_{p,\rho, r}) - U(p,r, \hat \pi_{p,\rho, r})}\geq \pmargin\,,
\end{equation*}
where $\hat \pi_{p,\rho, r} = \frac{1}{n_{p,\rho, r}}\sum_{t=1}^T y_t\ind{p_t = p, \rho_t = \rho, r_t = r}$.
\end{assumption}
\begin{remark}
    This assumption comes up from the distributional setting.
    In the distributional setting, there exists a prior distribution $\pi\in \Delta(\cY)$ such that $y_{1:T}\stackrel{\text{i.i.d.}}{\sim} \pi$.
    In this case, to distinguish $\rho\neq r$, we need to assume that for any $p,\rho \neq r$, $\abs{U(\rho,p,\pi) - U(r,p,\pi)} \geq 2\pmargin$.
    This would implies our Assumption~\ref{asp:utility-margin} since if $n_{p,\rho, r}>\frac{1}{\pmargin^2}$, we have $\abs{U(p,\bar r, \hat \pi_{p,\rho, r}) - U(p,r, \hat \pi_{p,\rho, r})}\geq \pmargin$ by concentration inequality.
\end{remark}
For $ r\neq \rho$, without Assumption~\ref{asp:utility-margin}, it is possible that the agent achieve the same utility by selecting either $r$ or $\rho$, which leads to different Principal's utilities.
To make an assumption on the connection between the Principal's utility and the agent utility, we can also make the following alternative assumption, which is a variant of Assumption~\ref{camara-asp:alignment}. 

Analogous to \cite{camara2020mechanisms}, we define a signal as well. Our signal is the triple of policy, recommendation and action, $I_t = (p_t,\rho_t,r_t)$.
Let $\cI$ denote the signal space.
% Let $\cI$ denote the signal space with $\abs{\cI} = \abs{\cR}$. For times steps $t$ and $\tau$, the signal $I_t=I_\tau$ implies that the agent would take the same action, i.e., $r_t = r_\tau$.
% All agent needs to do is selecting a mapping from the signal to the action.
For any prior distribution $\pi$, let $p^*(\pi)$ denote the policy deployed by the Principal when running the proposed mechanism $\sigma^*$.
In this work, $p^*(\pi) = \brp(\pi)$ is the best response. 




\begin{assumptionp}{\ref*{asp:utility-margin}$'$}[alignment]\label{asp-alt:alignment}
    For any $p\in \cP$ and any signal structure $\gamma(\cdot, y)\in \Delta(\cI)$, we say the respond $(r_I^\epsilon(p))_{I\in \cI}$ is $\epsilon$-approximately optimal iff 
    \begin{align*}
        \EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(r_J^\epsilon(p), p,y)}} \geq \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(r_J, p,y)}} -\epsilon\,.
    \end{align*}
    Let $\tilde r(p) \in \argmax_r \EEs{y\sim \pi}{U(r, p,y)}$ denote the optimal fixed respond without signal and $(\tilde r_I(p))_{I\in \cI} \in\argmax_{(r_I)_{I\in \cI}}\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(r_I, p,y)}}$ denote the optimal respond given the signal.
    We assume that there exists a constant $M_1>0$ such that for any $\epsilon$-approximately optimal responds $(r_I^\epsilon)_{I\in \cI}$,
    \begin{align}
        &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p^*(\pi)), p^*(\pi),y)}}\nonumber\\
        \leq& M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p^*(\pi)), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ) + \epsilon\,.\label{eq:alignment}
    \end{align}
    and for any fixed policy $p\in \cP$,
    \begin{align*}
        \EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p), p,y)}}-V(\tilde r(p),\tilde p, \pi)\nonumber
        \leq M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p), p,y)}} -  U(\tilde r (p), p, \pi) ) +  \epsilon\,,
    \end{align*}
\end{assumptionp}
\begin{remark}
    To parse this assumption, we can decompose Eq~\eqref{eq:alignment} into two parts. 
    First, 
    \begin{align}
        &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(\tilde r_J(p^*(\pi)), p^*(\pi),y)}}\nonumber\\
        \leq& M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p^*(\pi)), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ))\,,\label{eq:alignment-exact-opt}
    \end{align}
    and 
    \begin{equation}
        \EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(\tilde r_I(p^*(\pi)), p^*(\pi),y)}}-\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(r_I^\epsilon(p^*(\pi)), p^*(\pi),y)}}\leq \epsilon\,.\label{eq:align-approx}\,.
    \end{equation}
    Eq~\eqref{eq:alignment-exact-opt} together with Eq~\eqref{eq:align-approx} implies Eq~\eqref{eq:alignment}.
    % where $\bar r_I = \argmax_{r_I}\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(r_I, p^*(\pi),y)}}$. 
    
    Eq~\eqref{eq:alignment-exact-opt} assumes that if the agent's utility remains relatively unchanged when they optimize their action based on a given signal compared to the utility they would have obtained by selecting the best action in hindsight (i.e., without considering the signal), then the Principal's utility should also remain close. We only have one-sided inequality here as we only need this for the proof. 
    Consider an example of contract design example where the prior distribution $\pi$ is equally distributed over $\{\text{medium}, \text{hard}\}$. Shirking all the time achieves zero agent's utility  while working for medium tasks and working w.p. $(p-1)$ for hard tasks also achieves zero agent's utility.
    These two actions are indifferent to the agent.
    Eq~\eqref{eq:alignment-exact-opt} requires that the Principal's utility when the agent shirk all the time is not much worse than that when the agent work for medium tasks and $(p-1)$ for hard tasks.

    Eq~\eqref{eq:align-approx} assumes that $\epsilon$-approximation does not change the Principal's utility by much.
\end{remark}

% \begin{remark}
%     For some fixed $(p,r)$, let $\cD$ be a distribution over priors such that every $\pi\in \supp(\cD)$ satisfies that $\brr(p,\pi) = r$. Let $\supp(\gamma_\pi(y))\subset (p,r)\times \cR$.
%     Then the agent's utility gain given the information is
%     \begin{align*}
%         &\EEs{\pi\sim \cD}{\EEs{y\sim \pi}{\EEs{J\sim \gamma_\pi(\cdot, y)}{U(\tilde r_J(p,\cD), p,y)}} -  U(\tilde r(p,\cD), p, \pi)}\\
%         =& 
%     \end{align*}
% \end{remark}
% \begin{assumptionp}{\ref*{asp:utility-margin}$''$}\label{alt-asp:alignment-belief}
%     For any prior distribution $\pi$, the agent might have a different belief of the nature, i.e., a latent variable $z\sim \cD$ and then $y\sim \pi_z$. 
%     We assume that there exists a constant $M_1>0$ such that
%     \begin{align}
%         &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{V(r_z^\epsilon, p^*(\pi),y)}}\nonumber\\
%         \leq& M_1 (\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{U( \brr(p^*(\pi),\pi_z), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ) + \epsilon\,,
%     \end{align}
%     where $r_z^\epsilon$ is an $\epsilon$-approximate best respond to $(p^*(\pi),\pi_z)$.
%     For any fixed policy $p\in \cP$
%     \begin{align*}
%         &\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{V(r_z^\epsilon(p), p,y)}}-\max_{\tilde p}V(\tilde r(\tilde p),\tilde p, \pi)\nonumber\\
%         \leq& M_1 (\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{U(\brr(p,\pi_z), p,y)}} - U(\tilde r(p), p, \pi) ) +  \epsilon\,,
%     \end{align*}
%     where $r_z^\epsilon(p)$ is an $\epsilon$-approximate best respond to $(p,\pi_z)$.
% \end{assumptionp}
\begin{theorem}
    Under Assumptions~\ref{asp:principal-cal},\ref{asp:agent-cal},\ref{asp:no-sec-info}, and \ref{asp:utility-margin},  the Principal's regret satisfies that 
    \begin{equation*}
        \textrm{PR}(y_{1:T}) \leq \cO(\frac{\abs{\cP}\abs{\cR}^2 }{\pmargin^2}\alpha + \frac{\abs{\cP}\abs{\cR}^2 }{\pmargin^3T}+\frac{\epsilon}{\pmargin}).
    \end{equation*}
\end{theorem}
The proof of the theorem follows immediately by combining Lemma~\ref{lmm:regret-follow-recommendation} and the following lemma.
\begin{lemma}[the disagreement region is small.]\label{lmm:disagreement}
For any realized policies $p_{1:T}$ generated by the proposed mechanism $\sigma^*$ or the constant mechanism $\sigma^p$ and any sequence of nature states $y_{1:T}$, 
under Assumption~\ref{asp:no-sec-info} and \ref{asp:utility-margin} , we have
\begin{equation*}
     \sum_{t=1}^T \ind{\rho_t\neq r_t} = \cO\left(\frac{2\calerr(\pip) +2(1+\frac{1}{\pmargin})\calerr(\pir)+ \epsilon }{\pmargin}T+ \frac{\abs{\cP}\abs{\cR}^2}{\pmargin^3}\right)\,,
\end{equation*}
where 
$\calerr(\pir) = \frac{1}{T}\sum_{(p,\rho, r)}\norm{\sum_{t\in (p,\rho, r)} y_t - \pir_t}_1$ \\
and $\calerr(\pip) = \max\left(\sum_{p,r} \calerr(\pip,S_{p,r}), \max_{p}\sum_{r}\calerr(\pip,S'_{p,r})\right)$.
Here $t\in (p,\rho, r)$ represents that $t\in \{\tau\in [T]: p_\tau = p, \rho_\tau = r, r_\tau = \bar r\}$ and $t\in (p,r)$ represents that $t\in \{\tau\in [T]: p_\tau = p, \rho_\tau = r\}$.
\end{lemma}
\begin{proof}
% For any variable $x_{1:T}$, let $\sum_{t\in (p,r,\bar r)}x_t$ to denote $\sum_{t=1}^T \ind{(p_t,\rho_t,r_t)=(p,r,\bar r)} x_t$ and $\sum_{t\in (p,r)}x_t$ to denote $\sum_{t=1}^T \ind{(p_t,\rho_t)=(p,r)} x_t$.
Let $\hat \pi_{p,r,\bar r} = \frac{1}{n_{p,r,\bar r}} \sum_{t\in (p,r,\bar r)}y_t$ and $\pir_{p,r,\bar r} = \frac{1}{n_{p,r,\bar r}} \sum_{t\in (p,r,\bar r)}\pir_t$.
Let us define $\hat \pi_{p,r}, \pir_{p,r}$ and $\pip_{p,r}$ similarly.
Let $\calerr(\pir, p,r,\bar r) = \frac{1}{T}\norm{\sum_{t\in (p,r,\bar r)} (y_t - \pir_t)}_1 = \frac{n_{p,r,\bar r}}{T}\norm{ \hat \pi_{p,r,\bar r}-\pir_{p,r,\bar r} }_1$.

We can show that 
% \begin{align*}
%     \sum_{t=1}^T U(r_t,p_t,y_t) &= \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} \sum_{t\in (p,r,\bar r)} U(\bar r,p,y_t) \\
%     &= \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} n_{p,r,\bar r} \inner{U(\bar r,p,\cdot )}{\hat \pi_{p,r,\bar r}}\tag{linearity}\\
%     &\leq \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} n_{p,r,\bar r} \left (\inner{U(\bar r,p,\cdot )}{\pi_{p,r,\bar r}} + T\cdot\calerr(\pir, p,r,\bar r)\right)\tag{{calibration}}\\
%     &= \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} \sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\bar r,p,y)} + T\cdot\calerr(\pir)T\\
%     &=\sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} \max _{\tilde r\in \cR}\sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\tilde r,p,y)} + T\cdot\calerr(\pir)T\,. \tag{{best respond}}
% \end{align*}
\begin{align}
    \sum_{t\in (p,r,\bar r)}U(\bar r,p,y_t)=&  n_{p,r,\bar r} \inner{U(\bar r,p,\cdot )}{\hat \pi_{p,r,\bar r}}\tag{linearity}\nonumber\\
    \geq&  n_{p,r,\bar r} \inner{U(\bar r,p,\cdot )}{\pi_{p,r,\bar r}} - T\cdot\calerr(\pir, p,r,\bar r)\tag{{calibration}}\nonumber\\
    % &=  \sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\bar r,p,y)} + n_{p,r,\bar r}T\cdot\calerr(\pir, p,r,\bar r)\\
    =&\max _{\tilde r\in \cR}\sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\tilde r,p,y)} -  T\cdot\calerr(\pir, p,r,\bar r) \tag{{best response}}\nonumber\\
    \geq& \sum_{t\in (p,r,\bar r)} \inner{U( r,p,\cdot)}{\pi_{p,r,\bar r}} - T\cdot\calerr(\pir, p,r,\bar r)\nonumber\\
    \geq& n_{p,r,\bar r}U( r,p,\hat \pi_{p,r,\bar r}) -  2T\cdot\calerr(\pir, p,r,\bar r)\,,\label{eq:no-swap}
\end{align}
where the last inequality applies calibration.
On the other hand, we have that 
\begin{align}
    \sum_{\bar r\in \cR}n_{p,r,\bar r}U( \bar r,p,\hat \pi_{p,r,\bar r})&=\sum_{t\in (p,r)} U(r_t,p_t,y_t)
    =\max_{\tilde r}\sum_{t\in (p,r)} U(\tilde r,p,y_t) + \nr_{p,r}\tag{Def of $\nr_{p,r}$ in Eq~\eqref{eq:x-swap}}\nonumber\\
    &=\max_{\tilde r}n_{p,r} U(\tilde r,p,\hat \pi_{p,r}) + \nr_{p,r}\nonumber\\
    &\leq \max_{\tilde r}n_{p,r} U(\tilde r,p,\pip_{p,r}) +T\cdot\calerr(\pip,p,r)+ \nr_{p,r}\tag{calibration}\nonumber\\
    &= \max_{\tilde r}\sum_{t\in (p,r)} U(\tilde r,p,\pip_t) +T\cdot\calerr(\pip,p,r)+ \nr_{p,r}\tag{linearity}\nonumber\\
    &= \sum_{t\in (p,r)} U(r,p,\pip_t) +T\cdot\calerr(\pip,p,r)+ \nr_{p,r}\tag{best response}\nonumber\\
    &\leq \sum_{t\in (p,r)}U(r,p,y_t) + 2T\cdot\calerr(\pip,p,r) + \nr_{p,r}\tag{calibration}\nonumber\\
     &= \sum_{\bar r\in \cR}n_{p,r,\bar r}U(r,p,\hat \pi_{p,r,\bar r}) + 2T\cdot\calerr(\pip,p,r) + \nr_{p,r}\label{eq:nonneg-xswap}
\end{align}
According to Assumption~\ref{asp:utility-margin}, for all $(p,r,\bar r)$, either $n_{p,r,\bar r}\leq \frac{1}{\pmargin^2}$ or $\abs{U(p,\bar r, \hat \pi_{p,r,\bar r}) - U(p,r, \hat \pi_{p,r,\bar r})}\geq \pmargin$.
There are three cases:
\begin{itemize}
    \item Case 0: $n_{p,r,\bar r}\leq \frac{1}{\pmargin^2}$.
    \item Case 1: $U(p,\bar r,\hat \pi_{p,r,\bar r}) - U(p,r,\hat \pi_{p,r,\bar r}) \leq -\pmargin$. According to Eq~\eqref{eq:no-swap}, we have
    \begin{equation*}
        n_{p,r,\bar r}\pmargin \leq 2T\cdot\calerr(\pir,p,r,\bar r)\,,
    \end{equation*}
    which implies that $ n_{p,r,\bar r} \leq \frac{2T\cdot\calerr(\pir,p,r,\bar r)}{\pmargin}$.
    \item Case 2: $U(p,\bar r,\hat \pi_{p,r,\bar r}) - U(p,r,\hat \pi_{p,r,\bar r}) \geq \pmargin$, then according to Eq~\eqref{eq:nonneg-xswap}, we have
    \begin{align*}
        &-\sum_{\bar r\in \cR}\ind{\text{case 2}}n_{p,r,\bar r}\pmargin + 2T\cdot\calerr(\pip,p,r) + \nr_{p,r}\\
        \geq& -\sum_{\bar r\in \cR}(\ind{\text{case 1}}+\ind{\text{case 0}})n_{p,r,\bar r}U( r,p,\hat \pi_{p,r,\bar r})\\
        \geq &-\sum_{\bar r\in \cR}\frac{2T\cdot\calerr(\pir,p,r,\bar r)}{\pmargin} - \frac{\abs{\cR}}{\pmargin^2}\,.
    \end{align*}
    Hence we have
    \begin{align*}
        \sum_{\bar r\in \cR}\ind{\text{case 2}}n_{p,r,\bar r} &\leq \frac{2T\cdot\calerr(\pip,p,r) + \nr_{p,r}+\sum_{\bar r\in \cR}\frac{2T\cdot\calerr(\pir,p,r,\bar r)}{\pmargin} +\frac{\abs{\cR}}{\pmargin^2}}{\pmargin}
    \end{align*}
\end{itemize}
By combining all three cases, we have
\begin{equation*}
    \sum_{p,r}\sum_{\bar r\neq r }n_{p,r,\bar r}\leq \frac{2\calerr(\pip) +2\calerr(\pir)+ \epsilon  + \frac{2\cdot\calerr(\pir)}{\pmargin} }{\pmargin}T+ \frac{\abs{\cP}\abs{\cR}^2}{\pmargin^3}+ \frac{2\cdot\calerr(\pir)}{\pmargin} T+\frac{\abs{\cP}\abs{\cR}^2}{\pmargin^2}\,.
\end{equation*}
\end{proof}
\begin{lemma}[the Principal's utility difference is small]\label{lmm:utility-difference}
    For any sequence of nature states $y_{1:T}$, under Assumption~\ref{asp:no-sec-info} and \ref{asp-alt:alignment} , we have
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^*,p_t^*,y_t)\geq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t^*,y_t)-(M_1+1)T\eint-M_1T\eneg -(4M_1+2)\calerr(\pip)
\end{equation*}
and for all $p\in \cP$
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^p,p,y_t)\leq \frac{1}{T}\sum_{t=1}^T V(\rho^{p}_t,p,y_t)+2\calerr(\pip) +  (M_1+1)T\eint + M_1T \eneg
\end{equation*}
\end{lemma}
\begin{proof}
    
    
    
    \textbf{Proof of the first part.} 
    For each $(p,r)\in \cP\times \cR$, let the signal be the true action taken by the agent, i.e., $I_t = r_t^*$. Let the signal structure $\hat\gamma_{p,r}(\bar r, y) := \frac{\sum_{t\in (p,r)} \ind{I_t = \bar r, y_t = y}}{\sum_{t\in (p,r)} \ind{y_t = y}}$.
    \begin{align}
      \sum_{t=1}^TV(r^*_t,p^*_t,y_t) =& \sum_{(p,r)\in \cP\times \cR} \sum_{\bar r\in \cR} n_{p,r,\bar r}\sum_{t\in (p,r,\bar r)} V(\bar r, p, y_t)\nonumber\\
        = & \sum_{(p,r)\in \cP\times \cR}n_{p,r} \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
        \geq & \sum_{(p,r)\in \cP\times \cR}n_{p,r} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}} - \calerr(\pip,p,r)\label{eq:int-step-cal}\,.
    \end{align}
    Now we want to apply Eq~\eqref{eq:alignment} to lower bound Eq~\eqref{eq:int-step-cal}. The reason to apply calibration in Eq~\eqref{eq:int-step-cal} is that $p = \brp(\pip_{p,r})$ and $p\neq \brp(\hat \pi_{p,r})$ and Eq~\eqref{eq:alignment} only works for $(p,\pi)$ satisfying that $p = \brp(\pi)$.
    \begin{align}
        &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} \geq \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} -\norm{\pip_{p,r} - \hat \pi_{p,r}}_1\nonumber\\
        =& \max_{r_I} \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^*_{p,r} -\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\nonumber\\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^*_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1 \,. \label{eq:step1}
    \end{align}
    On the other hand, we have
    \begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} - \max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)} \nonumber\\
    \leq& \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} - \max_{\tilde r}\EEs{y\sim \hat \pi_{p,r}}{U(\tilde r,p,y)}+ 2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\nonumber\\
    =& \frac{1}{n_{p,r}}\nr_{p,r}+2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\,.\label{eq:step2}
    \end{align}
Combine Eq~\eqref{eq:step1} and \eqref{eq:step2}, we have
\begin{align}
    &\max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)}\nonumber\\
    \leq&  \frac{1}{n_{p,r}}\nr^*_{p,r}+\frac{1}{n_{p,r}}\ir^*_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\label{eq:setp-utility-gap}
\end{align}
According to Assumption~\ref{asp-alt:alignment}, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \geq& V(r,p,\pip_{p,r})-M_1(\frac{1}{n_{p,r}}\ir^*_{p,r}+\frac{1}{n_{p,r}}\nr^*_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) - \frac{1}{n_{p,r}}\ir^*_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\,.
\end{align*}
Hence, we have
\begin{align*}
&\sum_{t=1}^TV(r^*_t,p^*_t,y_t) \\
    \geq & \sum_{(p,r)\in \cP\times \cR} n_{p,r}V(r,p,\pip_{p,r})-(M_1+1)\ir^*_{p,r}-M_1\nr^*_{p,r} -(4M_1+2)\calerr(\pip,p,r)\\
    =& \sum_{t=1}^TV(\rho^{*}_t,p^*_t,y_t) -(M_1+1)T\eint-M_1T\eneg -(4M_1+2)\calerr(\pip)\,.
\end{align*}
\textbf{Proof of the second part under Assumption~\ref{asp-alt:alignment}.} 
Similarly, for any fixed mechanism $\sigma^p$, let the signal be the true action taken by the agent, i.e., $I_t = r_t^p$. Let the signal structure $\hat\gamma_{p,r}(\bar r, y) := \frac{\sum_{t\in (p,r)} \ind{I_t = \bar r, y_t = y}}{\sum_{t\in (p,r)} \ind{y_t = y}}$.
Similar to Eq~\eqref{eq:step1} and Eq~\eqref{eq:setp-utility-gap}, we also have
\begin{align*}
        &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} \\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^p_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M_1(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat \pi_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M_1(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M_1+1)T\eint + M_1T \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\textbf{Proof of the second part under Assumption~\ref{asp-alt-ver2:alignment}.} \todohs{not finished}
Let $\cD$ be the empirical distribution of $\pip_t$ for $t\in (p,r)$.
Let the signal structure $\hat\gamma_\pi((p,r,\bar r), y) := \frac{\sum_{t:\pip_t=\pi} \ind{I_t = \bar r, y_t = y}}{\sum_{t:\pip_t=\pi} \ind{y_t = y}}$ and $\hat\gamma_{p,r}((p,r,\bar r), y) := \frac{\sum_{t\in (p,r)} \ind{I_t = \bar r, y_t = y}}{\sum_{t\in (p,r)} \ind{y_t = y}}$.
Then we have
\begin{align*}
        &\EEs{\pi\sim \cD, y\sim \pi}{\EEs{J\sim \hat \gamma_{\pi}(\cdot,y)}{U(\bar r,p,y)}}= \frac{1}{n_{p,r}}\sum_{\bar r\in \cR} n_{p,r,\bar r} U(\bar r,p,\pip_{p,r,\bar r})\\
        \geq & \frac{1}{n_{p,r}}\sum_{\bar r\in \cR} n_{p,r,\bar r} U(\bar r,p,\hat \pi_{p,r,\bar r})-\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\\
        \geq & \frac{1}{n_{p,r}}\sum_{\bar r\in \cR} n_{p,r,\bar r} U(\bar r,p,\hat \pi_{p,r,\bar r})-\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^p_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M_1(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat \pi_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M_1(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M_1+1)T\eint + M_1T \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\end{proof}





\paragraph{Discussion on assumptions} Assumptions~\ref{asp:agent-cal} and \ref{asp:no-sec-info} are designed to restrict the behavior of the agent. Here we briefly discuss why these two assumptions are necessary in the following example. Consider an example of contract design where the contract space $\cP =\{1.5,1.6\}$, the action space of the agent/worker is $\{\text{work}, \text{shirk}\}$, and the nature state space is $\{\text{medium}, \text{hard}\}$. When the job is medium, working leads to success while shirking leads to failure; when the job is hard, both working and shirking lead to failure. The value of a job is $2$ and the cost of working is $1$. Suppose that the nature state $y_t = \text{medium}$ for odd $t$ and $y_t = \text{hard}$ for even $t$.
There are two candidate forecasts: 1) perfect forecast with $\pi_t = y_t$ for all $t$ and 2) mediocre forecast with $\pi_t = (0.5,0.5)$ for all $t$.
\begin{itemize}
    \item Is it enough to have agent's forecast be calibrated on $(p_t,\rho_t,r_t)$ instead of $(p_t,r_t)$? We can show a negative result if the agent is only calibrated on $(p_t,r_t)$.  Suppose that the Principal has a perfect forecast $\pip_t = y_t$ and then $p_t = 1.5$ for all $t$. 
    When the agent only has a mediocre forecast $\pir_t = (0.5,0.5)$ and then the agent will respond by $r_t = \text{shirk}$; when the agent also has the perfect forecast $\pir_t = y_t$, the agent will respond by $\text{work}$ iff. $y_t = \text{medium}$. 
    Both forecasts are calibrated on $(p_t,r_t)$.
    The Principal's regret will not vanish if the agent adopts the mediocre forecast for the proposed mechanism while adopts the perfect forecast for the constant mechanism of $1.6$.

    \item Why does the agent have to satisfy lower bounded cross-swap regret?
    Suppose that the Principal's forecast is the mediocre one while the agent's forecast can be mediocre or perfect. The agent can adopt the mediocre forecast for the proposed mechanism while adopts the perfect forecast for the constant mechanism.
\end{itemize}
\subsection{A set of alternative assumptions}
In this section, we propose a set of alternative assumptions to match the assumptions in \cite{camara2020mechanisms}.
The main difference in this subsection from the previous one is that the context is $(p_t,\rho_t,p^*_t,\rho^*_t, r_t)$ instead of $(p_t,\rho_t, r_t)$.  


\begin{assumptionp}{\ref*{asp:principal-cal}$'$}[finer calibration of Principal's forecast]\label{asp-alt:Principal-cal}
For any sequence of nature states $y_{1:T}$, assume that for both the proposed mechanism $\sigma^*$ and the fixed constant mechanisms $\{\sigma^p\}_{p\in \cP}$, the principle's forecast $\pip_{1:T}$ is calibrated conditional on $\pip_t\in S$ for all $S\in E'$, where $E = \{S_{p,r}|(p,r)\in \cP\times \cR\} \cup \{S''_{p,r,p',r'}|(p,r,p',r')\in \cP\times \cR\times \cP\times \cR\}$ where
\begin{equation*}
    S_{p,r} : = \{\pi| \brp(\pi) = p , \brr(p,\pi) =r\}\,,
\end{equation*}
and 
\begin{equation*}
    S''_{p,r,p',r'} : = \{\pi|\brp(\pi) = p' , \brr(p',\pi) =r',\brr(p,\pi) =r\}\,.
\end{equation*}
More specifically, there exists a small $\alpha>0$ such that for any $S\in E$,
\begin{equation*}
    \frac{1}{T} \norm{\sum_{t=1}^T \ind{\pip_t \in S} (\pip_t -y_t)}_1 \leq \alpha.
\end{equation*}
\end{assumptionp}

\begin{assumptionp}{\ref*{asp:agent-cal}$''$}[no finer counterfactual internal regret for agent]\label{asp-alt:no-finer-internal-reg}
Let $\eint$ be an upper bound on the internal regret with context of $(p_t,\rho_t, p^*_t, \rho^*_t, r_t)$ for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanisms.
\end{assumptionp}

% \begin{assumption}[agent has no secret information.]\label{asp:no-sec-info}
% Let $\eneg$ be an upper bound on the negative cross-swap regret for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by the proposed mechanism and constant mechanisms.
% That is,
%     \begin{equation*}
%         \nr(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^*_t,p^*_t,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p^*_t, \rho^{*}_t),p^*_t,y_t) \leq\eneg\,,
%     \end{equation*}
%     and for all $p\in \cP$,
%     \begin{equation*}
%         \nr(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^p_t,p,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p, \rho^{p}_t),p,y_t) \leq\eneg\,.
%     \end{equation*}
%     We assume that there exists a small $\eneg$.
% \end{assumption}

\begin{assumptionp}{\ref*{asp:utility-margin}$''$}[alignment]\label{asp-alt-ver2:alignment}\todohs{not finished}
    We assume that there exists a constant $M_1>0$ such that for any $\epsilon$-approximately optimal responds $(r_I^\epsilon)_{I\in \cI}$,
    \begin{align}
        &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p^*(\pi)), p^*(\pi),y)}}\nonumber\\
        \leq& M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p^*(\pi)), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ) + \epsilon\,.\label{eq:alignment}
    \end{align}
    and for any fixed policy $p\in \cP$,
    \begin{align*}
        \EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p), p,y)}}-\max_{p'\in \cP}V(\tilde r(p'),p', \pi)\nonumber
        \leq M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p), p,y)}} -  U(\tilde r (p), p, \pi) ) +  \epsilon\,,
    \end{align*}
\end{assumptionp}
\begin{theorem}
    Under Assumptions~\ref{asp-alt:principal-cal}, \ref{asp-alt:no-finer-internal-reg},\ref{asp:no-sec-info},\ref{asp-alt-ver2:alignment}, the principal achieves no regret.
\end{theorem}
\begin{proof}
    To prove the theorem, we will prove that
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^*,p_t^*,y_t)\geq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t^*,y_t)-(M_1+1)T\eint-M_1T\eneg -(4M_1+2)\calerr(\pip)\,,
\end{equation*}
and for all $p\in \cP$
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^p,p,y_t)\leq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t^*,y_t) +  (M_1+1)T\eint + M_1T \eneg\,.
\end{equation*}
The first part has been proved in Lemma~\ref{lmm:utility-difference}. We only need to prove the second part.
For any constant mechanism $\sigma^p$, now we consider the subsequence in which $\brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$. 
Let $t\in (p,\rho,p',\rho')$ to present $t: \brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$.
In this subsequence, we let the signal structure be $\hat\gamma_{p,\rho,p',\rho'}((p,\rho,r), y) := \frac{\sum_{t\in (p,\rho,p',\rho')} \ind{r^p_t = r, y_t = y}}{\sum_{t\in (p,\rho,p',\rho')} \ind{y_t = y}}$.
Then we have
\begin{align*}
        &\EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}} \\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} -2\norm{\pip_{p,\rho,p',\rho'}  - \hat \pi_{p,\rho,p',\rho'}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,\rho,p',\rho'}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,\rho,p',\rho'}}\nr^p_{p,\rho,p',\rho'}+\frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} +4\norm{\pip_{p,\rho,p',\rho'}  -\hat \pi_{p,\rho,p',\rho'}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt-ver2:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M_1(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat \pi_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M_1(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M_1+1)T\eint + M_1T \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\end{proof}


==> clean-label/section/0_abstract.tex <==
%!TEX root = ../main.tex
\begin{abstract}%
    We study the problem of robust learning under clean-label data-poisoning attacks, where the attacker injects (an arbitrary set of) \emph{correctly-labeled} examples to the training set to fool the algorithm into making mistakes on \emph{specific} test instances at test time. The learning goal is to minimize the attackable rate (the probability mass of attackable test instances), which is more difficult than optimal PAC learning. As we show, any robust algorithm with diminishing attackable rate can achieve the optimal dependence on $\epsilon$ in its PAC sample complexity, i.e., $O(1/\epsilon)$. On the other hand, the attackable rate might be large even for some optimal PAC learners, e.g., SVM for linear classifiers. Furthermore, we show that the class of linear hypotheses is not robustly learnable when the data distribution has zero margin and is robustly learnable in the case of positive margin but requires sample complexity exponential in the dimension. For a general hypothesis class with bounded VC dimension, if the attacker is limited to add at most $t>0$ poison examples, the optimal robust learning sample complexity grows almost linearly with $t$.
    \end{abstract}
    
    \begin{keywords}%
      adversarial machine learning, data poisoning, clean-label attack, PAC learning, sample complexity.
    \end{keywords}

==> clean-label/section/7_acknowledgements.tex <==
%!TEX root = ../main.tex
\acks{This work was supported in part by the National Science Foundation under grant CCF-1815011 and by the Defense Advanced Research Projects Agency under cooperative agreement HR00112020003. Jian Qian acknowledges support of the ONR through grant
\# N00014-20-1-2336. The views expressed in this work do not necessarily reflect the position or the policy of the Government and no official endorsement should be inferred. Approved for public release; distribution is unlimited.}

==> data-augmentation/section/0_abstract.tex <==
%!TEX root = ../main.tex
\begin{abstract}
Transformation invariances are present in many real-world problems.
For example, image classification is usually invariant to rotation and color transformation: a rotated car in a different color is still identified as a car.
Data augmentation, which adds the transformed data into the training set and trains a model on the augmented data, is one commonly used technique to build these invariances into the learning process.
However, it is unclear how data augmentation performs theoretically and what the optimal algorithm is in presence of transformation invariances.
In this paper, we study PAC learnability under transformation invariances in three settings according to different levels of realizability: (i) A hypothesis fits the augmented data; (ii) A hypothesis fits only the original data and the transformed data lying in the support of the data distribution; (iii) Agnostic case.
One interesting observation is that distinguishing between the original data and the transformed data is necessary to achieve optimal accuracy in setting (ii) and (iii), 
which implies that any algorithm not differentiating between the original and transformed data (including data augmentation) is not optimal.
Furthermore, this type of algorithms can even ``harm'' the accuracy.
In setting (i), although it is unnecessary to distinguish between the two data sets, data augmentation still does not perform optimally.
Due to such a difference, we propose two combinatorial measures characterizing the optimal sample complexity in setting (i) and (ii)(iii) and provide the optimal algorithms.
\end{abstract}

% \begin{keywords}%
%   transformation invariance, data augmentation, PAC learning, sample complexity
% \end{keywords}

==> data-augmentation/section/acks.tex <==
%!TEX root = ../main.tex
\section*{Acknowledgements}
This work was supported in part by the National Science Foundation under grant CCF-1815011 and by the Defense Advanced Research Projects Agency under cooperative agreement HR00112020003.
The views expressed in this work do not necessarily reflect the position or the policy of the Government and no official endorsement should be inferred. Approved for public release; distribution is unlimited.

We thank anonymous reviewers for their valuable suggestions.
HS thanks Freda Shi for discussion on the application of DA and suggestions from an applied viewpoint.

==> data-augmentation/section/app_eg_hurt.tex <==
%!TEX root = ../main.tex
\section{An example of $\dim(\cH,\cG) \gg \vcd(\cH)$}\label{app:eg-hurt}
\begin{example}
    For any $d>0$, let $\cX = \{\pm 1\}\times \{\be_i|i\in [2d]\}\subset \R^{2d+1}$, $\cH = \{x_1> 0, x_1\leq 0\}$ and $\cG = \{I_{2d+1}, I_{2d+1}-2\diag(\be_1)\}$ (i.e., the cyclic group generated by flipping the sign of $x_1$).
    It is easy to check that $\vcd(\cH) = 1$.
    Let $X = \{(1,\be_1), (1,\be_2),\ldots,(1,\be_{2d})\}$ and then the orbits generated from $X$ are $\bphi = \{\{(-1,\be_i),(1,\be_i)\}|i\in [2d]\}\}$.
    Every labeling $\bff\in \cY^{2d}$, if $\sum_{i\in [2d]}f_i$ is odd, let $\bx_\bff = ((2f_i-1,\be_i))_{i=1}^{2d}$; if $\sum_{i\in [2d]}f_i$ is even, let $\bx_f = ((1-2f_i,\be_i))_{i=1}^{2d}$.
    It is direct to check that $(\bff,\bx_\bff)\in B(\cH,\cG,\bphi)$ for all $\bff\in \cY^{2d}$.
    Then for all $i\in [2d]$, $\bff\oplus \bg=\be_i$ implies $x_{\bff,i}=x_{\bg,i}$.
    Hence, $\dim(\cH,\cG) = 2d$, where $d$ can be an arbitrary positive integer.
    According to Theorem~\ref{thm:re-mu-dim}, we have $\mu(\cH,\cG)\geq d$.
\end{example}

==> defection/src/macros.tex <==
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator{\Log}{Log}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\logloglog}{logloglog}
\DeclareMathOperator{\polyloglog}{polyloglog}

\newcommand{\bigO}{\mathcal{O}}
% \newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}
\renewcommand{\d}[1]{\ensuremath{\operatorname{d}\!{#1}}}

%\newcommand{\set}[1]{\left\{#1\right\}}
%\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}

%\newcommand{\ceil}[1]{\lceil#1\rceil}

\newcommand{\II}[1]{\mathds{1}_{\left\{#1\right\}}}
\newcommand{\I}{\mathds{1}}


%arrows
\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\longrightarrow}
\newcommand{\mt}{\mapsto}
\newcommand{\lmt}{\longmapsto}

%function
\newcommand{\func}[5]{
	\[
		\begin{array}{l|rcl}
			#1: & #2 & \longrightarrow & #3 \\
				& #4 & \longmapsto & #5 
		\end{array}
	\]
}

%distributions
\newcommand{\Bernoulli}{\mathrm{Bernoulli}}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Unif}{\mathrm{Unif}}


\newcommand{\specialcell}[2][c]{%
 \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

% \newtheorem{assumption}{Assumption}
% \newtheorem{innercustomasp}{Assumption}
% \newenvironment{customasp}[1]
%   {\renewcommand\theinnercustomasp{#1}\innercustomasp}
%   {\endinnercustomasp}
%\newtheorem{example}{Example}
% \newtheorem{conj}{Conjecture}
% \newtheorem{lm}{Lemma}
% \newtheorem{thm}{Theorem}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{claim}{Claim}
% \newtheorem{observation}{Observation}
% \newtheorem{example}{Example}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem*{remark}{Remark}
% \newtheorem{crl}{Corollary}
% \newtheorem{rmk}{Remark}
% \newtheorem{claim}{Claim}
% \newtheorem{eg}{Example}
% \newtheorem{theorem}{Theorem}
% \newtheorem{assumption}{Assumption}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{claim}{Claim}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem*{remark}{Remark}


% \newcommand{\R}{I\!\! R}
\newcommand{\R}{\mathbb{R}}
\newcommand{\realset}{\mathbb{R}}
\newcommand{\nats}{\mathbb{N}}

\newcommand{\NN}{{\mathbb N}}
\newcommand{\1}{\mathds{1}}
\newcommand{\ind}[1]{\mathds{1}[#1]}
\newcommand{\bOne}{{\bm 1}}
\newcommand{\bZero}{{\bm 0}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EEt}[1]{\mathbb{E}_t\left[#1\right]}
\newcommand{\EEs}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\EEc}[2]{\mathbb{E}\left[#1\left|#2\right.\right]}
\newcommand{\EEcc}[2]{\mathbb{E}\left[\left.#1\right|#2\right]}
\newcommand{\EEcct}[2]{\mathbb{E}_t\left[\left.#1\right|#2\right]}
\newcommand{\PP}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\PPs}[2]{\mathbb{P}_{#1}\left(#2\right)}
\newcommand{\PPt}[1]{\mathbb{P}_t\left[#1\right]}
\newcommand{\PPc}[2]{\mathbb{P}\left[#1\left|#2\right.\right]}
\newcommand{\PPcc}[2]{\mathbb{P}\left[\left.#1\right|#2\right]}
\newcommand{\PPct}[2]{\mathbb{P}_t\left[#1\left|#2\right.\right]}
\newcommand{\PPcct}[2]{\mathbb{P}_t\left[\left.#1\right|#2\right]}
\newcommand{\Cov}{\mathrm{Cov}}

%parens
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\sqpa}[1]{\left[#1\right]}
\newcommand{\ac}[1]{\left\{#1\right\}}
\newcommand{\ev}[1]{\left\{#1\right\}}
\newcommand{\card}[1]{\left|#1\right|}


\newcommand{\normtwo}[1]{\|#1\|_2}
% \newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\onenorm}[1]{\norm{#1}_1}
\newcommand{\infnorm}[1]{\norm{#1}_\infty}
\newcommand{\norminf}[1]{\infnorm{#1}}
\newcommand{\normm}[1]{\left\lVert#1\right\rVert}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\expp}[1]{\exp\left\{#1\right\}}

\newcommand{\CommaBin}{\mathbin{\raisebox{0.5ex}{,}}}
\newcommand*{\MyDef}{\mathrm{\tiny def}}
\newcommand*{\eqdefU}{\ensuremath{\mathop{\overset{\MyDef}{=}}}}% Unscaled version
%\newcommand*{\eqdef}{\mathop{\overset{\MyDef}{\resizebox{\widthof{\eqdefU}}{\heightof{=}}{=}}}}
\newcommand*{\eqdef}{\triangleq}
%\newcommand{\eqdef}{\stackrel{{\rm def}}{=}}
%\newcommand{\eqdef}{\stackrel{{\rm \tiny def}}{=}}
\newcommand{\transpose}{^\mathsf{\scriptscriptstyle T}}
\newcommand{\eqlog}{\overset{.}{=}}

%Calligraphic Shorthands
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\calL}{\cL}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\tcO}{\widetilde{\cO}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\tOO}{\wt{\OO}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\Sw}{\mathcal{S}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\T}{\cT}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\X}{\cX}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%Bolds Shorthands
\newcommand{\ba}{{\bf a}}
\newcommand{\bA}{{\bf A}}
% \newcommand{\bb}{{\bf b}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bP}{{\bf P}}
\newcommand{\br}{{\bf r}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\be}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bL}{{\bf L}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bq}{{\bf q}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bW}{{\bf W}}
\newcommand{\by}{{\bf y}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bx}{{\bf x}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bz}{{\bf z}}
\newcommand{\bZ}{{\bf Z}}

\newcommand{\eps}{\varepsilon}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}

\newcommand{\balpha}{{\boldsymbol \alpha}}
\newcommand{\talpha}{\widetilde{\alpha}}
\newcommand{\btheta}{{\boldsymbol \theta}}
\newcommand{\tTheta}{{\widetilde\Theta}}
\newcommand{\bdelta}{{\boldsymbol \delta}}
\newcommand{\bDelta}{{\boldsymbol \Delta}}
\newcommand{\blambda}{{\boldsymbol \lambda}}
\newcommand{\bLambda}{{\boldsymbol \Lambda}}
\newcommand{\bsigma}{{\boldsymbol \sigma}}
\newcommand{\bSigma}{{\boldsymbol \Sigma}}
\newcommand{\bphi}{{\boldsymbol \phi}}
\newcommand{\bmu}{{\boldsymbol \mu}}
\newcommand{\bxi}{{\boldsymbol \xi}}
\newcommand{\bpsi}{{\boldsymbol \psi}}
\newcommand{\bomega}{{\boldsymbol \omega}}
%\newcommand{\bell}{\boldsymbol \ell}

\newcommand{\nothere}[1]{}
\newcommand{\moveb}{\\ \bigskip}
\newcommand{\movebb}{\\[-0.25em]}
\newcommand{\moves}{\\ \smallskip}
\newcommand{\movess}{\\[-0.5em]}
\newcommand{\movesss}{\smallskip}

% bandits
%\newcommand{\hloss}{\hat\ell}
%\newcommand{\bloss}{\boldsymbol  \ell}
%\newcommand{\hbl}{\hat{\bloss}}
%\newcommand{\hbL}{\wh{\bL}}
%\newcommand{\wh}{\widehat}
%\newcommand{\ti}{_{t,i}}
%\newcommand{\wt}{\widetilde}

%fairness
\newcommand{\hcY}{\hat{\mathcal{Y}}}
\newcommand{\loss}[1]{\ell^{(#1)}}
\newcommand{\Loss}[1]{L^{(#1)}}
\newcommand{\hy}{\hat{y}}
\newcommand{\reg}[1]{R^{(#1)}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\vcd}{\mathrm{VCdim}}
\newcommand{\cFe}{\cF^{\epsilon}}

%robustness
\newcommand{\VS}{\mathrm{VS}}
\newcommand{\SVM}{\mathrm{SVM}}
\newcommand{\txi}{x^{(i)}}
\newcommand{\tyi}{y^{(i)}}
\newcommand{\DIS}{\mathrm{DIS}}
\newcommand{\ATK}{\mathrm{ATK}}
\newcommand{\Adv}{\mathrm{Adv}}
\newcommand{\atk}{\mathrm{atk}}
\newcommand{\adv}{\mathrm{adv}}
\newcommand{\prop}{\mathrm{prop}}
\newcommand{\trn}{\mathrm{trn}}
\newcommand{\conv}{\mathrm{Conv}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\attack}{R_{\mathrm{atk}}^{(t)}}
\newcommand{\attackone}{R_{\mathrm{atk}}^{(1)}}
\newcommand{\attackinfty}{R_{\mathrm{atk}}^{(\infty)}}
% \newcommand{\tr}{{\mathrm{tr}}}
\newcommand{\ERM}{{\mathrm{ERM}}}
\newcommand{\ER}{{\mathrm{ER}}}
\newcommand{\Proj}{{\mathrm{Proj}}}
\newcommand{\Rfl}{{\mathrm{Ref}}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\Major}{{\mathrm{Major}}}
\newcommand{\consistent}{{\mathrm{consist}}}
\newcommand{\supp}{{\mathrm{supp}}}
\newcommand{\po}{\leq_f^\cH}
\newcommand{\clsr}{\mathrm{Closure}}
\newcommand{\sph}{\Gamma}
\newcommand{\rbst}{{\mathrm{rbst}}}
\newcommand{\std}{{\mathrm{std}}}
\newcommand{\PAC}{{\mathrm{PAC}}}
% \newcommand{\Majority}{\mathrm{Majority}}
% \newcommand{\jian}[1]{\textcolor{red}{\{{\em #1}\}}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\CR}{\mathrm{CR}}
\newcommand{\vcao}{\mathrm{VC_{ao}}}
\newcommand{\vco}{\mathrm{VC_{o}}}
\newcommand{\st}{{\quad\mathrm{s.t.}\quad}}
\newcommand{\idx}{\mathrm{Idx}}
\newcommand{\rep}{\mathrm{rep}}
\newcommand{\dec}{\mathrm{dec}}
\newcommand{\tarc}{\mbox{\large$\frown$}}
\newcommand{\arc}[1]{\stackrel{\tarc}{#1}}


%mathematical operators
\newcommand{\norm}[1]{\left\lVert#1\right\rVert_2}
\newcommand\inner[2]{\left\langle #1, #2 \right\rangle}
\newcommand\ess[0]{\text{ess}}


%vectors
\renewcommand\a[0]{\boldsymbol{a}}
\renewcommand\b[0]{\boldsymbol{b}}
\renewcommand\c[0]{\boldsymbol{c}}
\renewcommand\d[0]{\boldsymbol{d}}
\newcommand\e[0]{\boldsymbol{e}}
\newcommand\f[0]{\boldsymbol{f}}
\newcommand\g[0]{\boldsymbol{g}}
\newcommand\h[0]{\boldsymbol{h}}
\renewcommand\i[0]{\boldsymbol{i}}
\renewcommand\j[0]{\boldsymbol{j}}
\renewcommand\k[0]{\boldsymbol{k}}
\renewcommand\l[0]{\boldsymbol{l}}
\newcommand\m[0]{\boldsymbol{m}}
\newcommand\n[0]{\boldsymbol{n}}
\renewcommand\o[0]{\boldsymbol{o}}
\newcommand\p[0]{\boldsymbol{p}}
\newcommand\q[0]{\boldsymbol{q}}
\renewcommand\r[0]{\boldsymbol{r}}
\newcommand\s[0]{\boldsymbol{s}}
\renewcommand\t[0]{\boldsymbol{t}}
\renewcommand\u[0]{\boldsymbol{u}}
\renewcommand\v[0]{\boldsymbol{v}}
\newcommand\w[0]{\boldsymbol{w}}
\newcommand\x[0]{\boldsymbol{x}}
\newcommand\y[0]{\boldsymbol{y}}
\newcommand\z[0]{\boldsymbol{z}}

%bold letters
\renewcommand\aa[0]{\mathbb{A}}
\newcommand\bb[0]{\mathbb{B}}
\newcommand\cc[0]{\mathbb{C}}
\newcommand\dd[0]{\mathbb{D}}
\newcommand\ee[0]{\mathbb{E}}
\newcommand\ff[0]{\mathbb{F}}
% \renewcommand\gg[0]{\mathbb{G}}
\newcommand\hh[0]{\mathbb{H}}
\newcommand\ii[0]{\mathbb{I}}
\newcommand\jj[0]{\mathbb{J}}
\newcommand\kk[0]{\mathbb{K}}
% \renewcommand\ll[0]{\mathbb{L}}
\newcommand\mm[0]{\mathbb{M}}
\newcommand\nn[0]{\mathbb{N}}
\newcommand\oo[0]{\mathbb{O}}
\newcommand\pp[0]{\mathbb{P}}
\newcommand\qq[0]{\mathbb{Q}}
\newcommand\rr[0]{\mathbb{R}}
\renewcommand\ss[0]{\mathbb{S}}
\renewcommand\tt[0]{\mathbb{T}}
\newcommand\uu[0]{\mathbb{U}}
\newcommand\vv[0]{\mathbb{V}}
\newcommand\ww[0]{\mathbb{W}}
\newcommand\xx[0]{\mathbb{X}}
\newcommand\yy[0]{\mathbb{Y}}
\newcommand\zz[0]{\mathbb{Z}}

%cursive letters
\newcommand\aaa[0]{\mathcal{A}}
\newcommand\bbb[0]{\mathcal{B}}
\newcommand\ccc[0]{\mathcal{C}}
\newcommand\ddd[0]{\mathcal{D}}
\newcommand\eee[0]{\mathcal{E}}
\newcommand\fff[0]{\mathcal{F}}
\renewcommand\ggg[0]{\mathcal{G}}
\newcommand\hhh[0]{\mathcal{H}}
\newcommand\iii[0]{\mathcal{I}}
\newcommand\jjj[0]{\mathcal{J}}
\newcommand\kkk[0]{\mathcal{K}}
\renewcommand\lll[0]{\mathcal{L}}
\newcommand\mmm[0]{\mathcal{M}}
\newcommand\nnn[0]{\mathcal{N}}
\newcommand\ooo[0]{\mathcal{O}}
\newcommand\ppp[0]{\mathcal{P}}
\newcommand\qqq[0]{\mathcal{Q}}
\newcommand\rrr[0]{\mathcal{R}}
\newcommand\sss[0]{\mathcal{S}}
\newcommand\ttt[0]{\mathcal{T}}
\newcommand\uuu[0]{\mathcal{U}}
\newcommand\vvv[0]{\mathcal{V}}
\newcommand\www[0]{\mathcal{W}}
\newcommand\xxx[0]{\mathcal{X}}
\newcommand\yyy[0]{\mathcal{Y}}
\newcommand\zzz[0]{\mathcal{Z}}

\newcommand\opt[0]{\x^\star}

%brackets
\newcommand\rb[1]{\left(#1\right)}
\renewcommand\sb[1]{\left[#1\right]}
\newcommand\cb[1]{\left\{#1\right\}}

\newcommand\Exp[0]{\mathbb{E}}

\usepackage[makeroom]{cancel}

%\usepackage[table]{xcolor}
\newcommand{\highlight}[1]{%
	\colorbox{yellow!50}{$\displaystyle#1$}}

\usepackage{lipsum}
\newcommand\NoIndent[1]{%
	\begingroup
	\par
	\parshape0
	#1\par
	\endgroup
}

%answer box
\usepackage[most]{tcolorbox}
\newcommand{\ans}[1]{
\NoIndent{\hspace{0.2in}\begin{tcolorbox}[breakable, enhanced, width=1.05\textwidth]
\textbf{Proof:} #1 \qed
\end{tcolorbox}}
}

\newcommand{\idea}[1]{
\NoIndent{\begin{tcolorbox}[breakable, enhanced, width=\textwidth]
\textbf{Future extension:} #1
\end{tcolorbox}}
}

%\newcommand{\box}[1]{
%\NoIndent{\hspace{0.2in}\begin{tcolorbox}[breakable, enhanced, width=1.05\textwidth]
%\textbf{} #1 \qed
%\end{tcolorbox}}

%matrix operations
\newcommand{\tr}[1]{\textrm{tr}\left(#1\right)}





\newcommand{\ngrad}[1]{\nabla \tilde F_{#1}}


==> defection/src/rational.tex <==
% \documentclass[tikz,border=10pt]{standalone}
% \usetikzlibrary{positioning}
% \usepackage{amssymb}
% \begin{document}
\begin{tikzpicture}[node distance=2cm]

% Central Server
\node[draw, very thick, minimum size=2cm, fill=cyan!30, align=center] (server) {\textbf{Server's objective}:\\ $\min_{w\in \mathbb{R}^d}\tilde F(w) := \mathbb{E}_{m \sim \mathcal{P}}[F_m(w)]$};

% Proxy Objective
\node[draw, very thick, minimum size=2cm, fill=orange!30, align=center, below=1cm of server] (proxy) {\textbf{Proxy objective}: Sample $[M]\sim \mathcal{P}^{\otimes M}$\\ $\min_{w\in \mathbb{R}^d}F(w) := \frac{1}{M}\sum_{m\in[M]}F_m(w)$};

% Agents
\node[draw, very thick, minimum size=2cm, below left=2cm of proxy, fill=lime!40, align=center] (agent1) {\textbf{Agent 1's objective}:\\ $ \min_{w\in \mathbb{R}^d} F_1(w):= \mathbb{E}_{z\sim \mathcal{D}_1}[f(w;z)]$};
\node[draw, very thick, minimum size=2cm, below=2cm of proxy, fill=lime!40, align=center] (agent2) {\textbf{Agent 2's objective}:\\ $ \min_{w\in \mathbb{R}^d}F_2(w):= \mathbb{E}_{z\sim \mathcal{D}_2}[f(w;z)]$};

% Curved dotted path to Agent M
\node[draw, very thick, minimum size=2cm, below right=2cm of proxy, fill=lime!40, align=center] (agentM) {\textbf{Agent $M$'s objective}:\\ $ \min_{w\in \mathbb{R}^d}F_M(w):= \mathbb{E}_{z\sim \mathcal{D}_M}[f(w;z)]$};
\draw[dotted, very thick] ([xshift=-0cm,yshift=2.5cm]agent2.south) to[bend right=45] ([xshift=-5cm,yshift=1.2cm]agentM.north);

% Connections
\draw[-] (proxy) -- (agent1);
\draw[-] (proxy) -- (agent2);
\draw[-] (proxy) -- (agentM);
\draw[-] (server) -- (proxy);

\end{tikzpicture}
% \end{document}


==> incentivized-active/src/abstract.tex <==
% \hs{TODO:
% \\
% 1. add a high-level sketch of the example in the proof of ``Greedy is not IR''. maybe also describe why OPT is IR in the same example
% \\
% 2. reduce the length of converting alg to IR/SIR. 
% \\
% 3. add a tree to illustrate the algorithmic idea, e.g., how to truncate the tree
% }


In collaborative active learning, where multiple agents try to learn labels from a common hypothesis, we introduce an innovative framework for incentivized collaboration. Here, rational agents aim to obtain labels for their data sets while keeping label complexity at a minimum. We focus on designing (strict) \emph{individually rational} (IR) collaboration protocols, ensuring that agents cannot reduce their expected label complexity by acting individually. We first show that given any optimal active learning algorithm, the collaboration protocol that runs the algorithm as is over the entire data is already IR. However, computing the optimal algorithm is NP-hard. We therefore provide collaboration protocols that achieve (strict) IR and are comparable with the best known tractable approximation algorithm in terms of label complexity. 

 

==> incentivized-active/src/ack.tex <==
\section*{Acknowledgements}
We would like to thank Avrim Blum for several useful discussions.
This work was supported in part by the National Science Foundation under grants 2212968 and 2216899, by the Simons Foundation under the Simons Collaboration on the Theory of Algorithmic Fairness, by the Defense Advanced Research Projects Agency under cooperative agreement HR00112020003. The views expressed in this work do not necessarily reflect the position or the policy of the Government and no official endorsement should be inferred. Approved for public release; distribution is unlimited.

==> multi-objective/section/0_abstract.tex <==
%!TEX root = ../main.tex
\begin{abstract}
% In classic sequential decision making  problems, policies are evaluated with respect to a scalar reward function, and all optimal policies are the same with regards to their expected return. However, many real-world problems involve balancing multiple, sometimes conflicting, objectives whose relative priority will vary according to the preferences of each user. Consequently, a policy that is optimal for one user might be  sub-optimal for another. 

In this work, we propose a multi-objective decision making framework that accommodates different user preferences over objectives, where preferences are learned via policy comparisons. Our model consists of a known Markov decision process with a vector-valued reward function, with each user having an unknown preference vector that expresses the relative importance of each objective. The goal is to efficiently compute a near-optimal policy for a given user. We consider two user feedback models. We first address the case where a user is provided with two policies and returns their preferred policy as feedback. We then move to a different user feedback model, where a user is instead provided with two small weighted sets of representative trajectories and selects the preferred one. In both cases, we suggest an algorithm that finds a nearly optimal policy for the user using a number of comparison queries that scales quasilinearly in the number of objectives.

%We then move forward to the more realistic case in which users need some demonstrations to understand the policy, and suggest an efficient algorithm that describes a policy as a small weighted trajectory set with expected value identical to that of the policy.
\end{abstract}

==> multi-objective/section/ack.tex <==
\section*{Acknowledgements}
This work was supported in part by the National Science Foundation under grants CCF-2212968 and ECCS-2216899 and by the Defense Advanced Research Projects Agency under cooperative agreement HR00112020003. The views expressed in this work do not necessarily reflect the position or the policy of the Government and no official endorsement should be inferred. Approved for public release; distribution is unlimited.

This project was supported in part by funding from the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation program (grant agreement number 882396), by the Israel Science Foundation (grant number 993/17), Tel Aviv University Center for AI and Data Science (TAD), the Eric and Wendy Schmidt Fund, and the Yandex Initiative for Machine Learning at Tel Aviv University.

We would like to thank all anonymous reviewers, especially Reviewer Gnoo, for their constructive comments.

==> multi-objective/section/app_gap-hatw-w_revised.tex <==
%!TEX root = ../main.tex
\section{Proof of Lemma~\ref{lmm:gap-hatw-w}}\label{app:gap-hatw-w}
\lmmhatww*
\begin{proof}
We introduce some notations first.
For any $x,y\in\R^k$, let $\theta(x,y)$ denotes the angle between $x$ and $y$.
For any subspace $U\subset \R^k$, let $\theta(x,U) := \min_{y\in U}\theta(x,y)$.
For any two subspaces $U,U'\subset \R^k$, $\theta(U,U') := \max_{x\in U} \min_{y\in U'}\theta(x,y)$.
For any matrix $M$, let $M_i$ denote the $i$-th row vector of $M$, $M_{i:j}$ denote the submatrix of $M$ composed of rows $i,i+1,\ldots,j$ and $M_{i:}$ denote the submatrix composed of all rows $j\geq i$.
Let $\Span(M)$ denote the span of the row vectors of $M$.
Recall that $\hat A\in \R^{d\times k}$ is defined in Eq~\eqref{eq:Ahat} as 
\begin{align*}
    \hat A = \begin{pmatrix}
    V^{\pi_1\top}\\
    (\hat \alpha_1 V^{\pi_1} -V^{\pi_2})^\top\\
    \vdots\\
    (\hat \alpha_{d-1} V^{\pi_1} -V^{\pi_d})^\top
    \end{pmatrix}\,,
\end{align*}
which is the approximation of matrix $A\in \R^{d\times k}$ defined by true values of $\alpha_i$, i.e.,
\begin{align*}
    A = \begin{pmatrix}
    V^{\pi_1\top}\\
    (\alpha_1 V^{\pi_1} -V^{\pi_2})^\top\\
    \vdots\\
    (\alpha_{d-1} V^{\pi_1} -V^{\pi_d})^\top
    \end{pmatrix}\,.
\end{align*}
Let $\hat A^{(\delta)} = \hat A_{1:d_\delta}, A^{(\delta)}=A_{1:d_\delta}\in \R^{d_\delta\times k}$ be the sub-matrix comprised of the first $d_\delta$ rows of $\hat A$ and $A$ respectively.
\lmmspanangle*

We will use the following lemma by~\cite{Balcan2015} to prove Lemma~\ref{lmm:spanangle}.
\begin{lemma}[Lemma 3 of~\cite{Balcan2015}]\label{lmm:Balcan}
Let $U_l = \Span(\xi_1,\ldots,\xi_l)$ and $\hat U_l = \Span(\hat \xi_1,\ldots,\hat \xi_l)$.
Let $\eacc, \gamma\geq 0$ and $\eacc\leq \gamma^2/(10l)$.
Assume for $i=2,\ldots, l$ that $\theta(\hat \xi_i, \hat U_{i-1})\geq \gamma$, and for $i=1,\ldots, l$, $\theta(\xi_{i}, \hat \xi_{i})\leq \eacc$. Then
$$\theta(U_l, \hat U_l)\leq 2l\frac{\eacc}{\gamma}\,.$$
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lmm:spanangle}]
For all $2\leq i \leq d_\delta$, we have that
\begin{align*}
    &\theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{2:i-1})) \geq \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})) \geq \sin( \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})))\\ \stackrel{(a)}{\geq}&\frac{\abs{\hat A^{(\delta)}_i \cdot u_i}}{\norm{\hat A^{(\delta)}_i}_2}\stackrel{(b)}{\geq}
    \frac{\delta}{\norm{\hat A^{(\delta)}_i}_2} = \frac{\delta}{\norm{\hat \alpha_{i-1} V_{1} -V_{i}}_2} \geq \frac{\delta}{(\calpha+1)\cv}
\,,
\end{align*}
where Ineq~(a) holds as $u_i$ is orthogonal to $\Span(\hat A^{(\delta)}_{1:i-1})$ according to line~\ref{alg-line:orthonormal-basis} of Algorithm~\ref{alg:policy-threshold-free} and Ineq~(b) holds due to the definition of $d_\delta$.
The last inequality holds due to $\norm{\hat \alpha_{i-1} V^{\pi_1} -V_{i}}_2 \leq \abs{\hat \alpha_{i-1}} \norm{V^{\pi_1}}_2+\norm{V_i}_2 \leq (\calpha+1)\cv$.
Similarly, we also have
\[\theta(A^{(\delta)}_i, \Span(A^{(\delta)}_{2:i-1}))\geq \frac{\delta}{(\calpha+1)\cv}\,.\]

We decompose $V_i$ in the direction of $V^{\pi_1}$ and the direction perpendicular to $V^{\pi_1}$. Denote by $v_i^\parallel = V_i\cdot \frac{V^{\pi_1}}{\norm{V^{\pi_1}}_2}$, $V_i^\parallel =v_i^\parallel \frac{V^{\pi_1}}{\norm{V^{\pi_1}}_2}$, $V_i^\perp =V_i -V_i^\parallel$ and $v_i^\perp = \norm{V_i^\perp}_2$.
Then we have 
\[\theta( A^{(\delta)}_i,\hat A^{(\delta)}_i) = \theta(\alpha_{i-1} V_{1} -V_{i},\hat\alpha_{i-1} V_{1} -V_{i})= \theta(\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp,\hat\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp)\,.\]
If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) \geq 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the same direction, then
\begin{align}
    \theta(A^{(\delta)}_i,\hat  A^{(\delta)}_i) 
    &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}-\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} }\nonumber\\
    & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} - \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\label{eq:arctan}\\
    &\leq\frac{\abs{\hat \alpha_{i-1} - \alpha_{i-1}}\norm{V^{\pi_1}}_2}{v_i^\perp}\nonumber\\
    &\leq \frac{\ealpha \cv}{\delta}\,,\label{eq:applytau}
\end{align}
where Ineq~\eqref{eq:arctan} follows from the fact that the derivative of $\arctan$ is at most 1, i.e., $\partial \arctan x/\partial x = \frac{1}{1+x^2}\leq 1$.
Ineq~\eqref{eq:applytau} holds since $v_i^\perp \geq \abs{\inner{V_i}{u_i}}\geq \delta$.

If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) < 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the opposite directions, then we have $\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2+\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2\leq \ealpha \norm{V^{\pi_1}}_2$. Similarly, we have
\begin{align*}
    \theta(\hat A^{(\delta)}_i, A^{(\delta)}_i) 
    &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}+\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} } \\
    & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} + \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\\
    &\leq\frac{\ealpha \norm{V^{\pi_1}}_2}{\abs{v_i^\perp}}\nonumber\\
    &\leq \frac{\ealpha \cv}{\delta}\,.
\end{align*}
% Now we are ready to apply Lemma~\ref{lmm:Balcan} by letting $\hat \xi_i = \hat A^{(\delta)}_{i+1}$, $\xi_i = A^{(\delta)}_{i+1}$, $\eacc = \frac{\ealpha u}{\delta}$ and $\gamma = \frac{\delta}{(\calpha+1)u}$.
By Lemma~\ref{lmm:Balcan}, we have that when 
$\delta \geq 3(\calpha+1)^{\frac{4}{3}}\cv\ealpha^\frac{1}{3}$,
\begin{equation*}
    \theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq \frac{2d_\delta(\calpha+1) \cv^2\ealpha }{\delta^2}=\eta_{\ealpha,\delta}\,,
\end{equation*}
and
\begin{equation*}
    \theta(\Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq 
\eta_{\ealpha,\delta}\,.
\end{equation*}
We are done with proof of Lemma~\ref{lmm:spanangle}.
\end{proof}
Let $b_1,\ldots,b_{d_\delta-1}$ be any orthonormal basis of $\Span(\hat A^{(\delta)}_{2:})$.
We construct a $\hat w^{(\delta)}$ s.t. $\hat A^{(\delta)}\hat w^{(\delta)} =\be_1$ by removing $w'$'s component in $\Span(\hat A^{(\delta)}_{2:})$ and rescaling.
Specifically, let 
\begin{equation}\label{eq:createwdelta}
    \hat w^{(\delta)} = \frac{ w'- \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}{1-\inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}}\,.
\end{equation}
Since $A^{(\delta)}w' = \be_1$, 
it is direct to check that $\inner{\hat A^{(\delta)}_1}{\hat w^{(\delta)}} = \inner{V^{\pi_1}}{\hat w^{(\delta)}} = 1$ and $\hat A^{(\delta)}_i \cdot \hat w^{(\delta)} = 0$ for $i=2,\ldots,d_\delta$, i.e., $\hat A^{(\delta)}\hat w^{(\delta)} =\be_1$.
Let $\gamma = \inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}$ and we show that $\gamma$ is small as follows.
Since $\theta( \Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq  \eta_{\ealpha,\delta}$, there exist unit vectors $\tilde b_1,\ldots,\tilde b_{d_\delta-1}\in \Span(A^{(\delta)}_{2:})$ such that $\theta(b_i,\tilde b_i)\leq \eta_{\ealpha,\delta}$.
Since $w'$ has zero component in $\Span(A^{(\delta)}_{2:})$, $w'$ should have a small component in $\Span(\hat A^{(\delta)}_{2:})$.
In particular,
\begin{align*}
     \abs{\inner{w'}{b_i}}= \abs{\inner{w'}{b_i-\tilde b_i}} \leq \norm{w'}_2 \eta_{\ealpha,\delta}\,,
\end{align*}
which implies that 
\begin{align*}
    \norm{\sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}_2\leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta}\,.
\end{align*}
Hence we have that $\abs{\gamma} \leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv$.
Besides, for any policy $\pi$, we also have \begin{equation*}
    \abs{\sum_{i=1}^{d_\delta-1} \inner{w'}{b_i} \inner{b_i}{V^\pi}} \leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv\,.
\end{equation*}
Hence
\begin{align}
    \abs{\inner{\hat w^{(\delta)}}{V^{\pi}} - \inner{w'}{V^{\pi}}}& \leq \abs{\inner{\hat w^{(\delta)}}{V^{\pi}} - \frac{1}{1-\gamma} \inner{w'}{V^{\pi}}} + \abs{\frac{1}{1-\gamma} \inner{w'}{V^{\pi}}- \inner{w'}{V^{\pi}}}\nonumber\\
    &\leq \frac{1}{1-\gamma}\abs{\sum_{i=1}^{d_\delta-1} \inner{w'}{b_i} \inner{b_i}{V^{\pi}}} +\frac{\gamma \norm{w'}_2 \cv}{1-\gamma}\nonumber\\
    &\leq \frac{\sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} u}{1-\gamma} + \frac{\gamma \norm{w'}_2 \cv}{1-\gamma}\nonumber\\
    & =\cO(\norm{w'}_2^2 \frac{d_\delta^{\frac{3}{2}}(\calpha+1)\cv^4\ealpha }{\delta^2})\label{eq:lmm2}
\end{align}
when $\sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv= \cO(1)$, which is true when $\epsilon$ is small enough.
\end{proof}

==> multi-objective/section/app_gap-w-w_.tex <==
%!TEX root = ../main.tex
\section{Proof of Lemma~\ref{lmm:gap-w-w'}}\label{app:gap-w-w'}
\begin{proof}
For every policy $\pi$, the value vector can be represented as a linear combination of row vectors of $A^\textrm{(full)}$, i.e.,there exists $a = (a_1,\dots,a_d)\in \R^d$ s.t. 
$$V^\pi = \sum_{i=1}^d{a_i A^\textrm{(full)}_i} = A^{\textrm{(full)}\top} a\,.$$ 
For any unit vector $\xi \in \Span(b_1,\ldots,b_{d-d_\delta})$, we have $\inner{V^\pi}{\xi} \leq \sqrt{k} \delta$.
This is because at round ${d_\delta+1}$, we pick an orthonormal basis $\rho_1,\ldots,\rho_{k-{d_\delta}}$ in line~\ref{alg-line:orthonormal-basis} of Algorithm~\ref{alg:policy-threshold-free} and pick $u_{d_\delta+1}$ to be the one in which there exists a policy with the largest component as described in line~\ref{alg-line:largest-component} of Algorithm~\ref{alg:policy-threshold-free}.
Hence, $\abs{\inner{V^\pi}{\rho_j}}\leq \delta$ for all $j\in [k-{d_\delta}]$.
Then, we have 
$\inner{V^\pi}{\xi}= \sum_{j=1}^{k-{d_\delta}} \inner{\xi}{\rho_j}\inner{V^\pi}{\rho_j} \leq \sqrt{k-d_\delta}\delta$ by Cauchy-Schwarz inequality.
Thus, we have $$\sum_{i={d_\delta+1}}^d a_i^2 = \abs{\inner{V^\pi}{\sum_{i=d_\delta+1}^d a_{i} \basis_{i-d_\delta}}} \leq \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \sqrt{k-d_\delta}\delta\,,$$
which implies that
\begin{equation}
    \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \leq \sqrt{k-d_\delta}\delta\,.\label{eq:anorm}
\end{equation}


Since $w'$ satisfies $Aw' =\be_1$, we have $$A^\textrm{(full)} w' = (1,0,\ldots,0, \inner{\basis_1}{w'},\ldots,\inner{\basis_{d-d_\delta}}{w'})\,.$$
For any $w \in \R^k$ satisfying $A^\textrm{(full)} w = \be_1$, consider $\tilde w = w +\sum_{i= 1}^{d-d_\delta}\inner{\basis_{i}}{w'} \basis_{i}$. 
Then we have $A^\textrm{(full)}\tilde w = A^\textrm{(full)}w'$.
Thus, we have
\begin{align*}
    \tilde w\cdot V^\pi =  \tilde w^\top A^{\textrm{(full)}\top}a = w'^\top A^{\textrm{(full)}\top}a = w'\cdot V^\pi\,.
\end{align*} 
Hence,
\begin{align*}
    &\abs{w\cdot V^\pi- w'\cdot V^\pi} = \abs{w\cdot V^\pi- \tilde w\cdot V^\pi} = \abs{\sum_{i=1}^d a_i (w - \tilde w)\cdot A^\textrm{(full)}_i  }\\
    =& \abs{\sum_{i=d_\delta +1}^{d} a_i \inner{\basis_{i-d_\delta}}{w'}} 
    \stackrel{(a)}{\leq}  \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \norm{w'}_2 \stackrel{(b)}{\leq} \sqrt{k-d_\delta} \delta \norm{w'}_2\,,
\end{align*}
where Eq~(a) applies Cauchy-Schwarz inequality and Eq~(b) applies Eq~\eqref{eq:anorm}.


% that 
% hold $A^\textrm{(full)}\tilde w =(e_1,\beta)$, we have
% \begin{align*}
%     \tilde w\cdot V =  \sum_{i=1}^d{a_i \tilde w \cdot A^\textrm{(full)}_i} = a_1 +\sum_{i=1}^{d-d_\delta} a_{d_\delta+i} \beta_i =\sum_{i=1}^d{a_i w' \cdot A^\textrm{(full)}_i}= w'\cdot V\,.
% \end{align*} 
% According to the definition of $d_\delta$, $\inner{V^\pi}{u_i} $
% For every value vector $V = \sum_{i=1}^d a_i A^\textrm{(full)}_i$, $V$'s component in $\Span(B)$ is upper bounded by $\sqrt{k-d_\delta}\delta$ due to the definition of the procedure (where there exists a basis of $\Span(\mathcal{V})^\perp$ such that no policy has $\geq \delta$ component in the direction of each basis vector). \lc{LC: The way it is written now implies that the rows in $B$ could be \textit{any} basis, we should change it so this will be correct.]}
% Then we have

% where the one before last inequality follows from Cauchy-Schwarz. Finally, since $w'$  holds $A^\mathrm{(full)}\tilde w = (e_1,\beta)$, it follows from the above that for every value vector $V$ we have $$\abs{w\cdot V- w'\cdot V} \leq \sqrt{k-d_\delta} \delta \norm{\beta}_2\,.$$


% Let $b_i=A^\mathrm{(full)}_{d_\delta +i}$ denote the $i$-th row of $B$.
% Then, for all $w$ satisfying $ A^{(\delta)} w = e_1$, we can construct a $\tilde w = w +\sum_{i=1}^{d-d_\delta}\beta_i b_i$ satisfying $A^\mathrm{(full)}\tilde w = (e_1,\beta)$.
% Thus, we have
% \lc{[LC: I'm missing the definition of $b_i$ in the following equation.  If there are the rows of the matrix $b$ from the pink part then we should store these in $B$ because currently $B$ is not necessarily the same as in the pink part. If it is any basis for $B$ then it's not clear to me why the one before last inequality holds. Also, if they are not related, it is confusing to have $b_1,...,$ as the members of an  arbitrary basis for $\Span(\mathcal V)^\perp$ at each step of the procedure.]}
% \hsedit{[HS:  $B$ is defined as an arbitrary othonormal basis of $\Span(\text{all policies})\setminus \Span(\mathcal V)$. It is unrelated to the pink part. It is unrelated to ``$b_1,...,$ as the members of an  arbitrary basis for $\Span(\mathcal V)^\perp$ at each step of the procedure'' either (I just changed the notations of this basis to $u_1, u_2,\ldots$ to avoid confusion). 
% (Sorry for abusing the notation)
% The second last inequality holds because $\sum_{i=d'+1}^d\abs{a_i} \abs{b_i\cdot (w-\tilde w)} \leq \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \sqrt{\sum_{i={d_\delta+1}}^d (b_i\cdot (w-\tilde w))^2}$ and $\sqrt{\sum_{i={d_\delta+1}}^d (b_i\cdot (w-\tilde w))^2}\leq  \norm{w-\tilde w}_2$ due to that $b_i$s are othonormal.] }


% for any $w\lc{\in \R^k}$ satisfying $Aw =\lc{c_1} e_1$we can construct a 
%  $\tilde w = w +\sum_{i=1}^{d-d'}\beta_i b_i$ satisfying $A'\tilde w = (e_1,\beta)$.
% Thus \lc{for every value vector $V$} we have $$\abs{w\cdot V- w'\cdot V}=\abs{w\cdot V- \tilde w\cdot V} \leq \sqrt{k-d'} \delta \norm{\beta}_2\,.$$
\end{proof}
% \begin{proof}
% Given the output $(V_1,\ldots,V_d)$ and $(u_1,\ldots,u_d)$ of Algorithm~\ref{alg:policy-threshold-free}, let $A^\textrm{(full)}\in \R^{d\times k}$ be the matrix of replacing the last $d-d_\delta$ rows of $A$ with $u_{d_\delta+1},\ldots,u_d$, i.e.,
% \begin{equation*}
%     A^\textrm{(full)} = \begin{pmatrix}
%     V^{\pi_1\top}\\
%     (\alpha_1 V^{\pi_1} -V^{\pi_2})^\top\\
%     \vdots\\
%     (\alpha_{d_\delta-1} V^{\pi_1} -V^{\pi_{d_\delta}})^\top\\
%     u_{d_\delta +1}^\top\\
%     \vdots\\
%     u_{d}^\top
%     \end{pmatrix}\,.
% \end{equation*}
% % Let $B\in \R^{(d-d_\delta)\times k}$ denote the matrix with the $i$-th row being $u_{d_\delta +i}^\top$.
% We have $\rank(A^\textrm{(full)})$

% According to the algorithm, we have $\Span(A^\textrm{(full)}) = \Span(\cV)$.
% For every policy $\pi$, the value vector can be represented as a linear combination of row vectors of $A^\textrm{(full)}$, i.e.,there exist $a = (a_1,\dots,a_d)\in \R^d$ s.t. 
% $$V^\pi = \sum_{i=1}^d{a_i A^\textrm{(full)}_i} = A^{\textrm{(full)}\top} a\,.$$ 
% For any unit vector $\xi \in \Span(u_{d_\delta+1},\ldots,u_d)$, we have $\inner{V^\pi}{\xi} \leq \sqrt{k} \delta$.
% This is because at round ${d_\delta+1}$, we pick an orthonormal basis $\rho_1,\ldots,\rho_{k-{d_\delta}}$ in line 3 of Algorithm~\ref{alg:policy-threshold-free} and pick $u_{d_\delta+1}$ to be the one in which there exists a policy with the largest component as described in line 4 of Algorithm~\ref{alg:policy-threshold-free}.
% Hence, $\abs{\inner{V^\pi}{\rho_j}}\leq \delta$ for all $j\in [k-{d_\delta}]$.
% Then, we have 
% $\inner{V^\pi}{\xi}= \sum_{j=1}^{k-{d_\delta}} \inner{\xi}{\rho_j}\inner{V^\pi}{\rho_j} \leq \sqrt{k-d_\delta}\delta$ by Cauchy-Schwarz inequality.
% Thus, we have $$\sum_{i={d_\delta+1}}^d a_i^2 = \abs{\inner{V^\pi}{\sum_{i=d_\delta+1}^d a_i u_i}} \leq \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \sqrt{k-d_\delta}\delta\,,$$
% which implies that
% \begin{equation}
%     \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \leq \sqrt{k-d_\delta}\delta\,.\label{eq:anorm}
% \end{equation}


% Since $w'$ satisfies $Aw' =\be_1$, we have $$A^\textrm{(full)} w' = (1,0,\ldots,0, \inner{u_{d_\delta +1}}{w'},\ldots,\inner{u_{d}}{w'})\,.$$
% Considering $\tilde w = w +\sum_{i=d_\delta + 1}^{d}\inner{u_i}{w'} u_i$, we have $A^\textrm{(full)}\tilde w = A^\textrm{(full)}w'$.
% Thus, we have
% \begin{align*}
%     \tilde w\cdot V^\pi =  \tilde w^\top A^{\textrm{(full)}\top}a = w'^\top A^{\textrm{(full)}\top}a = w'\cdot V^\pi\,.
% \end{align*} 
% Hence,
% \begin{align*}
%     &\abs{w\cdot V^\pi- w'\cdot V^\pi} = \abs{w\cdot V^\pi- \tilde w\cdot V^\pi} = \abs{\sum_{i=1}^d a_i (w - \tilde w)\cdot A^\textrm{(full)}_i  }\\
%     =& \abs{\sum_{i=d_\delta +1}^{d} a_i \inner{u_i}{w'}} 
%     \stackrel{(a)}{\leq}  \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \norm{w'}_2 \stackrel{(b)}{\leq} \sqrt{k-d_\delta} \delta \norm{w'}_2\,,
% \end{align*}
% where Eq~(a) applies Cauchy-Schwarz inequality and Eq~(b) applies Eq~\eqref{eq:anorm}.


% % that 
% % hold $A^\textrm{(full)}\tilde w =(e_1,\beta)$, we have
% % \begin{align*}
% %     \tilde w\cdot V =  \sum_{i=1}^d{a_i \tilde w \cdot A^\textrm{(full)}_i} = a_1 +\sum_{i=1}^{d-d_\delta} a_{d_\delta+i} \beta_i =\sum_{i=1}^d{a_i w' \cdot A^\textrm{(full)}_i}= w'\cdot V\,.
% % \end{align*} 
% % According to the definition of $d_\delta$, $\inner{V^\pi}{u_i} $
% % For every value vector $V = \sum_{i=1}^d a_i A^\textrm{(full)}_i$, $V$'s component in $\Span(B)$ is upper bounded by $\sqrt{k-d_\delta}\delta$ due to the definition of the procedure (where there exists a basis of $\Span(\mathcal{V})^\perp$ such that no policy has $\geq \delta$ component in the direction of each basis vector). \lc{LC: The way it is written now implies that the rows in $B$ could be \textit{any} basis, we should change it so this will be correct.]}
% % Then we have

% % where the one before last inequality follows from Cauchy-Schwarz. Finally, since $w'$  holds $A^\mathrm{(full)}\tilde w = (e_1,\beta)$, it follows from the above that for every value vector $V$ we have $$\abs{w\cdot V- w'\cdot V} \leq \sqrt{k-d_\delta} \delta \norm{\beta}_2\,.$$


% % Let $b_i=A^\mathrm{(full)}_{d_\delta +i}$ denote the $i$-th row of $B$.
% % Then, for all $w$ satisfying $ A^{(\delta)} w = e_1$, we can construct a $\tilde w = w +\sum_{i=1}^{d-d_\delta}\beta_i b_i$ satisfying $A^\mathrm{(full)}\tilde w = (e_1,\beta)$.
% % Thus, we have
% % \lc{[LC: I'm missing the definition of $b_i$ in the following equation.  If there are the rows of the matrix $b$ from the pink part then we should store these in $B$ because currently $B$ is not necessarily the same as in the pink part. If it is any basis for $B$ then it's not clear to me why the one before last inequality holds. Also, if they are not related, it is confusing to have $b_1,...,$ as the members of an  arbitrary basis for $\Span(\mathcal V)^\perp$ at each step of the procedure.]}
% % \hsedit{[HS:  $B$ is defined as an arbitrary othonormal basis of $\Span(\text{all policies})\setminus \Span(\mathcal V)$. It is unrelated to the pink part. It is unrelated to ``$b_1,...,$ as the members of an  arbitrary basis for $\Span(\mathcal V)^\perp$ at each step of the procedure'' either (I just changed the notations of this basis to $u_1, u_2,\ldots$ to avoid confusion). 
% % (Sorry for abusing the notation)
% % The second last inequality holds because $\sum_{i=d'+1}^d\abs{a_i} \abs{b_i\cdot (w-\tilde w)} \leq \sqrt{\sum_{i={d_\delta+1}}^d a_i^2} \sqrt{\sum_{i={d_\delta+1}}^d (b_i\cdot (w-\tilde w))^2}$ and $\sqrt{\sum_{i={d_\delta+1}}^d (b_i\cdot (w-\tilde w))^2}\leq  \norm{w-\tilde w}_2$ due to that $b_i$s are othonormal.] }


% % for any $w\lc{\in \R^k}$ satisfying $Aw =\lc{c_1} e_1$we can construct a 
% %  $\tilde w = w +\sum_{i=1}^{d-d'}\beta_i b_i$ satisfying $A'\tilde w = (e_1,\beta)$.
% % Thus \lc{for every value vector $V$} we have $$\abs{w\cdot V- w'\cdot V}=\abs{w\cdot V- \tilde w\cdot V} \leq \sqrt{k-d'} \delta \norm{\beta}_2\,.$$
% \end{proof}

==> multi-objective/section/app_min_norm_hatw_delta.tex <==
%!TEX root = ../main.tex
\section{Proof of Lemma~\ref{lmm:min_norm_hatw_delta}}\label{app:min_norm_hatw_delta}
\begin{proof}
% \iffalse
% We introduce some notations first.
% For any $x,y\in\R^k$, let $\theta(x,y)$ denotes the angle between $x$ and $y$.
% For any subspace $U\subset \R^k$, let $\theta(x,U) := \min_{y\in U}\theta(x,y)$.
% For any two subspaces $U,U'\subset \R^k$, $\theta(U,U') := \max_{x\in U} \min_{y\in U'}\theta(x,y)$.
% For any matrix $M$, let $M_{i:j}$ denote the submatrix of $M$ composed of rows $i,i+1,\ldots,j$ and $M_{i:}$ denote the submatrix composed of all rows $j\geq i$.
% To prove Lemma~\ref{lmm:gap-hatw-w}, we introduce the following lemma by~\cite{Balcan2015}.
% \begin{lemma}[Lemma 3 of~\cite{Balcan2015}]\label{lmm:Balcan}
% Let $U_l = \Span(\xi_1,\ldots,\xi_l)$ and $\hat U_l = \Span(\hat \xi_1,\ldots,\hat \xi_l)$.
% Let $\epsilon_{\text{acc}}, \gamma\geq 0$ and $\epsilon_{\text{acc}}\leq \gamma^2/(10l)$.
% Assume for $i=2,\ldots, l$ that $\theta(\hat \xi_i, \hat U_{i-1})\geq \gamma$, and for $i=1,\ldots, l$, $\theta(\xi_{i}, \hat \xi_{i})\leq \epsilon_{\text{acc}}$. Then
% $$\theta(U_l, \hat U_l)\leq 2l\frac{\epsilon_{\text{acc}}}{\gamma}\,.$$
% \end{lemma}
% Now we use Lemma~\ref{lmm:Balcan} to show that 
% \[\theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq 
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}\,,\]
% and
% \[\theta(\Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq 
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}\,.\]
% For all $2\leq i \leq d_\delta$, we have that
% \begin{align*}
%     &\theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{2:i-1})) \geq \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})) \geq \sin( \theta(\hat A^{(\delta)}_i, \Span(\hat A^{(\delta)}_{1:i-1})))\\ \stackrel{(a)}{\geq}&\frac{\abs{\hat A^{(\delta)}_i \cdot u_i}}{\norm{\hat A^{(\delta)}_i}_2}\geq
%     \frac{\delta}{\norm{\hat A^{(\delta)}_i}_2} = \frac{\delta}{\norm{\hat \alpha_{i-1} V_{1} -V_{i}}_2} \geq \frac{\delta}{(\sqrt{d}+1)u}
% \,,
% \end{align*}
% where Ineq~(a) holds as $u_i$ is orthogonal to $\Span(\hat A^{(\delta)}_{1:i-1})$ according to line 3 of Algorithm~\ref{alg:policy-threshold-free}.
% The last inequality holds due to $\norm{\hat \alpha_{i-1} V_1 -V_{i}}_2 \leq \abs{\hat \alpha_{i-1}} \norm{V_1}_2+\norm{V_i}_2 \leq (\sqrt{d}+1)u$ \hsedit{[HS:need to change $\sqrt d+1$ a little]}.
% Similarly, we also have
% \[\theta(A^{(\delta)}_i, \Span(A^{(\delta)}_{2:i-1}))\geq \frac{\delta}{(\sqrt{d}+1)u}\,.\]

% Denote by $v_i^\parallel = V_i\cdot \frac{V_1}{\norm{V_1}_2}$, $V_i^\parallel =v_i^\parallel \frac{V_1}{\norm{V_1}_2}$, $V_i^\perp =V_i -V_i^\parallel$ and $v_i^\perp = \norm{V_i^\perp}_2$.
% Then we have 
% \[\theta( A^{(\delta)}_i,\hat A^{(\delta)}_i) = \theta(\alpha_{i-1} V_{1} -V_{i},\hat\alpha_{i-1} V_{1} -V_{i})= \theta(\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp,\hat\alpha_{i-1} V_{1} -V_{i}^\parallel- V_i^\perp)\,.\]
% If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) \geq 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the same direction, then
% \begin{align}
%     \theta(A^{(\delta)}_i,\hat  A^{(\delta)}_i) 
%     &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}-\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} }\nonumber\\
%     & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} - \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\label{eq:arctan}\\
%     &\leq\frac{\abs{\hat \alpha_{i-1} - \alpha_{i-1}}\norm{V_1}_2}{v_i^\perp}\nonumber\\
%     &\leq \frac{\epsilon u}{\delta}\,,\label{eq:applytau}
% \end{align}
% where Ineq~\eqref{eq:arctan} follows from the derivative of $\arctan$ is at most 1, i.e., $\partial \arctan x/\partial x = \frac{1}{1+x^2}\leq 1$.
% Ineq~\eqref{eq:applytau} holds since $v_i^\perp \geq \abs{\inner{V_i}{u_i}}\geq \delta$.
% If $(\hat \alpha_{i-1} V_{1} -V_{i}^\parallel)\cdot(\alpha_{i-1} V_{1} -V_{i}^\parallel) < 0$, i.e., $\hat \alpha_{i-1} V_{1} -V_{i}^\parallel $ and $\alpha_{i-1} V_{1} -V_{i}^\parallel$ are in the opposite direction, then we have $\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}+\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}\leq \epsilon \norm{V_1}$
% \begin{align*}
%     \theta(\hat A^{(\delta)}_i, A^{(\delta)}_i) 
%     &= \abs{\arctan \frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}+\arctan \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} } \\
%     & \leq \abs{\frac{\norm{\hat \alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp} + \frac{\norm{\alpha_{i-1} V_{1} -V_{i}^\parallel}_2}{v_i^\perp}}\\
%     &\leq\frac{\epsilon \norm{V_1}_2}{\abs{v_i^\perp}}\nonumber\\
%     &\leq \frac{\epsilon u}{\delta}\,.
% \end{align*}
% Now we are ready to apply Lemma~\ref{lmm:Balcan} by letting Let $\hat \xi_i = \hat A^{(\delta)}_{i+1}$, $\xi_i = A^{(\delta)}_{i+1}$, $\epsilon_{\text{acc}} = \frac{\epsilon u}{\delta}$ and $\gamma = \frac{\delta}{(\sqrt{d}+1)u}$.
% When 
% $\delta \geq 3(\sqrt{d}+1)^{\frac{4}{3}}u\epsilon^\frac{1}{3}$, by Lemma~\ref{lmm:Balcan} we have that
% \[\theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq %\lc{ 2d'\cdot \frac{2u}{\delta}\frac{\epsilon u}{\delta}=}
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}=:\eta_{\ealpha,\delta}\,,\]
% and
% \[\theta(\Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq 
% \frac{2d_\delta(\sqrt{d}+1) u^2\epsilon }{\delta^2}\,.\]
% \fi

Recall that $\barwd =\argmin_{\hat A^{(\delta)} x =\be_1}\norm{x}_2$ is the minimum norm solution and thus, $\inner{\barwd}{\basis_i} = 0$ for all $i\in [d-d_\delta]$.
Let $\lambda_1,\ldots,\lambda_{d_\delta-1}$ be any orthonormal basis of $\Span(A^{(\delta)}_{2:})$.
Then we construct a $w$ satisfying $A^\textrm{(full)} w =\be_1$ by removing $\barwd$'s component in $\Span(A^{(\delta)}_{2:})$ and rescaling.
Let 
\begin{equation}\label{eq:creatw}
    w = \frac{\barwd - \sum_{i=1}^{{d_\delta}-1} \inner{\barwd}{\lambda_i} \lambda_i}{1 -V^{\pi_1}\cdot( \sum_{i=1}^{{d_\delta}-1} \inner{\barwd}{\lambda_i} \lambda_i)}\,.
\end{equation}


% Let $u_1,\ldots,u_k$ be an orthonormal basis of $\R^k$ s.t. $u_1,\ldots,u_{d_\delta-1}\in \Span(A^{(\delta)}_{2:})$ and $u_{d_\delta},\ldots,u_{k} \perp \Span(A^{(\delta)}_{2:})$.
% Let 
% \begin{equation}\label{eq:creatw}
%     w = \frac{\barwd - \sum_{i=1}^{{d_\delta}-1} (\barwd\cdot u_i) u_i}{A^{(\delta)}_1\cdot(\barwd - \sum_{i=1}^{{d_\delta}-1} (\barwd\cdot u_i) u_i)}\,.
% \end{equation}
It is direct to check that $A_1\cdot w = 1$ and $A_i \cdot w = 0$ for $i=2,\ldots,d_\delta$, i.e., $A^{(\delta)}w =\be_1$.
Combining with that $\barwd$ has zero component in $b_i$ for all $i\in [d-d_\delta]$, we have $A^\textrm{(full)} w =\be_1$.

According to Lemma~\ref{lmm:spanangle}, we have $\theta(\Span(A^{(\delta)}_{2:}), \Span(\hat A^{(\delta)}_{2:})) \leq  \eta_{\ealpha,\delta}$, there exist unit vectors $\tilde \lambda_1,\ldots,\tilde \lambda_{d_\delta-1}\in \Span(\hat A^{(\delta)}_{2:})$ such that $\theta(\lambda_i, \tilde \lambda_i)\leq \eta_{\ealpha,\delta}$.
Since $\hat A^{(\delta)} \barwd = \be_1$, we have $\barwd \cdot \tilde \lambda_i = 0$ for all %$i\in [d'-1]$
$i=1,\ldots,d_\delta-1$.
Thus,
\begin{align*}
    \abs{\barwd \cdot \lambda_i} =  \abs{\barwd \cdot (\lambda_i-\tilde \lambda_i)} \leq \norm{\barwd}_2 \eta_{\ealpha,\delta}\,,
\end{align*}
which implies that for any policy $\pi$ value vector $V^\pi$,
\[V^\pi\cdot\sum_{i=1}^{d_\delta-1} (\barwd\cdot \lambda_i) \lambda_i\leq \norm{V^\pi}_2 \sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta} \leq \cv\sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta} \,.\]
% Thus,
% \begin{equation}
%     A^{(\delta)}_1\cdot(\barwd - \sum_{i=1}^{d_\delta-1} (\barwd\cdot \lambda_i) \lambda_i)\geq 1-\sqrt{d_\delta}u\eta_{\ealpha,\delta}\norm{\barwd}_2\,.\label{eq:wrescale}
% \end{equation}
Denote by $\gamma =V^{\pi_1}\cdot( \sum_{i=1}^{{d_\delta}-1} \inner{\barwd}{\lambda_i} \lambda_i)$, then we have
\begin{align*}
    \abs{\barwd \cdot V^\pi - w\cdot V^\pi}& \leq \abs{\barwd \cdot V^\pi - \frac{1}{1-\gamma} \barwd\cdot V^\pi} + \abs{\frac{1}{1-\gamma} \barwd\cdot V^\pi - w\cdot V^\pi}\\
    &\leq \frac{\gamma \norm{\barwd}_2 \cv}{1-\gamma} +\frac{1}{1-\gamma}\abs{\sum_{i=1}^{d_\delta-1} (\barwd\cdot \lambda_i) \lambda_i\cdot V^\pi}\\
    &\leq \frac{\gamma \norm{\barwd}_2 \cv}{1-\gamma} +\frac{\cv\sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta}}{1-\gamma} =\cO\left( \frac{(\calpha+1)\cv^4 d_\delta^{\frac{3}{2}}\norm{\barwd}_2^2\ealpha }{\delta^2}\right)
\end{align*}
when $\cv\sqrt{d_\delta}\norm{\barwd}_2\eta_{\ealpha,\delta} = \cO(1)$.
Now we only need to show that $\norm {\barwd}_2 \leq C\norm{w'}_2$ for some constant $C$.
This can be proved by a construction similar to Eq~\eqref{eq:creatw}.
Let $b_1,\ldots,b_{d_\delta-1}$ be any orthonormal basis of $\Span(\hat A^{(\delta)}_{2:})$.
We construct a $\hatwo$ s.t. $\hat A^{(\delta)}\hatwo = \be_1$ by removing $w'$'s component in $\Span(\hat A^{(\delta)}_{2:})$ and rescaling.
Specifically, let 
\begin{equation}
    \hatwo = \frac{ w'- \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}{1-\inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}}\,.
\end{equation}
Since $A^{(\delta)}w' = \be_1$, 
it is direct to check that $\inner{\hat A_1}{\hatwo} = \inner{V^{\pi_1}}{\hatwo} = 1$ and $\hat A_i \cdot \hatwo = 0$ for $i=2,\ldots,d_\delta$, i.e., $\hat A^{(\delta)}\hatwo =\be_1$.



% Let $\lambda = \inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}$ and we show that $\lambda$ is small as follows.
Since $\theta( \Span(\hat A^{(\delta)}_{2:}), \Span(A^{(\delta)}_{2:})) \leq  \eta_{\ealpha,\delta}$ according to Lemma~\ref{lmm:spanangle}, there exist unit vectors $\tilde b_1,\ldots,\tilde b_{d_\delta-1}\in \Span(A^{(\delta)}_{2:})$ such that $\theta(b_i,\tilde b_i)\leq \eta_{\ealpha,\delta}$.
Since $w'$ has zero component in $\Span(A^{(\delta)}_{2:})$, $w'$ should have a small component in $\Span(\hat A^{(\delta)}_{2:})$.
In particular,
\begin{align*}
     \abs{\inner{w'}{b_i}}= \abs{\inner{w'}{b_i-\tilde b_i}} \leq \norm{w'}_2 \eta_{\ealpha,\delta}\,,
\end{align*}
which implies that 
\begin{align*}
    \norm{\sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i}_2\leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta}\,.
\end{align*}
Hence
\begin{equation*}
    \abs{\inner{V^{\pi_1}}{( \sum_{i=1}^{{d_\delta}-1} \inner{w'}{b_i} b_i)}} \leq \sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv\,,
\end{equation*}
and then there exists a constant $C>0$ such that 
$\norm{\hatwo}_2 \leq C \norm{w'}_2$ when $\sqrt{d_\delta -1} \norm{w'}_2 \eta_{\ealpha,\delta} \cv = \cO(1)$.
Since $\barwd$ is the minimum norm solution, we have $\norm{\barwd}_2\leq C \norm{w'}_2$.
\end{proof}

==> proposal.tex <==
Machine learning has witnessed remarkable breakthroughs in recent years.
Most machine learning techniques assume that the training and test data are sampled from an underlying distribution and aim to find a predictor with low population loss.
However, data may be generated by \emph{strategic} individuals, collected by \emph{self-interested} agents, possibly poisoned by \emph{adversarial} attackers, and used to create predictors, models, and policies satisfying \emph{multiple objectives}. As a result, predictors may underperform, such as deep neural networks' vulnerability to adversarial examples~\citep{szegedy2013intriguing,shafahi2018poison} and unbounded mistakes of the classic Perceptron algorithm in the presence of strategic individuals~\citep{ahmadi2021strategic}.
To ensure the success of machine learning, it is crucial to develop trustworthy algorithms capable of handling these factors. This thesis proposal focuses on modeling strategic and adversarial data sources, analyzing their effects on predictors, and designing new methods and insights to enhance accuracy. More specifically, we explore the following problems.
\begin{itemize}
    \item When dealing with adversarial attackers, algorithms that do not take these adversaries into account tend to perform poorly. Ensuring robustness in the presence of such adversaries constitutes a primary focus of my research. (Section~\ref{sec:adversarial})
    
    \item In strategic classification, examples can strategically manipulate their features in order to achieve a more favorable classification outcome. For example, given a classifier determining college admission, student candidates may try to take easier classes to improve their GPA, retake SAT and change schools in an effort to fool the classifier. Hence, I have also worked on developing an algorithm robust to agents' manipulation. (Section~\ref{sec:strategic})
    
    \item In multi-objective learning problem, users have more than one objectives. For example, for investment portfolio, people care about not only the gain but also the risk. Then instead of scalar losses, we should design techniques for vector losses. (Section~\ref{sec:multi-obj})
    
    \item Collaborative approaches like federated learning involve multiple data collectors who share data to train a shared model. The incentive issue arises if these collectors will not share data if they perceive insufficient benefits. The question is how to design algorithms to make sure data collectors will be willing to contribute their data. (Section~\ref{sec:incentive})
    
    \item Finally, both strategic classification and incentivized collaboration problems are learning problems involving gaming agents. Conversely, I also consider games in which agents are learning and design mechanisms to ensure low regret even when the agent is running a learning algorithm instead of best responding, which is commonly assumed in game theory literature. For example, in Stackelberg games, it is commonly assumed that the leader selects the policy, and the follower best responds to it. Nevertheless, when the agent is employing a learning algorithm, what level of utility can we attain for the principal? (Section~\ref{sec:game})
\end{itemize}





\section{Accuracy and Robustness under Adversarial Data}\label{sec:adversarial}
Adversarial attackers can poison the traing data~\citep{biggio2012poisoning,barreno2006can,papernot2016towards,steinhardt2017certified}, perturb the training data~\citep{koh2017understanding},perturb the test data~\citep{szegedy2013intriguing,goodfellow2014explaining,bubeck2019adversarial,cullina2018pac,montasser2019vc,montasser2020efficiently} and etc.
The extensive literature has delved into the exploration of ensuring the predictor's robustness against adversarial attackers
Under this topic, I have studied two problems---one on a specific type of data poisoning called clean-label data-poisoning attacks and one on transformation invariances.






% robustness under adversarial attacks. Extensive studies have explored various adversarial attacks, including data poisoning (which involves injecting malicious data points during training to deceive the predictor)~\citep{biggio2012poisoning,barreno2006can,papernot2016towards,steinhardt2017certified}, perturbation over training examples~\citep{koh2017understanding}, perturbation over test examples~\citep{szegedy2013intriguing,goodfellow2014explaining,bubeck2019adversarial,cullina2018pac,montasser2019vc,montasser2020efficiently} and etc.
% I have been considering two problems related to adversarial attacks.

% Regarding the second problem. 



\subsection{Robust Learning under Clean-Label Attack}
Data poisoning is an attack on machine learning algorithms where the attacker adds examples to the training set with the goal of causing the algorithm to produce a classifier that makes specific mistakes the attacker wishes to induce at test time.
Clean label attacks, involving the injection of \emph{correctly-labeled} data points, have been empirically verified to be effective on deep neural networks by~\citet{shafahi2018poison}.
However, we are curious whether this phenomenon is solely attributable to overparameterized models or if it can also occur for well-understood function classes like halfspaces.  It's important to note that the objective of these attacks is not to increase the overall error rate, but rather to induce errors specifically at targeted instances.

Formally, let $\cX$ denote the instance space, $\cY = \{0,1\}$ denote the label space and $\cH\subseteq \cY^\cX$ denote the hypothesis class. We focus on the realizable case where there exists a target function $h^*\in \cH$ such that the training set and the test set are realized by $h^*$. 
% Let $D_{h^*} = \{(x,h^*(x))|x\in \cX\}$ denote the data space where every instance is labeled by $h^*$.
A learning algorithm $\A$ is a map (possibly including randomization), from a labeled data set $S$ of any size, to a hypothesis $h\in \cY^\cX$. 
% For simplicity, we denote by $\cA(S,x) = \cA(S)(x)$ the prediction of $\cA(S)$ at an instance $x$.
An attacker $\Adv$ maps a target function $h^*$, a training data set $S_\trn$ and a specific test instance $x$ to a data set $\Adv(h^*,S_\trn,x)$ and injects $\Adv(h^*,S_\trn,x)$ into the training set with the intent of making the learning algorithm misclassify $x$. 
We call $\Adv$ a clean-label attacker if $\Adv(h^*,S_\trn,x)$ is consistent with $h^*$. 
For any deterministic algorithm $\A$, we say a point $x\in\cX$ is attackable if there exists a clean-label attacker $\Adv$ leading the algorithm to misclassify $x$, i.e.,
\begin{align*}
    \A(S_\trn\cup \Adv(h^*,S_\trn,x),x)\neq h^*(x)\,.
\end{align*}
% To be clear, we are defining $S_\trn\cup \Adv(h^*,S_\trn,x)$ as an unordered multiset. 
Then we define clean-label attackable rate as follows.
\begin{dfn}[clean-label attackable rate]\label{dfn:rate}
  For a target function $h^*$, a training data set $S_\trn$ and a (possibly randomized) algorithm $\A$, for any distribution $\cD$ over $\cX\times h^*(\cX)$, the attackable rate by an clean-label attacker $\Adv$ for $(h^*, S_\trn, \A)$ is defined as
    \begin{align*}
      \atk_\cD(h^*, S_\trn,\A,\Adv) := \EEs{(x,y)\sim \cD,\cA}{\1{\A(S_\trn\cup \Adv(h^*,S_\trn,x),x)\neq h^*(x)}}\,.  
    \end{align*}
    The clean-label attackable rate is defined by taking supremum over all clean-label attackers, i.e., 
    \begin{align*}
      \atk_\cD(h^*, S_\trn,\A) := \sup_\Adv \atk_\cD(h^*, S_\trn,\A,\Adv)\,.  
    \end{align*}
\end{dfn}

Now we define our learning problem as follows.
\begin{question}\label{q:clean-label}
Analogous to PAC learnability, we say $\cH$ is $(\epsilon,\delta)$-robust learnable if $\forall \epsilon,\delta \in (0,1)$, there exists an algorithm $\A$ such that for every target function $h^*\in\cH$ and data distribution over $\cX\times h^*(\cX)$, with probability at least $1-\delta$, we can achieve $\epsilon$ attackable rate using finite examples.
Then the question is: what hypothesis classes are $(\epsilon,\delta)$-robust learnable? Especially, can we robustly learn halfspaces?
\end{question}

\paragraph{Our Results.} In our work~\citep*{blum2021robust}, we initially introduce some robustly learnable hypothesis classes, including classes with VC dimension of 1, intersection-closed hypothesis classes, and etc. Besides, we also show a connection between robust learning and standard PAC learning: all robust algorithms can achieve optimal dependence on $\epsilon$ in their PAC sample complexity.

Regarding linear classifiers, we demonstrate that $n$-dimensional halfspaces for $n\geq 2$ are not robustly learnable. Additionally, we construct an linear example in which SVM requires at least $ e^{\Omega(n)}$ samples to achieve low attackable rate even if the attacker is only allowed to inject one poison example into the training set.
% Finally, we study the situation where the attacker is restricted to inject at most $t$ poison examples.

\subsection{Improved Accuracy under Transformation Invariances}
Consider an image classification scenario where an attacker perturbs test data by applying rotations and altering colors in an attempt to mislead the classifier into making errors.
It is important to note that the true label of an image is invariant to rotation and color transformations. To improve accuracy and robustness, such invariances are often built into the learning process by a universally applicable and easy way called \emph{data augmentation (DA)}. That is, adding the transformed data into the training set and training a model with the augmented data\footnote{We refer to ERM over the augmented data by DA.}.

% One is designing new architectures in neural networks to learn a transformation invariant feature, which is usually task-specific and challenging.
Such transformation invariances are present in many real-world learning problems.
That is, given a certain set of transformations, the label of an instance is preserved under any transformation from the set.
Image classification is often invariant to rotation/flip/color translation.
Syntax parsing is invariant to exchange of noun phrases in a sentence.
Empirical findings have substantiated the effectiveness of DA in improving accuracy, leading to its widespread adoption in modern deep learning, as illustrated by models such as AlexNet~\citep{krizhevsky2012imagenet}. Nevertheless, it remains uncertain under what circumstances DA provides a benefit.
As a result, it is natural to pose the following theoretical questions.
\begin{center}
    \emph{How does data augmentation perform theoretically? 
    \\What is the optimal algorithm in terms of sample complexity under transformation invariances?}
\end{center}
We study the binary classification under transformation invariances.
Let $\cX$ denote the instance space, $\cY=\{0,1\}$ denote the label space and $\cH$ denote the hypothesis class. 
We consider a group $\cG$ of transformations, which acts on the instance space: there is a mapping $\alpha: \cG \times \cX \mapsto \cX$ such that $\alpha(e,x)=x$ for the identity element $e\in \cG$ and $\alpha(g_1g_2,x)=\alpha(g_1, \alpha(g_2,x))$ for $g_1,g_2\in \cG$.
For convenience, we write $\alpha(g,x) =gx$ for $g\in \cG$ and $x\in \cX$. 
The \emph{orbit} of any $x\in \cX$ is the subset of $\cX$ that can be obtained by acting an element in $\cG$ on $x$, $\cG x := \{gx|g\in \cG\}$. 
Note that since $\cG$ is a group, for any $x'\in \cG x, \cG x' = \cG x$. 
Thus we can divide the instance space $\cX$ into a collection of separated orbits, which does not depend on the data distribution.

For any distribution $\cD_\cX$ over $\cX$, we say a hypothesis $h$ is \emph{$(\cG,\cD_\cX)$-invariant} if h is invariant over almost every orbit. That is to say, 
$h(gx) = h(x)$ for all $g\in \cG$, for almost every $x$, i.e., $\Pr_{x\sim \cD_\cX}(\exists x'\in \cG x : h(x')\neq h(x)) = 0$.
We say a distribution $\cD$ over $\cX\times \cY$ is \emph{$\cG$-invariant} if there exists a $(\cG,\cD_\cX)$-invariant hypothesis $f^*$ (possibly not in $\cH$) with $\err_\cD(f^*) = 0$. To model invariance, we assume that the data distribution is $\cG$-invariant.

% Given a data set $S\subset \cX\times \cY$, denote $\cG S = \{(gx,y)|(x,y)\in S,g\in \cG\}$ the augmented data set.
% For a transformation group $\cG$ and a multi-subset $X$ of $\cX$, we say a hypothesis $h$ is \emph{$(\cG,X)$-invariant} if 
% \[h(gx) = h(x),\forall g\in \cG, x\in X\,.\]
% That is to say, for every $x\in X$, $h$ predicts every instance in the orbit of $x$ the same as $x$.
% Given a sample $S$, we say $S$ is $\cG$-invariantly realizable by $\cH$ if there exists a $(\cG, S_\cX)$-invariant hypothesis $h\in \cH$ such that $y = h(x)$ for all $(x,y)\in S$.


We consider three settings with different levels of realizability: (i) invariantly realizable setting, where there exists a $(\cG, \cD_\cX)$-invariant hypothesis in $\cH$ with zero error; (ii) relaxed realizable setting, where there exists a hypothesis in $\cH$ with zero error; and (iii) agnostic setting.
To understand the difference between the two realizable settings, here is an example.
Consider $\cX = \{\pm 1,\pm 2\}$, $\cG=\{e,-e\}$ (i.e., $\cG x = \{x,-x\}$), and the data distribution $\cD$ being a uniform distribution over $\{(1,0),(2,0)\}$.
If $\cH$ contains the all-zero function $h(\cdot) = 0$, then it is in setting (i); If $\cH$ contains the hypothesis $\1{x<0}$ but does not contain the all-zero function, then it is in setting (ii).

\begin{question}\label{q:da}
    This immediately prompts the question: what are the optimal sample complexity, the sample complexity of DA, and the sample complexity of vanilla ERM in each setting?
    Addressing this question provides an answer to when DA is beneficial (i.e., when its sample complexity is lower than that of vanilla ERM) and when DA is optimal. Another natural question is how to construct optimal algorithms if DA is not optimal.
\end{question}

\paragraph{Our Results.} Our recent work~\citep*{shao2022theory} provides a comprehensive solution to this question. First, we show that DA outperforms vanilla ERM but is sub-optimal in setting (i) above.
We then introduce a complexity measure that characterizes the optimal sample complexity of learning in setting (i), 
and we give an optimal (up to log-factors) algorithm in this setting based on 1-inclusion-graph predictors.
Second, we characterize the complexity of learning in setting (ii) when the learner only receives the augmented data (without specifying which are natural).
Such a characterization provides us with a sufficient condition under which DA ``hurts''.
Finally, we introduce a complexity measure that characterizes the optimal sample complexity of learning in settings (ii) and (iii) above, and we give optimal algorithms for these settings. 
% \item Finally, we also provide adaptive learning algorithms that interpolate between settings (i) and (ii), i.e., when $h^*$ is {\em partially} invariant. 
% We want to emphasize that our complexity measures take into account the complexity of both the hypothesis class $\cH$ and the set of transformations being considered.




\section{Strategic Classification}\label{sec:strategic}
One of my research areas is strategic classification, where agents can strategically manipulate their feature vector up to an extent in order to be predicted as positive. For example, given a classifier determining college admission, student candidates may try to take easier classes to improve their GPA, retake SAT and change schools in an effort to fool the classifier. This area, first proposed by ~\citet{hardt2016strategic}, has received significant attention in subsequent research efforts~\citep{dong2018strategic,chen2020learning,ahmadi2021strategic, ahmadi2023fundamental,zhang2021incentive,sundaram2021pac,lechner2022learning}.
Most existing works assume uniform or known manipulation abilities, which do not reflect practical scenarios.
Unlike most prior work, we consider manipulations to be \emph{personalized}, meaning that agents can have different levels of manipulation abilities (e.g., varying radii for ball manipulations), and \emph{unknown} to the learner.

We consider the binary classification task.
Let $\cX$ denote the feature vector space, $\cY = \{+1,-1\}$ denote the label space, and $\cH$ denote the hypothesis class.
An example is represented by a triple $(x,u,y)$,  where $x \in \cX$ is the original feature vector, $y \in \cY$ is the label, and $u \subseteq \cX$ is the manipulation set, which is a set of feature vectors that the agent can modify their original feature vector $x$ to. 
In particular, given a hypothesis $h\in \cY^\cX$, the agent will try to manipulate her feature vector $x$ to another feature vector $x'$ within $u$ in order to receive a positive prediction from $h$.
More formally, for an agent $(x,u,y)$, given a predictor $h$, if $h(x) = -1$ and her manipulation set overlaps the positive region by $h$, i.e., $u \cap \cX_{h,+}\neq \emptyset$ with $\cX_{h,+}:= \{x\in \cX|h(x)=+1\}$, then the agent will manipulate $x$ to $\Delta(x,h,u)\in u\cap \cX_{h,+}$. Otherwise, the agent will do nothing and maintain her feature vector at $x$, i.e., $\Delta(x,h,u)=x$.

One commonly studied case is ball manipulations, where the manipulation set $u=\cB(x;r)$ is a ball centered at $x$ with some radius $r$ w.r.t. some metric $d$\footnote{For ball manipulations, agents break ties by selecting the closest one. For non-ball manipulations, agents break ties randomly.
}. 
The strategic loss of $h$ is the 0-1 loss of the prediction at the manipulated feature, i.e.,
\begin{align*}
    \lossstr(h,(x,u,y)) := \1{h(\Delta(x,h,u))\neq y}\,.
\end{align*}

We consider that a sequence of agents $(x_1,u_1,y_1),(x_2,u_2,y_2),\ldots, (x_T,u_T,y_T)\in \cQ\times \cY$ that arrives in an online manner.
At each round, the learner feeds a predictor to the environment and then observes his prediction $\hat y_t$, the true label $y_t$ and possibly along with some additional information about the original/manipulated feature vectors. The interaction protocol (which repeats for $t=1,\ldots,T$) is described in the following.
\begin{protocol}[H]
    \caption{Learner-Agent Interaction at round $t$}
    \label{prot:interaction}
        \begin{algorithmic}[1]
            \STATE The environment picks an agent $(x_t,u_t,y_t)$ and reveals some context $C(x_t)$. In the online setting, the agent is chosen adversarially, while in the distributional setting, the agent is sampled i.i.d.
            \STATE The learner $\cA$ observes $C(x_t)$ and picks a hypothesis $f_t\in \cY^\cX$.
            \STATE The learner $\cA$ observes the true label $y_t$, the prediction $\hat y_t = f_t(\Delta_t)$, and some feedback $F(x_t,\Delta_t)$, where $\Delta_t = \Delta(x_t,f_t,u_t)$ is the manipulated feature vector.
        \end{algorithmic}
    \end{protocol}
% \vspace{-4mm}
The context function {$C(\cdot)$} and feedback function {$F(\cdot)$} reveals information about the original feature vector $x_t$ and the manipulated feature vector $\Delta_t$. {$C(\cdot)$} reveals the information before the learner picks $f_t$ while {$F(\cdot)$} does after.
We study several different settings based on what and when information is revealed. The simplest setting for the learner is observing the original feature vector $x_t$ before choosing $f_t$ and the manipulated vector $\Delta_t$ after. In a slightly harder setting, the learner observes both the original and manipulated vectors after selecting $f_t$ and thus, $f_t$ cannot depend on the original feature vector in this case. An even harder setting involves observing only the manipulated feature vector after selecting $f_t$ (which can only be revealed after $f_t$ since $\Delta_t$ depends on $f_t$). The hardest and least informative scenario occurs when neither the original nor the manipulated feature vectors are observed.

The agents can be either generated by an adversary or sampled from a distribution. Our learning objectives can encompass regret in adversarial setting as well as sample complexity in the stochastic setting.
\begin{itemize}
    \item \textbf{Regret in the adversarial setting.} The agents $(x_1,u_1,y_1), (x_2,u_2,y_2),\ldots$ are selected by an adversary and the goal is to minimize the Stackelberg regret w.r.t. a hypothesis class $\cH$. More specifically, our goal is to construct an algorithm which generates a sequence of hypotheses $f_{1:T}$ to minimize Stackelberg regret,
    \begin{equation*}
        \sum_{t=1}^T\lossstr(f_t,(x_t,u_t,y_t)) -\min_{h\in \cH}\lossstr(h,(x_t,u_t,y_t))\,.
    \end{equation*}
    % \item \textbf{Regret in the stochastic setting.}  The agents $(x_t,u_t,y_t)\sim \cD$ is sampled from a distribution over agents. Similar to regret in the adversarial setting, our goal is to minimize the expected Stackelberg regret,
    % \begin{equation*}
    %     \EEs{(x_t,u_t,y_t)_{t=1}^T\sim \cD}{\sum_{t=1}^T\lossstr(f_t,(x_t,u_t,y_t)) -\min_{h\in \cH}\lossstr(h,(x_t,u_t,y_t))}\,.
    % \end{equation*}
    \item \textbf{Sample complexity in the stochastic setting.} Our goal is to find an $\epsilon$ optimal predictor, an $\hat h$ with $\EEs{(x,u,y)\sim \cD}{\lossstr(\hat h,(x,u,y))}\leq \min_{h\in \cH} \EEs{(x,u,y)\sim \cD}{\lossstr(h,(x,u,y))}+\epsilon $, with  the minimal sample complexity.   
\end{itemize}

\begin{question}\label{q:strategic}
    In classic (non-strategic) online learning, the Halving algorithm achieves a mistake bound of $\log(\abs{\cH})$ (in the realizable setting) by employing the majority vote and eliminating inconsistent hypotheses at each round. In classic PAC learning, the sample complexity of $\cO(\frac{\log(\abs{\cH})}{\epsilon})$ is achievable via ERM. Now we assume realizability in the strategic setting: there exists a hypothesis $h^*\in \cH$ such that for any $t\in [T]$, we have $y_t = h^*(\Delta(x_t,h^*,u_t))$. The question is:
    \begin{center}
    \emph{Can we achieve a logarithmic dependency on $\abs{\cH}$ in the strategic setting?}
\end{center}
\end{question}
\paragraph{Our Results.} We answer this question in our recent work~\citep*{shao2023strategic}. 
We show that in the case of ball manipulations, when the original feature vector $x_t$ is revealed prior to choosing $f_t$, we can achieve logarithmic mistake bound and sample complexity via a variant of Halving.
When the original feature vector $x_t$ is not revealed beforehand, the problem becomes significantly more challenging. 
Specifically, any learner will experience a mistake bound that scales linearly with $\abs{\cH}$, and any proper learner will face sample complexity that also scales linearly with $\abs{\cH}$.
We propose an improper learner with $\polylog(\abs{\cH})$ sample complexity.

In the case of non-ball manipulations, the situation worsens. Even in the simplest setting, where the original feature is observed before choosing $f_t$ and the manipulated feature is observed afterward, any learner will encounter a linear mistake bound and sample complexity. 

\paragraph{Open problems.} There are several fundamental open questions on extension to \emph{agnostic setting}, \emph{infinite hypothesis class}, and \emph{non-ball manipulations}.

\begin{question}[combinatorial measures]\label{q:strategic-combinatorial}
Just as VC dimension provides tight characterization for PAC learnability and Littlestone dimension characterizes online learnability, we are curious if there exists a combinatorial measure that captures the essence of strategic classification in this context so that we could provide guarantees for infinite hypotheses, including halfspaces. Note that the proofs of the most lower bounds in \citet{shao2023strategic} consider hypothesis class of singletons, in which both VC dimension and Littlestone dimension are $1$. Therefore, they cannot be candidates to characterize learnability in the strategic setting.
What are the combinatorial measures that tightly characterizes the mistake bound and the sample complexity?
\end{question}

The ball manipulations considered in \citet{shao2023strategic}, are balls of any radii.
Beyond ball manipulations, we can define manipulation function to be a mapping from $\cX$ to $2^\cX$. The agents under manipulation function $m$ should follow the form of $(x,m(x),y)$. Let manipulation class be a class of manipulation functions.
Assume that the manipulation class is known and that the true manipulation function is in the class. It is easy to see that the mistake bound/sample complexity depends on the manipulation class. For example, if the manipulation class contains only one function, it is equivalent to known manipulation. Then we have the following question.

\begin{question}[beyond ball manipulations]\label{q:strategic-nonball}
    Given a hypothesis class $\cH$ and a manipulation class $\cM$, can we find a combinatorial measure based on both $\cH$ and $\cM$ to characterize the mistake bound/sample complexity?
\end{question}

\begin{question}[agnostic setting]\label{q:strategic-agnostic}
Regarding the agnostic setting, in which there is no perfect classifier in the hypothesis class $\cH$, what is the optimal regret/sample complexity?
\end{question}
We can construct an example of $n$ one-dimensional thresholds and a data distribution $\cD$ where the marginal distribution $\cD_{\cX\times \cY}$ over $\cX\times \cY$ is realizable by the thresholds such that the sample complexity is $n/\epsilon^2$. This implies that to achieve logarithmic dependency on $\abs{\cH}$, some additional assumptions are necessary.

\section{Multi-Objective Learning}\label{sec:multi-obj}
While sequential decision making problems typically involve optimizing a single scalar reward, there are many domains for which it is desirable or necessary to optimize over multiple (potentially conflicting) objectives at once. For example, safety, speed, and comfort are all desired objectives of autonomous cars, but speed could negatively impact safety (e.g., it would take longer for the vehicle to suddenly stop) or comfort (e.g., fast turns). In multi-objective learning, I have been working on two problems---preference elicitation in multi-objective decision making and online learning with two losses.

\subsection{Eliciting User Preferences for Personalized Multi-Objective Decision Making through Comparative Feedback}
In this subsection, we consider a problem of designing efficient algorithms to find the optimal personalized policy for a user that reflects their unknown preferences over $k$ objectives.

Similar to prior works on multi-objective decision making, we model the problem using a finite-horizon Markov decision process (MDP) with a $k$-dimensional reward vector, where each entry is a non-negative scalar reward representative of one of the $k$ objectives. To account for user preferences, we assume that a user is characterized by a (hidden) $k$-dimensional \emph{preference vector} with non-negative entries, and that the \emph{personalized reward} of the user for each state-action is the inner product between this preference vector and the reward vector (for this state-action pair). We also distinguish between the $k$-dimensional value of a policy, which is the expected cumulative reward when selecting actions according to the policy, and the \emph{personalized value} of a policy, which is the scalar expected cumulative personalized reward when selecting actions according to this policy. The MDP is known to the agent and the goal is to learn an optimal policy for the personalized reward function (henceforth, the \emph{optimal personalized policy}) of a user.

As knowledge of the user's preference vector is sufficient to solve for their optimal personalized policy, the challenge is to learn a user's preference vector using a minimal number of easily interpretable queries. The problem of eliciting preferences has been studied in \citet{wang2022imo} using a strong query model that provides stochastic feedback on the quality of a single policy.
In contrast, we consider a more natural and intuitive query model, comparison queries, which query the user's preference over two selected policies.

The question is then what exactly to compare? Comparing state-action pairs might not be a good option for the aforementioned tasks---what is the meaning of two single steps in a route?
Comparing single trajectories would not be ideal either. Consider for example two policies: one randomly generates either GOOD or BAD trajectories while the other consistently generates MEDIOCRE trajectories. By solely comparing single trajectories without considering sets of trajectories, we cannot discern the user's preference regarding the two policies. 
Therefore, we are interested in learning preferences via policy comparison queries.

\begin{question}\label{q:multiobj-MDP}
    Given our aim of eliciting preferences through policy comparison feedback, two questions naturally emerge---one concerning efficiency and the other regarding interpretability.
    The efficiency question revolves around determining how to find the optimal personalized policy by querying as few policy comparisons as possible.
    As for interpretability, it's important to note that a policy's explicit representation is a mapping from states to action distributions, which may be challenging for humans to grasp. Consequently, we are intrigued by efficiently finding a more easily interpretable policy representation.
\end{question}

\paragraph{Our Results.} In the recent work~\citep*{shao2023eliciting}, we provide an \emph{efficient} algorithm for finding an approximate optimal personalized policy. As an alternative to an explicit policy representation, we propose a \emph{weighted trajectory set} as a more interpretable representation and design two efficient algorithms that find the weighted trajectory set representation of a policy.

\subsection{Online Learning with Primary and Secondary Loss}
I've also explored another multi-objective learning problem, which involves online learning with two losses, a primary loss and a secondary loss.
For example, a recruiter making decisions of which job applicants to hire might weigh false positives and false negatives equally (the primary loss) but the applicants might weigh false negatives much higher (the secondary loss). This leads us to the following inquiry: can we combine ``expert advice'' to achieve \emph{low regret} with respect to the primary loss, while at the same time performing \emph{not much worse than the worst expert} with respect to the secondary loss? 

We study the adversarial online learning setting with a set of $K$ experts $\cH = \{1,\ldots,K\}$. At round $t=1,2,\ldots,T$, an online learner $\cA$ computes a probability distribution $p_t\in \Delta_K$ over $\cH$ and selects one expert from $p_t$. Simultaneously an adversary selects two loss vectors $\loss{1}_t,\loss{2}_t\in [0,1]^K$, where $\loss{1}_{t,h}$ and $\loss{2}_{t,h}$ are the primary and secondary losses of expert $h\in \cH$ at time $t$. Then $\cA$ observes the loss vector and incurs expected losses $\loss{i}_{t,\cA}=p_t^\top \loss{i}_t$ for $i\in \{1,2\}$. Let $\Loss{i}_{T,h} = \sum_{t=1}^T\loss{i}_{t,h}$ denote the loss of expert $h$ and $\Loss{i}_{T,\cA}=\sum_{t=1}^Tp_t^\top \loss{i}_t$ denote the cumulative loss of algorithm $\cA$ for $i\in\{1,2\}$ during the first $T$ rounds. 

We use the standard regret to measure the primary loss performance of a learner, which compares the loss of the learner and the best expert in hindsight. Following~\citet{even2008regret}, we adopt the regret notion of $\cA$ with respect to the primary loss as
\begin{align*}
\reg{1} \triangleq  \max\left({\Loss{1}_{T,\cA}- \min_{h\in \cH} \Loss{1}_{T,h}},1\right)\:.
\end{align*} 
For secondary loss, as we mentioned at the beginning, the goal is to perform not much worse than the worst expert. Hence,
We introduce another metric called {\em regret to $cT$} for some $c\in[0,1]$, which compares the secondary loss of the learner with a linear term $cT$, 
\begin{align*}
\reg{2}_c \triangleq \max\left(\Loss{2}_{T,\cA}- cT,1\right)\,,
\end{align*}
where $c = \max_{h\in \cH} \Loss{2}_{T,h}/T$ is the average loss of the worst expert.

\begin{question}\label{q:primary-secondary}
Is it possible to achieve $\E[{\max(\reg{1}, \reg{2}_c)}]=o(T)$?
\end{question}

\paragraph{Our Results.} Our work~\citep{blum2020online} answers this question negatively. We show that given an expert set $\cH$, there exists an adversary such that any algorithm will incur $\E[{\max(\reg{1}, \reg{2}_c)}]=\Omega(T)$. Then we introduce a bounded variance assumption on the secondary loss that the secondary loss does not exceed the linear threshold by $o(T)$ for any time interval. We show that $\E[{\max(\reg{1}, \reg{2}_c)}]=o(T)$ when this assumption holds for all experts.



\section{Incentives in Collaborative Learning}\label{sec:incentive}
Aside from strategic individuals, the presence of strategic data sources is also significantly influenced by self-interested data collectors. Over recent years, there has been a growing embrace of federated learning as an approach that enables a multitude of learning agents to collectively achieve their objectives while conserving resources, such as smaller datasets. This potential to generate significant impact through mass participation has generated considerable interest in the machine learning research community regarding federated learning. As a result, we have witnessed the development of faster and more communication-efficient collaborative systems. However, the ultimate success and influence of collaborative federated learning hinges on the capacity to attract and retain a large number of learning agents. Achieving this requires collaborative algorithms that provide incentives for agents to actively participate in the learning process.

\subsection{Equilibria in Single Round Interaction}
In this subsection, we model collaborative learning as a single-round game with $k$ agents, wherein each agent determines their level of contribution at the beginning and must commit to it throughout the training process. 
Each agent is interested in accomplishing their learning objectives while keeping their individual sample collection burden low. 
To ensure the active participation of all agents, it is crucial to prevent any instances of inequity that may arise during collaborative learning.
We consider two inequitable circumstances. First, when part of an agent's data is exclusively used to accomplish another agent's learning goals; for example, if an agent's learning task can be accomplished even when she (unilaterally) lowers her data contribution.
Second, when an agent envies another agent; for example, if an agent's learning goal can be accomplished even when she swaps her contribution burden with another agent who has a lower burden.
Our learning goal is to help agents accomplish their learning objectives while ``equitably'' spreading the data contribution responsibilities among agents who want a lower sample collection burden.

Formally, there are $k$ agents and all agents collaboratively select a strategy $\btheta= (\theta_1,\ldots,\theta_k)$ from a strategy space $\Theta\subseteq \R_+^k$. Each agent $i$ selects a number $\theta_i$ as her contribution level, e.g., the number of samples.
We define $u_i:\Theta\mapsto \R$ as the utility function (which is the expected accuracy in collaborative learning) for each agent $i$ and her goal is to achieve 
\[
u_i(\btheta)\geq \mu_i
\]
for some $\mu_i$ (which is minimum accuracy required by the agent). 
% Without loss of generality, we assume that every agent can satisfy her constraint individually, i.e., $\forall i\in[k], \exists \vartheta_i\in \R_+^k$ such that $u_i(\vartheta_i,\bZero_{-i})\geq \mu_i$ and $u_i$ is non-decreasing with $\theta_j$ for any $j$. We say that $\btheta$ is \textbf{feasible} if  $u_i(\btheta)\geq \mu_i$ for all $i\in[k]$. 


The socially optimal solution is the optimal feasible solution that does not consider agents' incentives. More formally, $\btheta^*$ is a \emph{socially optimal solution} in $\Theta$ if it is the optimal solution to the following program
\begin{equation} \label{eq:gen-opt}
    \begin{array}{l}
        \min_{\btheta\in \Theta} \bOne^\top \btheta\\
        \st u_i(\btheta)\geq \mu_i,\forall i\in[k]\,.
    \end{array}
\end{equation}
Now we define two equilibria to avoid the aforementioned inequitable circumstances. A stable equilibrium is a feasible solution where no player has incentive to unilaterally decrease her strategy.  Specifically, for any $\btheta\in \R^k$, $x\in \R$, let $(x,\btheta_{-i})\in\R^k$ denote the vector with the $i$-th entry being $x$ and the $j$-th entry being $\theta_j$ for $j\neq i$. A feasible solution $\btheta^\eq$ is a \emph{stable equilibrium} over $\Theta$ if for any $i\in [k]$, there is no $(\theta_i',\btheta^\eq_{-i})\in \Theta$ such that $\theta_i'<\theta^\eq_i$ and $u_i(\theta_i',\btheta^\eq_{-i})\geq \mu_i$.

An envy-free equilibrium is a feasible solution where no agent has an incentive to swap their sampling load with another agent.
Specifically, for any $\btheta$, let $\btheta^{(i,j)}$ denote the $\btheta$ when the $i$-th and the $j$-th entries are swapped,
i.e., $\theta^{(i,j)}_i=\theta_j$, $\theta^{(i,j)}_j=\theta_i$ and $\theta^{(i,j)}_l=\theta_l$ for $l\neq i,j$. 
A feasible solution $\btheta^\ef$ is \emph{envy-free} if for any $i\in [k]$, there is no $\btheta^{\ef(i,j)}\in \Theta$ such that $\theta^\ef_j<\theta^\ef_i$ and $u_i(\btheta^{\ef(i,j)})\geq \mu_i$. 


% We call an equilibrium $\btheta$ optimal if it is an equilibrium with minimal resources, i.e., minimizes $\bOne^\top\btheta$. 
\begin{question}\label{q:one4one}
     The initial question that naturally arises pertains to the existence of equilibria. If such equilibria do indeed exist, the subsequent question revolves around quantifying the disparity between the socially optimal sample complexity and the complexity needed to attain optimal stability or envy-freeness within a system involving $k$ agents. Lastly, we inquire about the methodology for developing algorithms to identify these equilibria.
\end{question}

\paragraph{Our Results.} In our recent work~\citep*{blum2021one} we first show that the existence of a stable equilibrium depends on whether agents' learning objectives are ``well-behaved''.
In particular, we see that in the PAC learning setting, there may not exist a stable equilibrium, but under mild assumptions, a stable equilibrium exists in the random discovery (aka linear) and random coverage settings. On the other hand, an envy-free equilibrium with equal agent contribution trivially exists. 

Then we show that even for well-behaved learning objectives, such as random discovery and random coverage examples, there is a large gap between the socially optimal sample complexity and the optimal sample complexity achieved by any equilibrium.
In particular, we show that there is a factor $\Omega(\sqrt{k})$ gap between the socially optimal sample complexity and that of optimal stable or envy-free equilibria for $k$ agents.

Regarding algorithmic and structural Properties, we show that in the random discovery (aka linear) setting, in every
optimal stable equilibrium there is a core-set of agents for whom the equilibrium happens to also be socially optimal, and agents who do not belong to this set make $0$ contribution in the equilibrium.
This result allows us to characterize classes of problems where the optimal stable equilibria are also socially optimal.
We further show that in some cases, linear or convex programs can be used to compute socially optimal or optimal stable equilibria.





\subsection{Defection in Intermittently Communicating Algorithms}
Federated learning comes in various forms, ranging from models trained on millions of peripheral devices like Android smartphones to those trained on a limited number of large data repositories. The survey by \citet{kairouz2019advances} categorizes these two contrasting scales of collaboration, which come with distinct system constraints, as \emph{``cross-device''} and \emph{``cross-silo''} federated learning, respectively. This subsection concentrates on a scenario that falls between these two extremes. For example, consider a nationwide medical study led by a government agency to explore the long-term side effects of COVID-19. This agency selects several dozen hospitals to partake in the study to develop a robust model applicable to the entire national populace. Specifically, the server (the governmental agency) has a distribution $\cP$ over agents (hospitals), and each agent $m$ maintains a local data distribution $\ddd_m$ (the distribution of its local patients). The server's goal is to find a model $w$ with low \textbf{population loss}, i.e., 
\begin{equation}
    \mathbb{E}_{m\sim \cP}[F_m(w):= \ee_{z\sim\ddd_m}[f(w;z)]]\,,
\end{equation}
where \(f(w;z)\) represents the loss of model \(w\) at data point \(z\).

Due to constraints like communication overhead, latency, and limited bandwidth, training a model across all agents (say all the hospitals in a country) is infeasible. The server, therefore, aims to achieve its goal by sampling $M$ agents from $\cP$ and minimizing the ``average loss'', given by
\begin{align}\label{eq:relaxed}
    F(w) :=  \frac{1}{M}\sum_{m=1}^M F_m(w) \,.
\end{align}
If the sample size \(M\) is sufficiently large and the server can identify a model with low average loss, likely, the model will also have low population loss, provided the data is only moderately heterogeneous. Hence, our objective (from the agency's perspective) is to find a model with a low average loss. When all $M$ agents share some optima---meaning a model exists that satisfies all participating hospitals---such a model is also universally desirable. However, this collaborative approach may falter when agents aim to reduce their workload or, in the context of hospitals, aim to minimize data collection and local computation.

More specifically, prevalent federated optimization techniques like federated averaging (\textsc{FedAvg}) \citep{mcmahan2016communication} and mini-batch SGD \citep{dekel2012optimal, woodworth2020minibatch}, employ a strategy of intermittent communication. Specifically, for each round $r = 1, \ldots, R$:
\begin{itemize}
    \item 
    \textbf{Server-to-Agent Communication:} The server disseminates a synchronized model $w_{r-1}$ to all participating agents;
    \item \textbf{Local Computation:} Every device initiates local training of its model from $w_{r-1}$ using its own dataset;
    \item \textbf{Agent-to-Server Communication:} Each device transmits the locally computed updates back to the server;
    \item \textbf{Model Update:} The server compiles these updates and revises the synchronized model to $w_r$.
\end{itemize}
If all agents provide their assigned model updates and collaborate effectively, the synchronized model should converge to a final model $w_R$, with a low average loss \( F(w_R) \). However, agents face various costs, such as data collection, computational effort, and potential privacy risks. Thus, rational agents might exit the process once they are content with their current model's performance on their local data.

\textbf{Defections}, or the act of permanently exiting before completing $R$ rounds, can adversely affect the quality of the final model $w_R$. This occurs because defecting agents make their data unavailable, leading to a loss of crucial information for the learning process. The impact is particularly significant if the defecting agent had a large or diverse dataset or was the sole contributor to a specific type of data. Consequently, the final model $w_R$ may fail to achieve a low average loss $F(w_R)$.

\begin{question}\label{q:defection}
Then we have the following questions. Under what conditions are defections detrimental to widely-used FL algorithms like \textsc{FedAvg}? Is it possible to develop an algorithm that mitigates defections while still optimizing effectively?
\end{question}
\paragraph{Our Results.} In our manuscript~\citep*{Han2023defection}, we thoroughly study the effect of defections and how to prevent it.
We begin by distinguishing between benign and harmful defections and exploring the influence of (i) \emph{initial conditions}, (ii) \emph{learning rates}, and (iii) \emph{aggregation methods} on the occurrence of harmful defections. Our findings indicate that simply averaging local updates is insufficient to prevent harmful defections. We further validate our theoretical insights with empirical studies, confirming that defections can substantially degrade the performance of the final model.
Lastly, we introduce our novel algorithm, \textsc{ADA-GD}. Under mild (and possibly necessary) conditions, this algorithm converges to the optimal model for problem \eqref{eq:relaxed} without any agent defecting. 







\subsection{Incentivized Collaboration in Active Learning}
In addition to federated learning, I have also studied incentivized collaboration in active learning. 
Consider a scenario with a new drug like Paxlovid for Covid-19, which exhibits varying efficacy based on patient characteristics. Hospitals individually adopt active learning approaches to test the drug on their patients, but efficient collaboration among hospitals, each treating their own patients, can yield better outcomes. However, maintaining hospital incentives is crucial; otherwise, collaboration may suffer. In the context of data annotating, imagine that several data labeling companies have to recover the labels of unlabeled images assigned to them. Each data labeling company would like to collaborate with other companies to recover the labels of all images while minimizing the query complexity and not increasing their burden.

Let $\cX$ denote the input space, $\cY =\{0,1\}$ denote the label space, and $\cH$ denote the hypothesis class.
Following~\citet{dasgupta2004analysis}, we consider the pool-based active learning in the Bayesian setting, in which the target hypothesis is chosen in advance from some prior distribution $\pi$ over $\cH$. 
In the standard pool-based active learning setting, 
a single agent owns the pool of unlabeled data $X$ and her goal is to recover the labeling of $X$ by querying the labels of the points in the pool.
In the collaborative setting, there are $k$ agents and each agent $i$ has an individual unlabeled data set $X_i$ such that they together compose the pool, $X = \cup_{i\in [k]}X_i$, and each can query points from their own set $X_i$ (but cannot query points which are not in their set).

The collaboration protocol, also called principal, who knows $\xset$, $\cH$ and $\pi$, decides which point should be queried at each iteration, and her goal is to recover all the labels of $X$ using as few queries as possible. 
The goal of each agent is to recover the true labeling of their own set while performing as few queries as possible. 
For any algorithm $\cA$, given an input $\pi$ and any collection of unlabeled data sets $X_1,\ldots,X_\kappa\subseteq X$ of size $\kappa\geq 1$, we denote by $Q(\cA, \pi, \{X_1,\ldots,X_\kappa\})$ the expected (over $h\sim \pi$) number of label queries.
Let $Q_i(\cA, \pi, \{X_1,\ldots,X_\kappa\})$ denote the expected number of queries performed by agent $i$. 
% We remark that in addition to their own sets, each agent knows all the unlabeled data sets,  $\xset$, and the prior distribution $\pi$, otherwise they will not be able to compute $Q_i(\cA',\pi,\xset)$. The principal also has access to $\xset$ and $\pi$ and can therefore make sure these constraints are satisfied. 

Again, we view this collaborative learning as a single-round game, in which agents can decide to join the collaboration or learn individually at the beginning of the learning. And if they join the collaboration, they commit to follow the instructions of the query algorithm. Following the motivating examples, rational agents are modeled with the goal of recovering the labels within their own dataset while minimizing label complexity


\paragraph{Rational agents}
We assume that agents have access to a baseline algorithm and are able to run it on their own local data. 
% Agents can decide to join the collaboration or run the baseline individually at the beginning of the learning.
% If they join the collaboration, they commit to follow the instructions of the query algorithm.
Each agent is incentivized to join the collaboration if she could perform fewer label queries (assuming that all others join the collaboration) by pulling out and running the baseline $\cA$ individually. 
Formally, given a baseline algorithm $\cA$, a collaborative algorithm $\cA'$ is \emph{individually rational (IR)} if 
\begin{equation*}
    {Q_i(\cA',\pi, \xset)} \leq Q(\cA, \pi, \{X_i\}), \forall i\in [k]\,.\label{eq:def-incentive}
\end{equation*}
We say 
 $\cA'$ is \emph{strictly individually rational (SIR)} if
\begin{equation*}
    {Q_i(\cA',\pi, \xset)} < Q(\cA, \pi, \{X_i\}), \forall i\in [k]\,.
\end{equation*}

\begin{question}\label{q:active}
    Given any baseline algorithm $\cA$, how can we construct IR (SIR) collaborative algorithms?
\end{question}
We provide a construction of IR (SIR) collaborative algorithms in the recent manuscript~\citep{Cohen2023incentivized}.

\section{Gaming with Learning Agents}\label{sec:game}
Both strategic classification and incentivized collaboration problems are learning problems involving gaming agents.
Conversely, we study games with learning agents in this section.

Consider a repeated Stackelberg game with policy space $\cP$, action space $\cA$ and the space of nature states $\cY$.
The utilities of both the principal and the agent depend on the principal's policy, the agent's action, and the state of nature.
To illustrate, in the context of contract design, a policy corresponds to a contract, an action could be either working or shirking, and the state of nature might represent the difficulty level of the job.

At round $t=1,\ldots,T$, the principal selects a policy $p_t\in \cP$ and discloses $p_t$ and possibly some additional information to the agent. Then the agent responds by taking an action $a_t\in \cA$. At the end, the state of nature $y_t\in \cY$ is revealed.
Then the principal receives utility $V(a_t,p_t,y_t)$ and the agent receives utility $U(a_t,p_t,y_t)$. 


When there is a common prior $\pi\in \Delta(\cY)$ known to both the principal and the agent and the state of nature $y_t$ is drawn from $\pi$, both the principal and the agent will compute best responses as a function of the common prior. That is to say, for any prior $\pi$, if the principal selects policy $p$, the agent will best respond to $(p, \pi)$ by taking action
\begin{equation*}
    \brr(p,\pi) \in \argmax_{a\in \cA} U(a,p,\pi)\,.
\end{equation*}
Assuming that the agent will best respond, the principal will best respond to $\pi$ by selecting policy
\begin{equation*}
    \brp(\pi) \in \argmax_{p\in \cP} V(\brr(p,\pi),p,\pi)\,.
\end{equation*}
Hence the principal and the agent will choose $(\brp(\pi), \brr(\brp(\pi),\pi))$.

In this section, we study a setting where there is no such a common prior and the states of nature can be generated adversarially. 
Suppose that the principal runs a forecasting algorithm, which provides a forecast $\pi_t\in \Delta(\cY)$ for $y_t$ in each round $t$. 
The principal treats $\pi_t$ as the common prior and best responds to it. Specifically, he selects the optimal policy $p_t = \brp(\pi_t)$ assuming that the agent will best respond to $(p_t,\pi_t)$ and recommends the agent to play the best response $r_t = \brr(p_t,\pi_t)$. This is, however, not necessarily what the agent will do. 
The agent's learning algorithm $L: (\cY\times \cA^2\times \cP)^*\times \cP \mapsto \Delta(\cA)$ maps the state history $y_{1:t-1}$, the action history $a_{1:t-1}$, the recommendation history $r_{1:t-1}$, the policy history $p_{1:t-1}$ and the current policy $p_t$ to a distribution $\mu_t$ over actions. 
We compare the performance of the proposed mechanism to a set of constant mechanisms $\{\sigma^{p_0}|p_0\in \cP\}$ in which the principal consistently implements a fixed policy $p_0 \in \cP$.
For a realized sequence of states of nature $y_{1:T}$ and agent strategy $L$, the principal's (policy) regret is defined as
\begin{equation*}
    \textrm{PR}(L, y_{1:T}) = \max_{p_0\in \cP}\frac{1}{T}\sum_{t=1}^T\left(\EEs{a\sim \mu_t^{p_0}}{V(a,p,y_t)} - \EEs{a\sim \mu_t}{V(a,p_t,y_t)}\right) \,,
\end{equation*}
where $\mu_t^{p_0}$ is the distribution of actions selected by the agent in the counterfactual world of constant mechanism $\sigma^{p_0}$.
Our learning goal is to achieve sub-linear policy regret, i.e., $\textrm{PR}(L, y_{1:T}) = o(T)$.

\begin{question}\label{q:calibrated}
This leads to two fundamental questions.

The first question pertains to modeling the agent's behavior. It becomes evident that achieving sub-linear policy regret is impossible if the agent is allowed to employ any arbitrary learning algorithm. For example, if the learning algorithm consistently favors the principal in a counterfactual world of a constant mechanism, sub-linearity cannot be achieved. As a result, we make the assumption that the learning algorithm exhibits no-internal-regret and lacks any ``secret information''. At a high level, no ``secret information'' means that the agent does not possess additional information about $y_{1:T}$.

Another important issue is the matter of tie-breaking. Consider a scenario where two actions are almost indifferent to the agent but lead to different principal's utility. In this case, ensuring sub-linear regret becomes a challenge if the agent consistently selects the ``favorable'' action (from the principal's perspective) in the counterfactual world of a constant mechanism and the ``unfavorable'' action in the real world of the proposed mechanism.
\end{question}

The material discussed in this section is based on an
ongoing project with Natalie Collina and Aaron Roth.

\section{Plan}
I have completed the projects related to research questions~\ref{q:clean-label}, \ref{q:da}, \ref{q:strategic}, \ref{q:multiobj-MDP}, \ref{q:primary-secondary}, \ref{q:one4one}, \ref{q:defection}, and \ref{q:active}. Work on the project addressing question~\ref{q:calibrated} is in progress. While I intend to investigate questions~\ref{q:strategic-combinatorial}, \ref{q:strategic-nonball}, \ref{q:strategic-agnostic}, it is not guaranteed that these results will be present in my thesis.

==> strategic-finite/src/abstract.tex <==
\begin{abstract}
We study the fundamental mistake bound and sample complexity in the strategic classification, where agents can strategically manipulate their feature vector up to an extent in order to be predicted as positive. For example, given a classifier determining college admission, student candidates may try to take easier classes to improve their GPA, retake SAT and change schools in an effort to fool the classifier. \textit{Ball manipulations} are a widely studied class of manipulations in the literature, where agents can modify their feature vector within a bounded radius ball. Unlike most prior work, our work considers manipulations to be \textit{personalized}, meaning that agents can have different levels of manipulation abilities (e.g., varying radii for ball manipulations), and \textit{unknown} to the learner.

We formalize the learning problem in an interaction model where the learner first deploys a classifier and the agent manipulates the feature vector within their manipulation set to game the deployed classifier. We investigate various scenarios in terms of the information available to the learner during the interaction, such as observing the original feature vector before or after deployment, observing the manipulated feature vector, or not seeing either the original or the manipulated feature vector. We begin by providing online mistake bounds and PAC sample complexity in these scenarios for ball manipulations. We also explore non-ball manipulations and show that, even in the simplest scenario where both the original and the manipulated feature vectors are revealed, the mistake bounds and sample complexity are lower bounded by $\Omega(|\mathcal{H}|)$ when the target function belongs to a known class $\mathcal{H}$.
\end{abstract}

==> strategic-finite/src/ack.tex <==
\section*{Acknowledgements}
% \vspace{-5pt}
This work was supported in part by the National Science Foundation under grant CCF-2212968, by the Simons Foundation under the Simons Collaboration on the Theory of Algorithmic Fairness, by the Defense Advanced Research Projects Agency under cooperative agreement HR00112020003. The views expressed in this work do not necessarily reflect the position or the policy of the Government and no official endorsement should be inferred. Approved for public release; distribution is unlimited.

==> strategic-finite/src/extra_related_work.tex <==
\section{Additional Related Work}\label{app:relatedwork}
There has been a lot of research on various other issues and models in strategic classification. 
Beyond sample complexity, \cite{hu2019disparate,milli2019social} focused on other social objectives, such as social burden and fairness. 
Recent works also explored different models of agent behavior, including
proactive agents~\cite{zrnic2021leads}, non-myopic agents~\citep{haghtalab2022learning} and noisy agents~\citep{jagadeesan2021alternative}.
\cite{ahmadi2023fundamental} considers two agent models of randomized learners: a randomized algorithm model where the agents respond to the realization, and a fractional classifier model where agents respond to the expectation, and our model corresponds to the randomized algorithm model.
Additionally, there is also a line of research on agents interested in improving their qualifications instead of gaming~\citep{kleinberg2020classifiers, haghtalab2020maximizing,ahmadi2022classification}.
Strategic interactions in the regression setting have also been studied~\citep{bechavod2021gaming}.

Beyond strategic classification, there is a more general research area of learning using data from strategic sources, such as a single data generation player who manipulates the data distribution~\citep{bruckner2011stackelberg,dalvi2004adversarial}. Adversarial perturbations can be viewed as another type of strategic source~\citep{montasser2019vc}.

==> strategic-infinite/sec/ack.tex <==
Lee Cohen is supported by the Simons Foundation Collaboration on the Theory of Algorithmic Fairness, the Sloan Foundation Grant 2020-13941, and the Simons Foundation investigators award 689988.

Yishay Mansour was supported by funding from the European Research Council (ERC) under the European Union’s Horizon 2020 research and innovation program (grant agreement No. 882396), by the Israel Science Foundation,  the Yandex Initiative for Machine Learning at Tel Aviv University and a grant from the Tel Aviv University Center for AI and Data Science (TAD).


Shay Moran is a Robert J.\ Shillman Fellow; he acknowledges support by ISF grant 1225/20, by BSF grant 2018385, by an Azrieli Faculty Fellowship, by Israel PBC-VATAT, by the Technion Center for Machine Learning and Intelligent Systems (MLIS), and by the the European Union (ERC, GENERALIZATION, 101039692). Views and opinions expressed are however those of the author(s) only and do not necessarily reflect those of the European Union or the European Research Council Executive Agency. Neither the European Union nor the granting authority can be held responsible for them.


Han Shao was supported in part by the National Science Foundation under grants CCF-2212968 and ECCS-2216899, by the Simons Foundation under the Simons Collaboration on the Theory of Algorithmic Fairness, and by the Defense Advanced Research Projects Agency under cooperative agreement HR00112020003. The views expressed in this work do not necessarily reflect the position or the policy of the Government and no official endorsement should be inferred.

==> strategic-infinite/sec/related.tex <==
Our work aligns with strategic classification, a recent line of research that explores the influence of strategic behavior on decision making and machine learning algorithms. This line of study is extensive and encompasses various settings, including distributional vs. online, different knowledge of manipulation structure, pre-manipulation vs. post-manipulation feedback, and the goals of gaming vs. improving. However, none of the prior work has addressed the learnability gaps between standard learning and strategic learning studied in this work.



Strategic classification was first studied in a distributional model by~\cite{hardt2016strategic}, assuming that agents manipulate by best responding with respect to a uniform cost function known to the learner. Building on the framework of \cite{hardt2016strategic}, \cite{lechner2022learning,hu2019disparate,milli2019social,sundaram2021pac,zhang2021incentive} studied the distributional learning problem with the goal of returning a classifier with small strategic population loss, and all of them assumed that the manipulations are predefined and known to the learner, either by a cost function or a predefined manipulation graph. Then \cite{lechner2023strategic} and \cite{shao2023strategic} studied the unknown manipulation structure. However, \cite{lechner2023strategic} considered a different loss function that penalizes manipulation even when the prediction at the manipulated feature is correct, and \cite{shao2023strategic} provided guarantees only for finite hypothesis classes.

For the online setting,
\cite{chen2020learning, dong2018strategic,ahmadi2021strategic,ahmadi2023fundamental,shao2023strategic} studied Stackelberg regret in the online setting learning. 
However, \cite{dong2018strategic} studied Stackelberg regret in linear classification and focused on finding appropriate conditions of the cost function to achieve sub-linear Stackelberg regret.
\cite{chen2020learning} studied linear classification under uniform ball manipulations and  \cite{ahmadi2021strategic,ahmadi2023fundamental} studied Stackelberg regret under a predefined and known manipulation. \cite{shao2023strategic} studied the mistake bound under unknown manipulation structures, but only provided results for finite hypothesis classes.

\paragraph{Models of manipulation structure} \cite{hardt2016strategic} modeled manipulation structure by a cost function, where agents manipulate to maximize their utility function, which is the reward of obtaining a positive prediction minus the cost of manipulation.
It then naturally leads to two modeling ways of manipulation structure: The first is a geometric model (e.g., ~\cite{dong2018strategic,sundaram2021pac,chen2020learning, Ghalme21,haghtalab2020maximizing,ahmadi2021strategic,shao2023strategic}), where each agent is able to manipulate within a bounded-radius ball in some known metric space. Other works (e.g., \cite{zhang2021incentive,lechner2022learning,lechner2023strategic,ahmadi2023fundamental}) modeled feasible manipulations using a manipulation graph, where each agent is represented by a node $x$, and an arc from $x$ to $x'$ indicates that an agent with the feature vector $x$ may adjust their features to $x'$ if it increases their likelihood of receiving a positive classification. However, these two ways of modeling are actually equivalent as we can define a manipulation graph given the manipulation balls and we can define ball manipulations w.r.t. the graph distance on a predefined known graph. 

\paragraph{Different information settings}
All PAC learning scenarios involving either known manipulation structures or known local neighborhoods \citep{hardt2016strategic,lechner2022learning,sundaram2021pac,zhang2021incentive,hu2019disparate,milli2019social} can be encompassed within our fully informative setting. We remark that the work of \cite{lechner2022learning} considered the task of learning the manipulation graph, but assumed that each sample is of the form $(x,$ neighborhood of $x)$, which is closer to our fully informative setting as our results also only require the neighborhood information.
\cite{ahmadi2021strategic} examined online learning within our fully informative setting, while \cite{ahmadi2023fundamental} explored online learning within our post-manipulation feedback setting.
Regarding unknown graph settings, \cite{lechner2023strategic} and \cite{shao2023strategic} have made contributions. However, \cite{lechner2023strategic} considered a different loss function that penalizes manipulation even when the prediction at the manipulated feature is correct and \cite{shao2023strategic} provided guarantees solely based on the cardinality of the hypothesis class.
We primarily study strategic classification in online and distributional settings in various restrictive feedback settings. 

% \paragraph{Gaming vs. improving} 



\paragraph{Other works.} Other works explored strategic classification in various contexts, e.g.: noisy classifiers~\citep{Braverman20}, causality~\citep{miller2020strategic,shavit2020causal}, noisy agents~\citep{jagadeesan2021alternative}, decision making~\citep{Khajehnejad19,tang2021linear}, sequential setting~\citep{cohen23}, social objectives (e.g., social burden)~\citep{hu2019disparate, Liu20,milli2019social,lechner2023strategic}, Strategic interactions in the regression~\citep{bechavod2021gaming}, non-myopic agents~\citep{haghtalab2022learning,harris2021stateful}, and lack of transparency in decision rules~\citep{bechavod2022information}.
Beyond strategic classification, there is a more general research area of learning using data from strategic sources, such as a single data generation player who manipulates the data distribution~\citep{bruckner2011stackelberg,dalvi2004adversarial}. Adversarial perturbations can be viewed as another type of strategic source~\citep{montasser2019vc}.














% including~\citep{bruckner2011stackelberg, hardt2016strategic,kleinberg2020classifiers, Braverman20,miller2020strategic,Liu20,jagadeesan2021alternative,Reshef10,Reshef11,dekel2010incentive,Chen18,Cummings15,Khajehnejad19,tang2021linear,hu2019disparate,milli2019social,performative2020,ahmadi2022classification,bechavod2021gaming, bechavod2022information,cohen23,haghtalab2022learning,shavit2020causal,harris2021stateful}.





% The most related work to ours is that of~\cite{ahmadi2023fundamental}.
% They considered the online setting we present as post-manipulation feedback-- i.e., the manipulation graph is known and the feature is revealed to the learner after implementing the selected hypothesis. They used the maximum out-degree of the manipulation graph to upper and lower bounded the Stackelberg regret. But different from our work, they only consider finite hypothesis class, and their results are based on the cardinality of the hypothesis class. 


% They studied two agent models of randomized learners: a randomized algorithm model where the agents respond to the realization of the selected hypothesis and a fractional classifier model where agents respond to the expectation. They derive results for finite hypotheses classes, and we generalize these results for any hypothesis class with finite complexity measures (VC-dim for the PAC case and Littlestone dimension for online). 

% We remark that the work of \cite{lechner2022learning} considered the task of learning the manipulation graph, but assumed that each sample is of the form $(x,$neighberhood of $x)$, which provides much more information than what we assumed to be available (which is $(x,$ a single neighbor of $x)$.



\begin{comment}
\textcolor{blue}{
- distributional setting with known graph \citep{hardt2016strategic,lechner2022learning,sundaram2021pac,zhang2021incentive,hu2019disparate,milli2019social}\\
-online setting with known graph and feature before implementing the learner~\citep{ahmadi2021strategic}\\
- online setting with known graph and feature after implementing the learner~\citep{ahmadi2023fundamental}\\
-distributional setting with an unknown graph, knowing manipulated feature afterward
\citep{lechner2023strategic}, all feature information settings \citep{shao2023strategic} \\
-online setting with an unknown graph, all feature information settings\citep{shao2023strategic}\\
-\citep{haghtalab2022learning},\citep{bechavod2022information}, \citep{chen2020learning}\\
===========below is the related work from my previous work=======\\
\paragraph{Related work}
% \textbf{Related work }
Our work is primarily related to strategic classification in online and distributional settings.
Strategic classification was first studied in a distributional model by~\cite{hardt2016strategic} and subsequently by~\cite{dong2018strategic} in an online model.
\cite{hardt2016strategic} assumed that agents manipulate by best response with respect to a uniform cost function known to the learner.
Building on the framework of \citep{hardt2016strategic}, \cite{lechner2022learning,sundaram2021pac,zhang2021incentive,hu2019disparate,milli2019social} studied the distributional learning problem, and all of them assumed that the manipulations are predefined and known to the learner, either by a cost function or a predefined manipulation graph.
For online learning, \cite{dong2018strategic} considered a similar manipulation setting as in this work, where manipulations are personalized and unknown. However, they studied linear classification with ball manipulations in the online setting and focused on finding appropriate conditions of the cost function to achieve sub-linear Stackelberg regret.
\cite{chen2020learning} also studied Stackelberg regret in linear classification with uniform ball manipulations. \cite{ahmadi2021strategic} studied the mistake bound under uniform (possbily unknown) ball manipulations, and \cite{ahmadi2023fundamental} studied regret under a predefined and known manipulation.
The most relevant work is a recent concurrent study by~\cite{lechner2023strategic}, which also explores strategic classification involving unknown personalized manipulations but with a different loss function. 
In their work, a learner incurs a loss of $0$ if and only if the agent refrains from manipulation and the learner correctly predicts at the unmanipulated feature vector. 
In our work, the learner's loss is $0$ if it correctly predicts at the manipulated feature, even when the agent manipulates.
As a result, their loss function serves as an upper bound of our loss function.\\
There has been a lot of research on various other issues and models in strategic classification. 
Beyond sample complexity, \cite{hu2019disparate,milli2019social} focused on other social objectives, such as social burden and fairness. 
Recent works also explored different models of agent behavior, including
proactive agents~\cite{zrnic2021leads}, non-myopic agents~\citep{haghtalab2022learning} and noisy agents~\citep{jagadeesan2021alternative}.
\cite{ahmadi2023fundamental} considers two agent models of randomized learners: a randomized algorithm model where the agents respond to the realization, and a fractional classifier model where agents respond to the expectation, and our model corresponds to the randomized algorithm model.
Additionally, there is also a line of research on agents interested in improving their qualifications instead of gaming~\citep{kleinberg2020classifiers, haghtalab2020maximizing,ahmadi2022classification}.
Strategic interactions in the regression setting have also been studied (e.g.,~\cite{bechavod2021gaming}).\\
Beyond strategic classification, there is a more general research area of learning using data from strategic sources, such as a single data generation player who manipulates the data distribution~\citep{bruckner2011stackelberg,dalvi2004adversarial}. Adversarial perturbations can be viewed as another type of strategic source~\citep{montasser2019vc}.}

% We postpone the discussion of studies on other objectives and models in the strategic setting to the Appendix~\ref{app:relatedwork}.

% There has been a lot of research on various other issues and models in strategic classification. 
% Beyond sample complexity, \cite{hu2019disparate,milli2019social} focused on other social objectives, such as social burden and fairness. 
% Recent works also explored different models of agent behavior, including
% proactive agents~\cite{zrnic2021leads}, non-myopic agents~\citep{haghtalab2022learning} and noisy agents~\cite{jagadeesan2021alternative}.
% Additionally, there is also a line of research on agents interested in improving their qualifications instead of gaming~\cite{kleinberg2020classifiers, haghtalab2020maximizing,ahmadi2022classification}.

% Beyond strategic classification, there is a more general research area of learning using data from strategic source, such as a single data generation player who manipulates the data distribution~\cite{bruckner2011stackelberg,dalvi2004adversarial}. Adversarial perturbations can be viewed as another type of strategic source~\citep{montasser2019vc}.
\end{comment}

==> todos.tex <==

%%% todos
\usepackage[textsize=scriptsize]{todonotes} % Add the 'disable' flag to hide comments
\usepackage{xspace}
\setlength{\marginparsep}{0.2cm} % Changing these seems to have no effect
\setlength{\marginparwidth}{1.9cm}


%\usepackage[colorinlistoftodos, textwidth=30mm, shadow, textsize=small]{todonotes}
%\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
%\definecolor{citrine}{rgb}{0.89, 0.82, 0.04}
\definecolor{misocolor}{rgb}{0.16,0.27,0.86}
%\newcommand{\todom}[1]{\todo[color=misocolor!30]{#1}\xspace}
%\newcommand{\todomi}[1]{\todo[inline,color=misocolor!30]{#1}}

\definecolor{graphicbackground}{rgb}{0.96,0.96,0.8}
\definecolor{rouge1}{RGB}{226,0,38}  % red P
\definecolor{orange1}{RGB}{243,154,38}  % orange P
\definecolor{jaune}{RGB}{254,205,27}  % jaune P
\definecolor{blanc}{RGB}{255,255,255} % blanc P
\definecolor{rouge2}{RGB}{230,68,57}  % red S
\definecolor{orange2}{RGB}{236,117,40}  % orange S
\definecolor{taupe}{RGB}{134,113,127} % taupe S
\definecolor{gris}{RGB}{91,94,111} % gris S
\definecolor{bleu1}{RGB}{38,109,131} % bleu S
\definecolor{bleu2}{RGB}{28,50,114} % bleu S
\definecolor{vert1}{RGB}{133,146,66} % vert S
\definecolor{vert3}{RGB}{20,200,66} % vert S
\definecolor{vert2}{RGB}{157,193,7} % vert S
\definecolor{darkyellow}{RGB}{233,165,0}  % orange S
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}
\definecolor{darkgray}{rgb}{0.6,0.6,0.6}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{citrine}{rgb}{0.89, 0.82, 0.04}
\definecolor{misogreen}{rgb}{0.25,0.6,0.0}

\newcommand{\rcol}[1]{\textcolor{red}{\textit{#1}}}
\newcommand{\defcol}[1]{\textcolor{vert3}{\textbf{#1}}}
\newcommand{\yellcol}[1]{\textcolor{babyblue}{\textbf{#1}}}
\newcommand{\gcol}[1]{\textcolor{vert3}{\textbf{#1}}}

\newcommand{\emphcol}[1]{\textcolor{vert3}{\textbf{#1}}}

\newcommand{\grcol}[1]{\textcolor{gray}{#1}}
\newcommand{\notecol}[1]{\textcolor{gray}{#1}}

\newcommand{\bcol}[1]{\textcolor{blue}{\textit{#1}}}
\newcommand{\ycol}[1]{\textcolor{darkyellow}{\textit{#1}}}
\newcommand{\rcolb}[1]{\textcolor{red}{\textit{\textbf{#1}}}}
\newcommand{\gcolb}[1]{\textcolor{vert3}{\textit{\textbf{#1}}}}
\newcommand{\bcolb}[1]{\textcolor{blue}{\textit{\textbf{#1}}}}
\newcommand{\ycolb}[1]{\textcolor{darkyellow}{\textit{\textbf{#1}}}}
\newcommand{\mcolA}[1]{{\color{bleu1} #1}}
\newcommand{\mcolB}[1]{{\color{darkyellow} #1}}
\newcommand{\mcolC}[1]{{\color{misogreen} #1}}
\newcommand{\hs}[1]{\todo[inline,color=meganta]{{\it HS:~}#1}}
\newcommand{\todohs}[1]{\todo[fancyline,color=magenta!40]{HS: #1}\xspace}

